Job Dispatching Policies for Queueing Systems with Unknown Service Rates

In multi-server queueing systems where there is no central queue holding all incoming jobs, job dispatching policies are used to assign incoming jobs to the queue at one of the servers. Classic job dispatching policies such as join-the-shortest-queue and shortest expected delay assume that the service rates and queue lengths of the servers are known to the dispatcher. In this work, we tackle the problem of job dispatching without the knowledge of service rates and queue lengths, where the dispatcher can only obtain noisy estimates of the service rates by observing job departures. This problem presents a novel exploration-exploitation trade-off between sending jobs to all the servers to estimate their service rates, and exploiting the currently known fastest servers to minimize the expected queueing delay. We propose a bandit-based exploration policy that learns the service rates from observed job departures. Unlike the standard multi-armed bandit problem where only one out of a finite set of actions is optimal, here the optimal policy requires identifying the optimal fraction of incoming jobs to be sent to each server. We present a regret analysis and simulations to demonstrate the effectiveness of the proposed bandit-based exploration policy.

==> header.tex <==
\newif\ifmoment
%\momenttrue
\newif\iflong
\longtrue
\newif\ifNIPS
%\NIPStrue
\newif\ifShowDeprecated
%\ShowDeprecatedtrue
\newif\ifNotForSubmission
\NotForSubmissiontrue
%\documentclass[11pt]{article}


\ifNIPS

\PassOptionsToPackage{numbers,sort,compress}{natbib}
\usepackage{neurips_2019}

\usepackage[format=hang,font={footnotesize}]{caption}
\else
%\documentclass[11pt,letterpaper]{article}
\usepackage[papersize={8.5in,11in},margin=1in]{geometry}
\usepackage[numbers,sort,compress]{natbib} % flexible bibliography support
\usepackage[format=hang,font={footnotesize}]{caption}
\fi
\usepackage[title]{appendix}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
% \usepackage{algorithmic}
% \usepackage{subfigure}
\usepackage{wrapfig}
\usepackage{color}
\usepackage{enumitem}
\usepackage{parskip}

\usepackage{graphicx}
\usepackage{dirtytalk}
\usepackage{complexity}
\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{setspace}
\usepackage{subcaption}

\usepackage{tcolorbox}

\usepackage{url}
\usepackage{graphicx}
\usepackage{color}
\usepackage{algorithm} % pseudocode support
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
%\renewcommand\algorithmiccomment[1]{ \hfill $\diamond$ \ {\footnotesize \em #1} }

\usepackage{xspace}
\usepackage{dsfont} % to allow mathds (mathbb)
\usepackage{pifont} % to allow circled numbers
\usepackage{bbm}
\usepackage{comment}
\usepackage{float}
\usepackage{listings}
\usepackage{xcolor}
% \usepackage[colorinlistoftodos]{todonotes}

\newtheorem{innercustomthm}{Theorem}
\newenvironment{stheorem}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
\newtheorem{innercustomlemma}{Lemma}
\newenvironment{slemma}[1]
  {\renewcommand\theinnercustomlemma{#1}\innercustomlemma}
  {\endinnercustomlemma}
\newtheorem{innercustomclaim}{Claim}
\newenvironment{sclaim}[1]
  {\renewcommand\theinnercustomclaim{#1}\innercustomclaim}
  {\endinnercustomclaim}
\newtheorem{ctheorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Theorem}[section]
\newtheorem{claim}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{ccorollary}[ctheorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{cconcept}{Concept}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{lem}[lemma]{Lemma}
\newtheorem{clm}[claim]{Claim}
\newtheorem{property}[theorem]{Property}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{conj}[theorem]{Conjecture}
\newtheorem*{assumption*}{Assumption}
\newtheorem*{question*}{Question}


\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}


\newreptheorem{theorem}{Theorem}
\newreptheorem{lemma}{Lemma}
\newreptheorem{proposition}{Proposition}
\newreptheorem{claim}{Claim}
\newreptheorem{definition}{Definition}
%\newreptheorem{problem}{Problem}


%\ifCOLT\else
\theoremstyle{definition}
%\fi
\newtheorem{construction}[theorem]{Construction}
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{problem}[theorem]{Problem} %%% added by Zhao
\newtheorem{param}[theorem]{Parameter}
\newtheorem*{defn}{Definition}
\newtheorem*{exmp}{Example}

\captionsetup[subfigure]{subrefformat=simple,labelformat=simple}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
 
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=none,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
\lstset{style=mystyle}
%\ifCOLT\else
\theoremstyle{remark}
%\fi
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem*{note}{Notation}
\newtheorem{case}{Case}
\newtheorem*{rem}{Remark}
\newtheorem*{hnote}{Historical Note}
\newtheorem*{ack}{Acknowledgments}
\newtheorem{example}[theorem]{Example}

\numberwithin{equation}{section}

\newenvironment{proofsketch}{\noindent{\it Proof sketch.}\hspace*{1em}}{\qed\bigskip}

%\ifCOLT\else
\renewcommand{\qedsymbol}{\hfill{\Large $\square$}}
%\fi
\newcommand{\bqed}{\hfill{\Large $\blacksquare$}}



\newcommand{\namedref}[2]{\mbox{\hyperref[#2]{#1~\ref*{#2}}}}

\newcommand{\chapterref}[1]{\namedref{Chapter}{#1}}
\newcommand{\sectionref}[1]{\namedref{Section}{#1}}
\newcommand{\appendixref}[1]{\namedref{Appendix}{#1}}
\newcommand{\theoremref}[1]{\namedref{Theorem}{#1}}
\newcommand{\factref}[1]{\namedref{Fact}{#1}}
\newcommand{\remarkref}[1]{\namedref{Remark}{#1}}
\newcommand{\definitionref}[1]{\namedref{Definition}{#1}}
\newcommand{\figureref}[1]{\namedref{Figure}{#1}}
\newcommand{\figurerefb}[2]{\mbox{\hyperref[#1]{Figure~\ref*{#1}#2}}}
\newcommand{\tableref}[1]{\namedref{Table}{#1}}
\newcommand{\lemmaref}[1]{\namedref{Lemma}{#1}}
\newcommand{\claimref}[1]{\namedref{Claim}{#1}}
\newcommand{\propositionref}[1]{\namedref{Proposition}{#1}}
\newcommand{\corollaryref}[1]{\namedref{Corollary}{#1}}
\newcommand{\constructionref}[1]{\namedref{Construction}{#1}}
\newcommand{\itemref}[1]{\namedref{Item}{#1}}
\newcommand{\propertyref}[1]{\namedref{Property}{#1}}
\newcommand{\protocolref}[1]{\namedref{Protocol}{#1}}
\newcommand{\algorithmref}[1]{\namedref{Algorithm}{#1}}
\newcommand{\assumptionref}[1]{\namedref{Assumption}{#1}}
\newcommand{\conceptref}[1]{\namedref{Concept}{#1}}
\newcommand{\stepref}[1]{\namedref{Step}{#1}}
\newcommand{\paramref}[1]{\namedref{Parameter}{#1}}
\newcommand{\footnoteref}[1]{\namedref{Footnote}{#1}}
\newcommand{\equationref}[1]{\mbox{\hyperref[#1]{(\ref*{#1})}}}
\renewcommand{\eqref}{\equationref}
%\newcommand{\equationref}[1]{\namedref{Equation}{#1}}
\newcommand{\exampleref}[1]{\namedref{Example}{#1}}
\newcommand{\plineref}[1]{\namedref{Line}{#1}}


\newcommand{\var}{\mathbf{Var}}
\newcommand{\new}{{(\mathsf{new})}}

\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}
\DeclareMathOperator*{\sign}{sign}

\makeatletter
% LeftRightArrow
\newcommand\xLongLeftRightArrow[2][]%
  {\ext@arrow 0099{\LongLeftRightArrowfill@}{#1}{#2}}
\def\LongLeftRightArrowfill@
  {\arrowfill@\Leftarrow\Relbar\Rightarrow}
% Rightarrow
\newcommand\xLongRightArrow[2][]%
  {\ext@arrow 0099{\LongRightArrowfill@}{#1}{#2}}
\def\LongRightArrowfill@
  {\arrowfill@\Relbar\Relbar\Rightarrow}
\makeatother


% defeq
\iflong
\newcommand{\defeq}{\stackrel{\mathrm{\scriptscriptstyle def}}{=}}
\newcommand{\defem}[1]{\textsf{#1}}
\else
\newcommand{\defeq}{:=}
\newcommand{\defem}[1]{\emph{\textsf{\small #1}}}
\fi

% paragraph headings
\newcommand{\loss}{\mathbf{Obj}}
\newcommand{\lossh}{\tilde{\mathbf{Obj}}}
\newcommand{\lloss}{\mathbf{Loss}}
\newcommand{\llossh}{\tilde{\mathbf{Loss}}}
\newcommand{\xE}{{\mathsf{xE}}}
\newcommand{\CE}{{\mathsf{CE}}}
\newcommand{\reg}{\mathbf{Reg}}
\renewcommand{\bar}{\overline}
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\emptyset}{\varnothing}

\newcommand{\da}{\text{\ding{172}}\xspace}
\newcommand{\db}{\text{\ding{173}}\xspace}
\newcommand{\dc}{\text{\ding{174}}\xspace}
\newcommand{\dd}{\text{\ding{175}}\xspace}
\newcommand{\de}{\text{\ding{176}}\xspace}
\newcommand{\df}{\text{\ding{177}}\xspace}
\newcommand{\dg}{\text{\ding{178}}\xspace}

\newcommand{\tW}{\tilde{W}}
\newcommand{\SUM}{\mathbf{Sum}}
\newcommand{\SYM}{\mathbf{Sym}}
\newcommand{\Fstar}{G^\star}
\newcommand{\tA}{\tilde{A}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\ta}{\tilde{a}}
\newcommand{\tg}{\tilde{g}}
\newcommand{\tD}{\tilde{D}}

\newcommand{\Ws}{W^\divideontimes}
\newcommand{\ws}{w^\divideontimes}

%\newcommand{\bWz}{{\bW^{(0)}}}
%\newcommand{\bVz}{{\bV^{(0)}}}
%\renewcommand{\star}{\divideontimes}
\newcommand{\bWbar}{\breve{\bW}}
\newcommand{\bWhat}{\bar{\bar{\bW}}}
\newcommand{\bWp}{\bW'}
\newcommand{\bWg}{\bW^\star}
\newcommand{\kappap}{\tilde{\kappa}}
\newcommand{\kb}{\bar{k}}
\newcommand{\Bb}{\bar{B}}
\newcommand{\bVg}{\bV^\star}
\newcommand{\bVgg}{\bV^{\star,w}}
\newcommand{\bDp}{\bD'}
\newcommand{\bDpp}{\bD''}
\newcommand{\bDz}{\tilde{\bD}}
\newcommand{\bDbar}{\breve{\bD}}
\newcommand{\bDs}{\bD^{\mathsf{0/1}}}
\newcommand{\hp}{h'}
\newcommand{\hz}{\tilde{h}}
\renewcommand{\hbar}{\breve{h}}
\newcommand{\gp}{g'}
\newcommand{\gz}{g^{(0)}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\gbar}{\breve{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\lhat}{\hat{\loss}}
\newcommand{\lbar}{\breve{\loss}}
\newcommand{\done}{\mathds{1}}
\newcommand{\II}{\mathds{1}}
\newcommand{\tauS}{\tau_\triangledown}
\newcommand{\xs}{x^\star}
\newcommand{\ys}{y^\star}
\newcommand{\dx}{{d_x}}
\newcommand{\vepss}{\veps_{\mathsf{s}}}
\newcommand{\vepsx}{\veps_x}
\newcommand{\vepsc}{\veps_c}
\newcommand{\vepse}{\veps_e}
\newcommand{\complexity}{\mathfrak{C}}
\newcommand{\complexitys}{\mathfrak{C}_\mathfrak{s}}
\newcommand{\complexityE}{\mathfrak{C}_\veps}
\newcommand{\complexityalpha}{\mathfrak{C}_\alpha}
\newcommand{\complexitytalpha}{\mathfrak{C}_{\tilde{\alpha}}}
\newcommand{\obj}{\mathsf{Obj}}

\newcommand{\TauZeroBound}{\rhob^{100}}
\newcommand{\rhob}{\varrho}
\newcommand{\rhobVal}{n L d \delta^{-1} \log (m/\veps)}

\newcommand{\veps}{\varepsilon}
\newcommand{\GS}{\mathsf{GS}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\sgn}{\mathsf{sgn}}
\newcommand{\lmax}{\lambda_{\max}}
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\Va}{\mathcal{V}}

\newcommand{\out}{\mathsf{out}}
\newcommand{\outK}{\mathfrak{K}}
\newcommand{\outF}{\mathfrak{F}}
\newcommand{\outa}{\mathsf{out}_1}
\newcommand{\Lg}{\mathfrak{L}_\cG}
\newcommand{\Bf}{\mathfrak{B}_\cF}
\newcommand{\Bg}{\mathfrak{B}_\cG}
\newcommand{\Bfg}{\mathfrak{B}_{\cF\circ \cG}}
\newcommand{\az}{a}
\newcommand{\bz}{b}
\newcommand{\ReLU}{\sigma}



\newcommand{\nbr}[1]{{\left\| {#1} \right\|}}

\renewcommand{\E}{\operatornamewithlimits{\mathbb{E}}}
\renewcommand{\Pr}{\operatornamewithlimits{\mathbf{Pr}}}
\newcommand{\Lap}{\mathcal{L}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Real}{\mathbb{R}}
%\newcommand{\dd}{\rm{d}}
%\newcommand{\PP}{\rm{P}}
\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\NumContext}{N}
%\newcommand{\diag}{\textsf{diag}}

\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cF}{\mathcal{F}}
%\newcommand{\cS}{\mathcal{S}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cI}{\mathcal{I}}

\newcommand{\N}{\mathcal{N}}

\newcommand{\matrixstyle}{\mathbf}
\newcommand{\bF}{\matrixstyle{F}}
\newcommand{\bE}{\matrixstyle{E}}
\newcommand{\bC}{\matrixstyle{C}}
\newcommand{\bN}{\matrixstyle{N}}
\newcommand{\bM}{\matrixstyle{M}}
\newcommand{\bA}{\matrixstyle{A}}
\newcommand{\bAg}{\matrixstyle{A}^\star}
\newcommand{\bB}{\matrixstyle{B}}
\newcommand{\bX}{\matrixstyle{X}}
\newcommand{\bY}{\matrixstyle{Y}}
\newcommand{\bU}{\matrixstyle{U}}
\newcommand{\bu}{\matrixstyle{u}}
\newcommand{\bV}{\matrixstyle{V}}
\newcommand{\bL}{\matrixstyle{L}}
\newcommand{\btV}{\widetilde{\matrixstyle{V}}}
\newcommand{\bG}{\matrixstyle{G}}
\newcommand{\bH}{\matrixstyle{H}}
\newcommand{\bO}{\matrixstyle{O}}
\newcommand{\bP}{\matrixstyle{P}}
\newcommand{\bQ}{\matrixstyle{Q}}
\newcommand{\btE}{\widetilde{\matrixstyle{E}}}
\newcommand{\bD}{\matrixstyle{D}}
\newcommand{\bJ}{\matrixstyle{J}}
\newcommand{\bK}{\matrixstyle{K}}
\newcommand{\bR}{\matrixstyle{R}}
\newcommand{\btR}{\matrixstyle{\widetilde{R}}}
\newcommand{\btQ}{\matrixstyle{\widetilde{Q}}}
\newcommand{\bS}{\matrixstyle{S}}
\newcommand{\bI}{\matrixstyle{I}}
\newcommand{\btM}{\widetilde{\matrixstyle{M}}}
\newcommand{\bT}{\matrixstyle{T}}
\newcommand{\bTb}{\matrixstyle{T}_{\bot}}
\newcommand{\btXb}{\widetilde{\matrixstyle{X}}_{\bot}}
\newcommand{\btX}{\widetilde{\matrixstyle{X}}}
\newcommand{\bbX}{\overline{\matrixstyle{X}}}
\newcommand{\btY}{\widetilde{\matrixstyle{Y}}}
\newcommand{\btYb}{\widetilde{\matrixstyle{Y}}_{\bot}}
\newcommand{\bbY}{\overline{\matrixstyle{Y}}}
\newcommand{\btSigma}{\widetilde{\matrixstyle{\Sigma}}}
\newcommand{\bZ}{\matrixstyle{Z}}
\newcommand{\bW}{\matrixstyle{W}}
\newcommand{\bOne}{\matrixstyle{1}}

\newcommand{\ckappa}{\tau}
\newcommand{\bSigma}{\matrixstyle{\Sigma}}
\newcommand{\bDelta}{\matrixstyle{\Delta}}
%\newcommand{\bMg}{\matrixstyle{M}^*}
\newcommand{\bNoise}{\matrixstyle{N}}
\newcommand{\bGamma}{\matrixstyle{\Gamma}}
\newcommand{\bLambda}{\matrixstyle{\Lambda}}

\newcommand{\tY}{\widetilde{\matrixstyle{Y}}}

\newcommand{\bbSigma}{\overline{\matrixstyle{\Sigma}}}

\newcommand{\dmaxp}{D_2}
\newcommand{\dmax}{D_1}
\newcommand{\sP}{\set{P}}

%\newcommand{\Us}{(\bU^*)}
%\newcommand{\Vs}{(\bV^*)}

\newcommand{\bUb}{\matrixstyle{U}_{\bot}}
\newcommand{\bVb}{\matrixstyle{V}_{\bot}}
\newcommand{\bXb}{\matrixstyle{X}_{\bot}}
\newcommand{\bYb}{\matrixstyle{Y}_{\bot}}
\newcommand{\bOneb}{\matrixstyle{1}_{\bot}}


\newcommand{\lambdal}{\underline{\lambda}}
\newcommand{\lambdau}{\overline{\lambda}}
\newcommand{\sigmas}{{\sigma}_s}
\newcommand{\sigmal}{{\sigma}_l}
\newcommand{\sigmat}{\tilde{\sigma}}


\newcommand{\cds}{\textsf{dist}_c}

\newcommand{\leftll}{\left\|}
\newcommand{\rightll}{\right\|}
%\newcommand{\hp}{\odot}
%\newcommand{\ortho}{\textsf{O}}
\newcommand{\QR}{\textsf{QR}}
\newcommand{\SVD}{\textsf{SVD}}
%\newcommand{\rank}{k}
\newcommand{\trace}{\bold{Tr}}
\newcommand{\tr}{\trace}
\newcommand{\diag}{\bold{diag}}
\newcommand{\Tr}{\trace}
\newcommand{\Rad}{\mathfrak{R}}
\newcommand{\OPT}{\mathsf{OPT}}

\newcommand{\AlgRInitial}{\textsf{RandInitial}}
\newcommand{\AlgInitial}{\textsf{SVDInitial}}
\newcommand{\AlgWhitening}{\textsf{Whitening}}
\newcommand{\AlgMain}{\textsf{Alt}}
\newcommand{\AlgClip}{\textsf{Clip}}

\newcommand{\incoherentpartial}{\rho}
\newcommand{\incoherentfull}{\mu}
\newcommand{\valupdate}{\textsf{val}}
\newcommand{\valdelta}{\textsf{c}}

\newcommand{\subs}{\text{SS}}
\newcommand{\subsr}{\text{RSS}}
\newcommand{\subsc}{\text{CSS}}

\newcommand{\tx}{\tilde{x}} % the decoding before threshold
\newcommand{\xp}{{x'}} % the decoding for the shadow sample
\newcommand{\yp}{{y'}} % the shadow sample
\newcommand{\thres}[2]{\phi_{#1}\rbr{#2}} % the threshold
\newcommand{\ntopic}{K}
\newcommand{\nword}{n}
\newcommand{\damp}{R}
\newcommand{\ntdoc}{s} % number of topics in each document
\newcommand{\rbr}[1]{\left(#1\right)} % brackets
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\replace}{\text{Rep}}
\newcommand{\postime}[2]{{#1}^{(#2)}_{+}}
\newcommand{\negtime}[2]{{#1}^{(#2)}_{-}}
\newcommand{\titime}[2]{{#1}^{(#2)}}

\newcommand{\pt}[1]{\postime{#1}{t}}
\newcommand{\nt}[1]{\negtime{#1}{t}}
\newcommand{\ti}[1]{\titime{#1}{t}}

\newcommand{\pto}[1]{\postime{#1}{t+1}}
\newcommand{\nto}[1]{\negtime{#1}{t+1}}
\newcommand{\tio}[1]{\titime{#1}{t+1}}
\newcommand{\sym}[1]{\left\|{#1}\right\|_{\mbox{sym}}}

\newcommand{\xmin}{x_{\textrm{min}}} 
\newcommand{\xexpc}{c_0} 
\newcommand{\corr}{c_1}
\newcommand{\minprob}{c_3}
\newcommand{\eqnref}[1]{(\ref{#1})} 
\newcommand{\sigmac}{C}
\newcommand{\sigmamax}{\Sigma_{\max}}

\newcommand{\AlgDecode}{\textsf{Decode}}

\newcommand{\AlgRen}{\textsf{Renormalization}}
\newcommand{\valupE}{c}
\newcommand{\correlation}{\mathcal{C}}
\newcommand{\corre}{\mathcal{C}}



\DeclareMathOperator*{\prox}{prox}


\usepackage{lineno}
\def\linenumberfont{\normalfont\small}

\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

==> old/old_files/algorithm.tex <==
\section{Regret analysis of randomized policy}
We now assume that our class of policy is restricted only to randomized policy. In other words, we want our bandit algorithm to learn optimum randomized policy given Section \ref{sec:optimal_randomized_policy}. Hence, our aim is to minimze the regret given by 
\begin{equation}
    \regret(t) = \expectation\left(\sum_i \left[\queue_i(t) - \queue^*(t)\right]\right)
\end{equation}
where $\queue_i(t)$ and $\queue_i^*(t)$ are the queue length at server $i$ at time $t$ using the bandit policy and optimal randomized algorithm.

Since, in the beginning the user has no information about the true values of $\mu_i$, the system will have do some exploration to learn the values of $\mu_i$. Every time a job departs from server $i$, the user learns the time taken by the job from server $i$. Since at every time slot,  the departure from a server is decided according to an i.i.d. Bernoulli random variable with parameter $\mu_i$, the service time is distributed according to a geometric random variable. As more and more jobs leave from server $i$, the user can estimate the success probability of server $i$, $\hat{\mu}_i = \frac{n}{\sum_j X_{ij}}$, where $X_{ij}$ is the service time of $j^{th}$ job departing from server $i$.  Define $\hat{\mu}_i(t)$ to be the estimate of $\mu_i$ at time $t$. As, more jobs departs from server $i$, $\hat{\mu}_i(t)$ becomes closer and closer to $\mu_i$, and user have more information about the system. So, in the later stages, the user should exploit the knowledge of the system and explore less often. To maintain a balance between exploration and exploitation, we follow an $\epsilon(t)$ - greedy bandit policy, where at each time $t$, the user decides to explore with probability $\epsilon(t)$ where $\epsilon(t)\rightarrow 0$ as $t\rightarrow \infty$. So, at each time $t$, if the user chooses to explore, it sends any incoming to job to any server at random. However, if the user decides to exploit, it sends the job to server $i$ where $i$ is taken from the multinomial distribution generated by Algorithm \ref{find_support} using the current estimates of $\hat{\mu}_i(t)$'s instead of $\mu_i$.
We provide an Algorithm[\ref{bandit_alg}] and prove that our algorithm achieves $\mathcal{O}\left(\frac{\left(\ln t\right)^{\frac{3}{2}}}{\sqrt{t}}\right)$.
\subsection{Algorithm}
\begin{algorithm}[H]
\caption{Bandit algorithm}
\label{bandit_alg}
\begin{algorithmic}[1]
\While{$t\geq 0$}
\If{\mbox{a job arrives}}
\State $E(t) \sim Ber(\min(1, \frac{K\ln t}{t}))$
\If{$E(t) = 1$}
\State{Choose any server at random}
\Else
\State{Choose $j \sim \mathcal{M}^*\left(\lambda, \hat{\mu}_1(t), \hat{\mu}_2(t), \cdots \hat{\mu}_K(t)\right)$}
\EndIf
\EndIf
\For{$i = 1, 2, \cdots K$}
\If{\mbox{a job departs from server } i}
\State {Update $\hat{\mu}_i(t)$}
\EndIf
\EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}
The main result is given as follows
\begin{theorem}
\label{thm:main}
There exists a $t_0$ such that $\forall t \geq t_0$
\begin{equation*}
    \Psi (t) \leq \sum_{i=1}^{\numofserver} \left[ \frac{192 \ln^2 t}{\epsilon_i^2 t} + k_1 \frac{96\ln t}{\epsilon_i^2}\sqrt{\frac{\ln t}{t}}  + \numofserver\left(\frac{1}{t^{9}} + \frac{9}{t^{6}} + \frac{5k_2 + 1}{t^2} + \frac{4}{t^3} + t^2 \exp\left(-\frac{p_i^*\lambda t}{128}\right)\right) \right],
\end{equation*}
where $k_1, k_2$ is constant.
\end{theorem}
\Gauri{If we use cumulative regret as the metric instead of instantaneous regret, this expression will be a lot cleaner because the higher order terms will all be swallowed by a constant}

\subsection{Analysis}
To analyze the system, we will define a few terminologies. Let $\arrival_i(t)$ and $\departure_i(t)$ denote the indicator random variable of arrival and departure to and from the server  $i$ at time $t$ respectively, $\forall i$. Since, a job can enter the system through either exploration or exploitation, we define $\explore_i(t)$ and $\exploit_i(t)$ as the indicator random variable denoting arrival of job through exploration and exploitation respectively at server $i$ at time $t$. From the definition, clearly
\begin{equation*}
    \arrival_i(t) = \explore_i(t) + \exploit_i(t)
\end{equation*}
holds true for all $i,\>\forall t$.
\Weina{Can we just define $\arrival_i(t)$ and $\departure_i(t)$ to be the number of arrivals and departures instead of indicator random variables?  This way the notation may generalize to non-geometric distributions for interarrival and service times.}
%\Weina{I think $E$ looks too much like expectation and $I$ looks too much like a generic indicator function.  How about we use $\arrival^{(\text{E})}$ and $\arrival^{(\text{I})}$?}
%\Gauri{Good idea! We could even write something like  $\arrival^{(\text{Explore})}$ and $\arrival^{(\text{Exploit})}$ for better clarity.}

For our system, imagine that every server $i$ provides service at time $t$ with probability $\mu_i$ and denies service service with probability $(1-\mu_i),\>\forall t$. At any time $t$, server $i$ sees a departure iff the $\queue_i(t)> 0$ and the server offers a service. Let $\service_i(t)$ denotes the indicator random variable that server $i$ offered service at time $t$. Then from definition,  $S_i(t) \sim Ber( \mu_i)$, and $D_i(t) = S_i(t)$ if $Q_i(t) > 0$ and $D_i(t) = 0$ otherwise.
\begin{equation*}
    \sum_t \departure_i(t) \leq \sum_t\service_i(t).
\end{equation*}
For all the above notations, $(.)^*$ will correspond to system following the optimal policy $\policy^*$. For example $\arrival_i^*(\ell)$ is an indicator random variable showing arrival to server $i$ at time $\ell$ using the optimal policy $\policy^*$.\\\\
Recall, $\support^*$ is defined as the optimal support vector for a system with arrival rate $\lambda$ and departure rate $\mu_i$'s. In other words, 
\begin{equation*}
    i \in \support^* \implies p_i^* \geq 0.
\end{equation*}
Define, $\support^{(t)} = \support\left(\hat{\mu}_1(t), \hat{\mu}_2(t), \cdots\hat{\mu}_\numofserver(t), \lambda\right)$ to be the optimal support vector for the system with arrival rate $\lambda$ and departure rate $\hat{\mu}_i(t)$'s. In other words, the randomized policy might choose server $i$ at time $t$ using the estimates $\hat{\mu}_i(t)$'s iff $\support^{(t)}_i =1$. In the optimal case, when $\hat{\mu}_i(t) = \mu_i$, $\support^{(t)} = \support^*$. Define, $\Delta_{support}$ to be the optimal support set gap for the system . Formally,
\begin{equation}\label{def_optimal_support_set}
    \Delta_{support} = \sup \left\{\delta \geq 0 \>:\>\support\left(\mu_1 - \epsilon_1, \mu_2 - \epsilon_2, \cdots, \mu_K - \epsilon_{\numofserver}, \lambda\right) = \support^*,\>\forall \epsilon_1, \epsilon_2, \cdots, \epsilon_{\numofserver} \mbox{ s.t. } \left|\epsilon_i\right|\leq \delta,\>\forall i\right\}.
\end{equation}
\Gauri{We used $\epsilon_i$ already to denote $\mu_i - \lambda p_i^*$. These $\epsilon$'s are different from that, right?}
This means that if one can learn $\mu_i$'s within a error margin of $\Delta_{support}$, the support vector is same as the optimal support vector. Given $\lambda, \mu_i$'s, it is easy to prove that $\Delta_{support} > 0$, unless there exists an $i$ s.t. $i \in \support^*$ and $p_i^* = 0$. For simplicity, we will consider that $\Delta > 0$. A summary of all the paramters and notations is given in table \ref{tab:parameter_description} and \ref{tab:notation}.
\begin{table}[H]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Parameter} & \textbf{Description} \\ \hline
$\lambda$   &   Arrival rate of jobs    \\ \hline
$\mu_i$     &   Departure rate of jobs from $i^{th}$ server \\ \hline
$\hat{\mu}_i(t)$ & Estimate of $\mu_i$ at time $t$   \\ \hline
$\hat{p}_i(t)$ & Probability of sending job to server $i$ at time $t$ estimated using $\hat{\mu}_1(t), \hat{\mu}_2(t),\cdots \hat{\mu}_\numofserver(t)$   \\ \hline
$p_i^*$       & Probability of sending job to server $i$ according to optimal randomized policy   \\ \hline
$\epsilon_i$       & $\mu_i - \lambda p_i^*$   \\ \hline
$\mu_{min}$       & $\min_{j:\support_j^* = 1} \mu_j$  \\ \hline
$\epsilon_{min}$       & $\min_{j:\support_j^* = 1} \epsilon_j$  \\ \hline
$\mathcal{M}^*\left(\lambda, \mu_1, \mu_2, \cdots, \mu_\numofserver\right)$    &   Optimal multinomial distribution   \\ \hline
$\Delta_{support}$    &   Optimal support vector gap  \\ \hline
\end{tabular}
\caption{Parameter description}
\label{tab:parameter_description}
\end{table}
\begin{table}[H]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Symbol} & \textbf{Description} \\ \hline
$\arrival_i(t)$    &   Indicator random variable showing arrival of job to server $i$ at time t     \\ \hline
$\departure_i(t)$    &   Indicator random variable showing departure of job from server $i$ at time t     \\ \hline
$\service_i(t)$    &   Indicator random variable showing service offered by server $i$ at time     \\ \hline
$\explore_i(t)$    &   Indicator random variable showing arrival of job using exploration to server $i$ at time $t$     \\ \hline
$\exploit_i(t)$    &   Indicator random variable showing arrival of job using exploitation to server $i$ at time $t$   \\ \hline
$Q_i(t)$    &   Number of jobs queued at server $i$ at time $t$     \\ \hline
\end{tabular}
\caption{Variable description}
\label{tab:notation}
\end{table}
Unless specified any normal script is used to denote parameters or variables of the bandit policy and $(.)^*$ is used to define the parameters or variables of the optimal policy

==> old/old_files/analysis.tex <==
%-------------------------------------Section showing all the lemmas---------------------------------------------%
\section{Analysis}
%\Gauri{Unfortunately, all the notations are currently hard-coded -- no macros. It will be very tedious to change them, and I think we will definitely need to change some of the notation...}
%\Tuhin{Did not get which notation you are referring to}
%\Gauri{All the notations in the paper such as $K$, $p$, $A$, $D$, $S$ etc.}
% Lemma to show the convergence of p with the convergence of p
Since, the arrival and departure of jobs in to the system is random, we will couple the system to track difference of queue length at each server $i$. Assume the following coupling between the bandit system $\mathcal{P}$ and optimal system $\mathcal{P}^*$.
\begin{itemize}
    \item \textit{Assignment process} - The assignment process is coupled in a way that minimizes 
    $$\probability\left(\mbox{decision of } \mathcal{P} \neq \mbox{decision of } \mathcal{P}^*\right)$$
    \item \textit{Arrival process}\\
    Job arrives at $\mathcal{P}\iff $ job arrives at $\mathcal{P}^*$.
    \item \textit{Departure process}\\
    Server $i$ in system $\mathcal{P}$ and system $\mathcal{P}^*$ generates a common bernoulli random variable $\service$ with parameter $\mu_i$. If $\service=0$, then there is no departure. If $\service=1$, then server $i$ in system $\policy$ sees a departure, if server $i$ has a job in that system. Similarly, server $i$ in system $\policy^*$ sees a departure, if server $i$ has a job in that system. 
\end{itemize}
Hence, the difference between $\queue_i(t)$ and $\queue_i^*(t)$ ca be written as follows
\begin{align}\label{rel:queue_process}
    \queue_i(t) - \queue_i^*(t) &= \sum_{l = 1}^t\left(\arrival_i(l) - \departure_i(l) - \left(\arrival_i^*(l) - \departure_i^*(l)\right)\right)
\end{align}
If the system is stable, we expect to see a cycle to busy  period and idle period at each server. Now queues at each server resets at the end of each busy period. Define $B_i(t)$ as the length of the current busy cycle period as seen at time $t$, i.e.,
% \Gauri{$B_i(t)$ is not the start of the busy period -- it is the length of the ongoing busy period at time $t$}
\Weina{Google how to correctly write ``i.e.''.}
\begin{equation}
    B_i(t) = \min\left\{s : \queue_i(t - s - 1) =0\right\}
\end{equation}
Since, $\queue_i(t) = 0$ at time $t - B_i(t) - 1$, the difference in queue length at time $t - B_i(t) - 1$ is non-positive. Using this and equation \ref{rel:queue_process} we get
\begin{align}
    \queue_i(t) - \queue_i^*(t) &= \queue_i(t-B_i(t) - 1) - \queue_i^*(t - B_i(t)-1)  + \sum_{\ell = t- B_i(t)}^t\left(\arrival_i(\ell) - \departure_i(\ell) - \left(\arrival_i^*(\ell) - \departure_i^*(\ell)\right)\right)\\
    &\leq   \sum_{\ell = t- B_i(t)}^t\left(\arrival_i(\ell) - \arrival_i^*(\ell)\right)  + \sum_{\ell = t- B_i(t)}^t\left(\departure_i^*(\ell) - \departure_i(\ell)\right)\\
    &\leq \sum_{\ell = t- B_i(t)}^t \indicatorofevents_{ \arrival_i(\ell)\neq \arrival_i^*(\ell)} +  \sum_{\ell = t- B_i(t)}^t \left(\service_i^*(\ell) - \service_i(\ell) \right)\label{label:align_queue_a}\\
    &\leq  \sum_{\ell = t- B_i(t)}^t \left( \indicatorofevents_{ \explore_i(\ell)\neq \explore_i^*(\ell)}\right) + \sum_{\ell = t- B_i(t)}^t \left( \indicatorofevents_{\{ \exploit_i(\ell)\neq \exploit_i^*(\ell)\}}\right)\\
    &\leq  \sum_{\ell = t- B_i(t)}^t \explore_i(\ell) + \sum_{\ell = t- B_i(t)}^t \left( \indicatorofevents_{\{ \exploit_i(\ell)\neq \exploit_i^*(\ell)\}}\right) \label{label:align_queue_b}
\end{align}
\Weina{Use curly brackets for events.  This means all the subscripts of indicators should be inside curly brackets, e.g., $\indicatorofevents_{\{\exploit_i(\ell)\neq \exploit_i^*(\ell)\}}$.}
\Weina{If you want to put superscript $^*$ on quantities to mean that they are corresponding quantities under the optimal policy, you need to explain this notation system explicitly and clearly.}
where, 
\begin{itemize}
    \item Equation \ref{label:align_queue_a} used the fact that since $\queue_i(l) > 0, \forall l \in \left[t-b(t), t\right]$ gives $\departure_i(l) = \service_i(l)$. Also, $\departure_i^*(l) \leq\service_i^*(l)$.
    \item Equation \ref{label:align_queue_b} used the fact that $\explore_i^*(l) = 0$.
\end{itemize}
Hence, taking an expectation would give us, 
\begin{equation}\label{rel:regret_equation}
   \expectation\left[ \queue_i(t) - \queue_i^*(t)\right] &\leq \expectation\left[\sum_{l = t- B_i(t)}^t \explore_i(l)\right] + \expectation\left[\sum_{l = t- B_i(t)}^t  \indicatorofevents_{\{ \exploit_i(l)\neq \exploit_i^*(l)}\}\right]
\end{equation}
% \Gauri{We should simplify the first term further by saying that $\expectation[E_i(l)] = K \ln t / t$ so that it is clear that the first term is proportional to the length of the busy period.}
% \Gauri{Adding a couple of more equations here simplifying the terms will also help untangle the web of lemmas that follow.}
Now, notice that for any $l$, 
\begin{equation}\label{rel_diff_p}
    \expectation\left[\indicatorofevents_{ \{\exploit_i(l) \neq \exploit_i^*(l)\}} \right] = \left|\hat{p}_i(l) - p_i^*\right|,
\end{equation}
\Weina{Unnecessary parentheses around the indicator.}
\Weina{As Gauri pointed out before, this needs to be proved after you introduce the coupling of the assignment processes.}
because of the way we decide the assignment policy. The proof of equation \ref{rel_diff_p} is given in appendix \ref{prf_rel_diff_p} .Also, since $\expectation\left(\explore_i(l)\right) = \frac{\ln l}{l}$. For any $t_1, t_2 \in \left[\frac{t}{2}, t\right]$
\begin{equation}\label{rel_explore}
    \expectation\left[\sum_{l = t_1}^{t_2} \explore_i(l)\right] \leq \frac{1}{2}\left(\ln^2 t_2 - \ln^2 t_1\right) \leq \frac{(t_2 - t_1)\ln t_1}{t_1} \leq \frac{2(t_2 - t_1)\ln t}{t}
\end{equation}
\Weina{Just do this for your specific $t_1$ and $t_2$ in \eqref{rel:regret_equation}.  This is unnecessary generalization.}
\Tuhin{This relation is used more than once. So, I thought it is better to put it in general.}
\Gauri{Why don't we substitute the expression of the RHS of 6.9 into all the equations below? Then we can analyze the two terms in 6.12 separately. The expectation of the exploration term will be proportional to $\expectation[B_i(t)]$, which we can bound in one of the lemmas. And the expectation of the exploitation term will be proportional to the difference between $\hat{p}_i$ and $p_i$, which we can bound in another lemma}
\Tuhin{The term corresponding to exploration is not proportional to $\expectation[B_i(t)]$ unless we have some information about $B_i(t)$. The term corresponding to exploitation is a random sum of random variables. The random variables are not independent how can we separate them? I used $B_i(t) \leq t/2$}
\Gauri{Expectation of a sum of random variables is the sum of the expectations of individual terms, even if they are correlated random variables}
\Tuhin{Okay, I think I can manage that.}
\Gauri{What information about  $B_i(t)$ do you need? Why is it not proportional to $\expectation[B_i(t)]$?}
\Tuhin{Because the $\frac{ln \ell}{\ell}$ term has its minima at $l=t - B_i(t)$.}
\Gauri{Okay, got it}
If we can show that $B_i(t) \leq v_i(t) \leq t/2$ with high probability and $\left|\hat{p}_i(l) - p_i^*\right| \leq g(t),\> \forall l\in [t/2, t]$ for some function $g$, then using equation \ref{rel:regret_equation}, \ref{rel_diff_p} and \ref{rel_explore}, we have 
\begin{align}\label{rel:simplified_final_regret}
    &\expectation\left[ \queue_i(t) - \queue_i^*(t)\right] \\
    \leq &\expectation\left[\sum_{\ell = t- B_i(t)}^t \explore_i(\ell) + \sum_{\ell = t- B_i(t)}^t  \indicatorofevents_{ \exploit_i(\ell)\neq \exploit_i^*(\ell)}\right]\\
    \leq &\expectation\left[\sum_{\ell = t- B_i(t)}^t \explore_i(\ell) + \sum_{\ell = t- B_i(t)}^t  \indicatorofevents_{ \exploit_i(\ell)\neq \exploit_i^*(\ell)}\Big| B_i(t) \leq v_i(t) \leq t/2, \left|\hat{p}_i(\ell) - p_i^*\right| \leq g(t),\forall \ell\in [t/2, t] \right]+\\
    & t\left[\probability\left(B_i(t) \geq v_i(t)\right)+ \probability\left(\left|\hat{p}_i(\ell) - p_i^*\right| \leq g(t),\mbox{ for some } \ell\in [t/2, t]\right)\right]\\
    \leq &\expectation\left[\sum_{\ell = t- v_i(t)}^t \explore_i(\ell) + \sum_{\ell = t- v_i(t)}^t  \indicatorofevents_{ \exploit_i(\ell)\neq \exploit_i^*(\ell)}\Big|  \left|\hat{p}_i(\ell) - p_i^*\right| \leq g(t),\forall \ell\in [t/2, t] \right]+\\
    & t\left[\probability\left(B_i(t) \geq v_i(t)\right)+ \probability\left(\left|\hat{p}_i(\ell) - p_i^*\right| \leq g(t),\mbox{ for some } \ell\in [t/2, t]\right)\right]\\
    \leq &\frac{2v_i(t) \ln t}{t} + v_i(t)g(t) + t\left[\probability\left(B_i(t) \geq v_i(t)\right)+ \probability\left(\left|\hat{p}_i(\ell) - p_i^*\right| \leq g(t),\mbox{ for some } \ell\in [t/2, t]\right)\right]\label{rel:simplified_final_regret}
\end{align}
\Weina{This is incorrect.  $B_i(t)$ is a random variable.  The first term on the right-hand-side should be $\frac{2\expectation[B_i(t)] \ln t}{t}$.  To get this you also need to explain that $\explore_i(\ell)$'s are independent from $B_i(t)$.  For the second term on the right-hand-side, I don't know how to separate $B_i(t)$ out since it is not independent from the $\exploit_i(\ell)$'s.}
% \Gauri{We discussed during the last meeting that the above equation should have a equality}
% \Gauri{Write the above equation in terms of $\exploit_i(l)\neq \exploit_i^*(l)$}
Hence, to bound the queue-regret, we need to bound $2$ quantities with high probability, mainly
% \Gauri{Specify the events and lemmas corresponding to each of the items in the following list}
\begin{enumerate}
    \item Length of the busy period. This is small if 
     \begin{enumerate}
         \item arrival rate of jobs in queues is less than the departure rate - Proved in lemma \ref{lm_p_wt}.
         \item queue length is not too large at some time - Proved in lemma \ref{lm_bound_q_length}, \ref{lm_bound_busy_period_1} and \ref{lm_tighter_queue_length}.
     \end{enumerate}
    \item Number of false exploitations in a busy period - This is small if 
         \begin{enumerate}
             \item the estimate $\hat{p}_i(t)$ is close to $p_i^*$ - Proved in lemma \ref{lm_tight_bound_p}.
             \item To show the convergence of the estimate, we need the number of arrivals to queue $i$ to be linear in time $t$ which is true if arrival rate of jobs into queues is at least some positive constant - Proved in lemma \ref{lm_p_wt}.
         \end{enumerate}
\end{enumerate}
Define 
\begin{equation}\label{eq:t_0}
    t_0 = \inf_\tau \left\{\tau \in \mathbb{R}:\epsilon_{min} w(\tau) \geq 48 \ln \tau, \frac{2}{9} w(\tau) \geq 4 \ln \tau, \frac{32 w(\tau)}{3} \leq \frac{\tau}{4}, \frac{96 \ln \tau}{\epsilon_{min}^2} + \frac{16 \ln \tau}{3 \epsilon_{min}} \leq \frac{\tau}{2} \right\}
\end{equation}
where $w(\tau) = 2\exp\left(\frac{1}{\Delta_0}\sqrt{\frac{16 \ln \tau}{c_g\lambda}}\right)$. \\
To upper bound the number of false exploitations, we need to bound the error in the estimate of $\hat{p}_i(t)$. Lemma \ref{lm_tight_bound_p} provides a bound on  the estimation error of assignment probabilities.
\Weina{Again, use curly brackets for all the events.}
\begin{lemma}
\label{lm_tight_bound_p} 
Define the event $\eventsix$ as
\begin{equation}\label{event6}
    \eventsix := \left| \hat{p}_i(\tau) - p_i^*\right| \leq k_1\sqrt{\frac{ \ln t}{t}},\>\> \forall i, \>\forall \tau \in \left[\frac{t}{2}, t\right]
\end{equation}
for some constant $k_1$. Then,
$$\probability\left(\eventsix^c\right) \leq \numofserver\left(\frac{1}{t^7} + \frac{k_2}{t^3} + \frac{1}{t^3} + t \exp\left(-\frac{p_i^*\lambda t}{128}\right)\right)$$
for any $t \geq t_0$ and $k_1 \geq c\sqrt{\frac{160}{c_g p_{min}^* \lambda}}$.
\end{lemma}
\textit{Proof} - Given is given in Appendix \ref{prf_lm_tight_bound_p}.\\
For the above lemma to hold, we need at least $\mathcal{O}(t)$ number of departure of jobs from each server. For this we want our arrival rate of jobs into each queue to be some positive constant. Lemma \ref{lm_p_wt} will show that the queue $i$ will see arrival rate of some positive constant.  Meanwhile, to upper bound the expected regret, we showed that we need to bound the length of busy cycle as seen at time $t$. Define 
\begin{equation}
    v_i(t) = \frac{96}{\epsilon_{i}^2}\ln t.
\end{equation}
\begin{lemma}
\label{lm_final_busy_period} 
Define the event $\eventfive$ as 
\Weina{Again, use curly brackets for all the events.}
\begin{equation}\label{event5}
    \eventfive := B_i(t) \leq v_i(t).
\end{equation} 
Then,
$$\probability\left(\eventfive^c\right) \leq \numofserver\left(\frac{1}{t^{10}} + \frac{8}{t^{7}} + \frac{4k_2}{t^3} + \frac{4}{t^4}\right)$$
for any $t \geq t_0$.
\end{lemma}
\textit{Proof} - Given is given in Appendix \ref{prf_lm_final_busy_period}.\\
Now, lemma \ref{lm_final_busy_period} proves that that busy period length at time $t$ is upper bounded by $\mathcal{O}\left(\ln t\right)$. Since $\ln t = o\left(t\right)$, we can use the relation \ref{rel:simplified_final_regret} to get the expression of regret. Using the above $2$ lemmas, we can bound the regret of queue length as given in theorem \ref{thm:main}\\
\textit{Proof of Theorem \ref{thm:main}}
\begingroup
    \allowdisplaybreaks
    \begin{align}
        &\expectation\left(\queue_i(t) - {\queue_i^*}(t)\right)\\
        \leq &\expectation\left(\queue_i(t) - {\queue_i^*}(t)\Big | \eventfive, \eventsix\right)  + t\left(\probability\left(\eventfive^c\right) + \probability\left(\eventsix^c\right)\right)\\
        \leq& \expectation\left(\sum_{l = t- B_i(t)}^t \explore_i(l) + \sum_{l = t- B_i(t)}^t \left( \indicatorofevents_{ \exploit_i(l)\neq \exploit_i^*(l)}\right)\Big | \eventfive, \eventsix\right)  + \\
        &\numofserver t\left(\frac{1}{t^{10}} + \frac{9}{t^{7}} + \frac{5k_2 + 1}{t^3} + \frac{4}{t^4} + t \exp\left(-\frac{p_i^*\lambda t}{128}\right)\right) \\
        \leq& \frac{192 \ln^2 t}{\epsilon_i^2 t} + k_1 \frac{96\ln t}{\epsilon_i^2}\sqrt{\frac{\ln t}{t}}  + \numofserver\left(\frac{1}{t^{9}} + \frac{9}{t^{6}} + \frac{5k_2 + 1}{t^2} + \frac{4}{t^3} + t^2 \exp\left(-\frac{p_i^*\lambda t}{128}\right)\right)\label{calc:regret_simplification}
    \end{align}
    \endgroup
where the equation \ref{calc:regret_simplification} follows from equation \ref{rel:simplified_final_regret}.\\\\
Now, the main idea to prove the lemma \ref{lm_final_busy_period} is to argue that queue length is bounded by some function of $t$ and departure rate exceeds the arrival rate by a fixed constant. This results in a negative drift, which forces the length of the busy period to be bounded. Lemma \ref{lm_tighter_queue_length} ensures that the queue length is upper bounded by some function of $t$. Define the term $\queue_{0i}$ as
\begin{equation}
    \queue_{0i} = \left(5 + \frac{16}{\epsilon_i}\right)\ln t + \frac{32 w(t)\ln t}{3t}.
\end{equation}
\Weina{Change to a lower-case letter.  It is a good practice to use upper-case letters for random variables and lower-case letters for non-random variables.  You can have exceptions for indexing integers like $K$, $N$, etc.}
Observe that 
\begin{equation}
    \queue_{0i} \leq \frac{32 \ln t}{\epsilon}.
\end{equation}
\Weina{I suggest that we eliminate the definitions of many of the events and write them out directly.  The number of indexed events is just too large.  It is impossible to memorize the events.  If we do not need to do complicated unions or intersections, we do not need to give the event a symbol.  For example, the following lemma can be rewritten as follows.
\begin{lemma}
For any $t\ge t_0$ with $t_0$ defined in \eqref{eq:t_0}, it holds that
\begin{equation}
\probability\left(Q_i(t - v_i(t)) > \queue_{0i}\right)\leq \numofserver\left(\frac{6}{t^{7}} + \frac{3k_2}{t^3} + \frac{4}{t^4}\right).
\end{equation}
\end{lemma}
Later when you need to use the event $\eventfour$, just write out $Q_i(t - v_i(t)) > \queue_{0i}$.
This is just an example and I think we should do this also for at least $\eventfive$, $\eventthree$, $\eventtwo$.  You need to think carefully about which ones to keep and keep as few as possible.}
\begin{lemma}
\label{lm_tighter_queue_length} 
\Weina{Again, use curly brackets for all the events.}
Define the event $\eventfour$ as 
\begin{equation}\label{event4}
    \eventfour := Q_i(t - v_i(t)) \leq \queue_{0i}.
\end{equation}
Then,
$$\probability\left(\eventfour^c\right) \leq \numofserver\left(\frac{6}{t^{7}} + \frac{3k_2}{t^3} + \frac{4}{t^4}\right)$$
for any $t \geq t_0$.
\end{lemma}
\textit{Proof} - Given is given in Appendix \ref{prf_lm_tighter_queue_length}.\\
Notice that to prove that busy period length is bounded, we used a combination of bounded queue length and negative drift in the queue length process. To prove lemma \ref{lm_tighter_queue_length}, we will use the reverse argument that the busy period is bounded and there is a negative drift in the queue length process. Lemma \ref{lm_bound_busy_period_1} proves that the busy period length seen at time $(t - v_i(t))$ is bounded. 
\begin{lemma}
\label{lm_bound_busy_period_1}
Define the event $\eventthree$ as 
\begin{equation}\label{event3}
    \eventthree := B_i(t - v_i(t)) \leq \frac{16}{3\epsilon_{i}}w(t),
\end{equation}
for all $i$. Then,
$$\probability\left(\eventthree^c\right) \leq \numofserver\left(\frac{4}{t^{7}} + \frac{2k_2}{t^3} + \frac{2}{t^4}\right)$$
for any $t \geq t_0$.
\end{lemma}
\textit{Proof} - Given is given in Appendix \ref{prf_lm_bound_busy_period_1}.\\
And similar to previous argument to prove lemma \ref{lm_bound_busy_period_1}, we will prove that the queue length is bounded and there is a negative drift. Lemma \ref{lm_queue_upper} proves the weaker bound on the queue length seen at any time. 
\Weina{Is $\eventtwo$ the intersection $\cap_{\tau=1}^t\{\queue_i(\tau)\leq 2w(t)\}$ or just $\{\queue_i(\tau)\leq 2w(t)\}$?}
\Tuhin{Intersection one.}
\begin{lemma}\label{lm_queue_upper}
\label{lm_bound_q_length}
Define the event $\eventtwo$ as 
\begin{equation}\label{event2}
    \eventtwo := \queue_i(\tau)\leq 2w(t),\>\> \forall \tau \in [1,t]
\end{equation}
then
$$\probability\left(\eventtwo^c\right) \leq \numofserver\left( \frac{1}{t^4} + \frac{2}{t^{7}} + \frac{k_2}{t^3}\right)$$
for any $t \geq t_0, \forall i.$
\end{lemma}
\textit{Proof} - Given is given in Appendix \ref{prf_lm_bound_q_length}.\\
To prove all the lemmas, we needed that there is a negative drift in the queue length process and arrival rate of jobs into each queue is at least positive constant. Lemma \ref{lm_p_wt} proves that all these conditions are satisfied after time $w(t)$ with high probability.
\begin{lemma}
\label{lm_p_wt}
Define the event $\eventone$ as 
\begin{equation}\label{event1}
    \eventone := \mathcal{E}_{11} \cap \mathcal{E}_{12}\cap\mathcal{E}_{13}
\end{equation} where
\begin{enumerate}
    \item $\mathcal{E}_{11}:=\support^{(\tau)} = \support^*,\>\>\forall \tau \in \left[w(t), t\right]$
    \item $\mathcal{E}_{12}:=\frac{p_i^*}{2} \leq \hat{p}_i(\tau)\leq \frac{3p_i^*}{2},\>\>\forall i,\forall \tau \in \left[w(t)), t\right]$
    \item $\mathcal{E}_{13}:= 
            \expectation\left(\arrival_i(\tau)\right) \leq \mu_i - \frac{\epsilon_i}{2},\>\>\forall i,\forall \tau \in \left[w(t)), t\right]$.
\end{enumerate}
where, $\Delta_0 = \min\left\{\Delta, t_g, \frac{p_{min}}{2c}, \sqrt{\frac{\epsilon_{min}}{3}}\right\}$. Then, $\forall t\geq t_0$ $$\probability\left(\eventone^c\right)\leq \numofserver\left(\frac{2}{t^{7}} + \frac{k_2}{t^3}\right)$$
where $k_2 = \frac{1}{1 - \exp\left( -c_g\Delta_0^2 \right)}$
\end{lemma}
\textit{Proof} - Given is given in Appendix \ref{prf_lm_p_wt}.\\
From the service times of the departed jobs, the system can learn the $\mu_i$'s. Since $\expectation\left(\hat{\mu}_i(t)\right) \neq \mu_i$ and geometric random variable is unbounded, standard hoeffding bounds cannot be used to bound the estimation error. Lemma \ref{lm_conc_geoemtric} provides a relation to bound the error in the estimate $\hat{\mu}_i(t)$. However, the ultimate goal of the system is to learn $p_i^*$. Since $\hat{p}_i(t)$ is a function of $\hat{\mu}_i(t)$, we want a relation between the estimation error of $\mu_i$ and $p_i^*$ for all $i$. Lemma \ref{lm_relation_p_mu} provides a relation between the estimation error of $\mu_i$ and $p_i^*$ for all $i$. 
\begin{lemma}
\label{lm_conc_geoemtric}
For any sequence of i.i.d. geometric random variable $X_1, X_2, X_3, \cdots, X_n$ with success probability $\mu$, $\exists c_g, t_g \geq 0$ such that 
$$\probability\left(\left|\frac{n}{\sum_i X_i} - \mu\right| \geq x\right) \leq \exp\left(-n c_g x^2\right),\>\> \forall x\in [0, t_g],$$
where $c_g = \min\left\{\frac{1}{16\mu^2(1-\mu)}, \frac{c_{g_-}}{4\mu^4}, 1 \right\}, t_g=\min\left\{\frac{\mu(1-\mu)}{2}, 2\mu^2t_{g_-}, \mu \right\}, c_{g_-} = \frac{\mu^2}{4(1-\mu)}$, 
\begin{equation*}
    t_{g_-} = \sup \left\{x:\left( \ln \left(1-\frac{\mu x}{1-\mu}\right)- \left(\frac{1}{\mu} - x\right)\ln \left(1 - \frac{\mu^2x}{(1-\mu)(1-\mu x)}\right) + c_{g_-}x^2\right) \leq 0\right\}.
\end{equation*}
\end{lemma}
\textit{Proof} - Given in Appendix \ref{prf_lm_conc_geoemtric}.
\begin{lemma}
\label{lm_relation_p_mu}
\Gauri{What is the index of $\hat{\mu}_i$ and $\hat{p}_i$ here? Is it $t$ or $n$?}
\Tuhin{Does not matter. It is true for any estimate. Changed the lemma though}
\Gauri{I know it does not matter for the result :). But to be consistent you shouldn't drop indices like that!}
For all $\delta \in (0, \Delta)$ and for any estimate $\hat{\mu}_i$ of $\mu_i$, if $\> \lvert\hat{\mu}_i - \mu_i\rvert \leq \delta$ for all $i$, then
\begin{equation}
    \lvert\hat{p}_i - p_i^*\rvert \leq \min \left\{c\delta, \frac{\epsilon^*}{2\lambda}\right\}
\end{equation}
for all $i$, where $\hat{p}_i$'s are the probability values corresponding to the distribution $\mathcal{M}^*\left(\lambda, \hat{\mu}_1, \cdots, \hat{\mu}_\numofserver \right)$, $c\geq 1$ is some positive constant and $\Delta = \min \left\{\frac{\tilde{\mu}}{2}, \frac{\epsilon_{min}}{||\support^*||_1}, \frac{\epsilon_{min}}{2c\lambda}, \Delta_{support}\right\}, \tilde{\mu} = \min_i \{\min \{\mu_i, 1- \mu_i\}\}$.
\end{lemma}
\textit{Proof} - Given is given in Appendix \ref{prf_lm_relation_p_mu}.
% Now, we proved that arrival rate of jobs in to each queue is at-least some positive constant after $w(t)\>\forall t\geq t_0$, we in turn want to argue that with high  probability, the estimates $\hat{p}_i(t)$ becomes closer and closer to $p_i$. Lemma \ref{lm_tight_bound_p} proves a tighter bound on the estimate $\hat{p}_(t)$.
% Now, we have to prove that with high probability the length of the busy period cycle at time $t$ is upper bound by some number with high probability. Now, to argue that the busy period is bounded, it is sufficient to argue that the queue length is bounded and the queues are stable. This is because bounded stable queues will become zero within a bounded interval of time with high probability. We will use a $2$- step method to bound the length of the busy period. We will first prove in Lemma \ref{lm_bound_q_length} that the queue length at server $i$ is bounded. In lemma \ref{lm_bound_busy_period_1}, we will use the bounded queue length to prove that the busy period is also bounded.
% Now that we have tight  bounded on the length of the busy period, we can repeat the above steps to get a even tighter bound on the length of the busy period. Lemma \ref{lm_tighter_queue_length} uses the bound on busy period to derive a tighter bound on the queue length. Lemma \ref{lm_final_busy_period} uses the tighter bound of queue length to get an even tighter bound on busy period.

==> old/old_files/intro.tex <==
\section{Introduction} \label{sec intro}
\Gauri{Please fix the compilation errors}
\Weina{I second Gauri here.  Can you look at the ``logs and output files'' button on the right of the recompile button and fix the errors in it?}
Multi-arm bandit and Queueing theory have been one of the most extensively researched areas over the last century. The traditional queueing problem studied the relation of system metrics like response time and expected queue length concerning server speed and job arrival rate. Change in the metrics is also studied w.r.t scheduling of jobs. However, in most of the settings, people assumed that they have full knowledge about the system i.e. service time and job arrival rate are known. These assumptions simplify the system by a great extent. However, in real life, it is difficult to know the parameters beforehand. The problem studied in this paper is an example of such a case. 
% \Weina{Do not use line break at the end of a paragraph.}

We considered the scenario where jobs arrive at a system consisting of multiple servers. There is a queue assigned to each server. Jobs are serviced at its designated server with service time sampled randomly from a distribution with unknown mean. Jobs are stored in the queue until the server services it. We are interested in finding an efficient algorithm for which the expected queue length is minimized. This problem is like a typical MAB problem. 

A traditional MAB problem consists of $k$-arms. Arm $i$, when pulled give reward randomly sampled from a random variable with mean $\mu_i$. The problem is to identify the arm with the highest expected reward. Under this setting, many algorithms have been derived to determine the best-arm. \cite{jamieson2014lil} proposes a lil' UCB algorithm to identify the best arm. Another version of the problem is regret minimization. Regret is the difference between reward received from the algorithm and reward received if one only pulls the optimal arm.\cite{garivier2011kl}, \cite{auer2002finite}, \cite{agrawal2012analysis} gives some algorithm to minimize the regret over finite or infinite time-horizons. The problem that we are studying is a direct map to the MAB problem with regret minimization where regret corresponds to mean response time of the system. A similar setup  was studied in \cite{krishnasamy2016learning}; however, they assumed a single queue multi-server model, unlike the multi-queue multi-server model,  where multiple servers can remain active at a particular+ instance.

==> old/old_files/old_algorithm.tex <==
\section{Pure exploitation is sub-optimal}
\Gauri{Alternate title for this section: The Necessity of Exploration}
With policy $\policy^*$ defined, we want to design a policy $\policy$ that minimizes the expected regret $\mathbb{E}\left[\regret_{\policy \policy^*}(t)\right]$. The main idea behind policy $\policy$ is to use a routing vector that converges to the optimal routing vector as time progresses.  Every time a job departs, the policy $\policy$ has information about the service time of the job. Using this information, the policy can estimate the service rate vector, which further can be used to estimate the optimal routing vector. Let $N_i(t)$ be the number of jobs that departed from server $i$ till time $t$. Let $X_1, X_2, \cdots, X_{N_i(t)}$ be the service time of the $N_i(t)$ jobs respectively. Define $\hat{\bm{\mu}}(t) = \left(\hat{\mu}_1(t), \hat{\mu}_2(t), \cdots, \hat{\mu}_\numofserver(t)\right)$ to be the estimated service rate vector at time $t$, where $\hat{\mu}_i(t)$  is given by 
\begin{equation}
    \hat{\mu}_i(t) = \frac{N_i(t)}{\sum_{j=1}^{N_i(t)} X_j},
\end{equation}

Now, a naive algorithm could use the estimate $\hat{\bm{\mu}}(t)$ at every time to estimate the routing vector and assign the job to different servers accordingly. However, this might lead to a situation where an optimal server is not included in the support vector because of bad estimation. The best way to get over this issue is to force \textit{exploration} of the servers, where the policy ensures that it has sufficient samples of service time from each server before rejecting it. One way to do this is given as follows:
\begin{enumerate}
    \item Fix a a number $n$.
    \item Send the first $n$ jobs to any server uniformly at random.
    \item For the remaining jobs, use the estimate $\hat{\bm{\mu}}(t)$ to calculate the routing vector and correspondingly assign the job.
\end{enumerate}

However, this type of algorithm is also not enough to ensure that the policy achieves a sub-linear regret w.r.t. time. Consider the example given below that illustrates the issue of this type of algorithm. 

Consider a two server system. $\lambda = 0.05, \bm{\mu} = \left(0.5, 0.5\right)$. The optimal routing vector is given by $\left(0.5, 0.5\right)$. Assume $k$ jobs out of the first $n$ jobs are sent to server $1$. If the estimate of the service rate is $(\hat{\mu}_1, \hat{\mu}_2)$, where $\hat{\mu}_1 \leq 0.1$ and $\hat{\mu}_2\geq 0.2$, then the routing vector is given by $(0, 1)$. Let $\mathcal{E}$ be event where the estimate $\hat{\mu}_2(t) \geq 0.2$ for all time $t$ and the estimate $\hat{\mu}_1(t) \leq 0.1$, till all the first $k$ job has departed. Then event $\mathcal{E}$ implies that for rest of the time no job would be sent to first server at all. The above situation would then lead regret to scale linearly with time. Now 
    % \Weina{The hat symbol should only be over $\mu$}
    \begin{align}
        \probability(\mathcal{E}) &\geq \left(\sum_{k = 1}^n {n \choose k}(0.5)^n \left((0.5)^{10}\right)^k\right) \probability\left(\cap_{t = 1}^{\infty}\left\{\hat{\mu}_2(t) \geq 0.2\right\}\right)\\
        &\geq \left(1 -  \sum_{t = 1}^{\infty}\probability\left(\hat{\mu}_2(t) < 0.2\right)\right) \sum_{k = 1}^n {n \choose k}(0.5)^n \left((0.5)^{10}\right)^k\\
        &\geq \frac{1}{3} \sum_{k = 1}^n {n \choose k}(0.5)^n \left((0.5)^{10}\right)^k> 0
    \end{align}
Notice that if event $\mathcal{E}$ is true, then algorithm would use only server $2$ in the long run. Now, the steady state queue length, when using only server $2$ is $1/18$, while the steady state queue length using the optimal routing vector is $1/19$. Thus the regret would scale roughly as $t/342$. Hence with some finite probability $\probability(\mathcal{E})>0$, any policy of this kind would also give a linear regret.
    % \Weina{Can you give a short, clear argument on why this gives a linear regret?}
\section{Algorithm}
% \Gauri{Shall we add a section called 'Pure Exploitation Policies Cannot Achieve Sublinear Regret'}


Exploring for a fixed amount of time leads to a linear regret. Hence, one would like never to stop exploration, but reduce the amount of exploration over time. This is to ensure that one does not overdo exploration, which would also lead to a higher regret. One way to do this is to use the $\mathcal{E}(t)$-greedy exploration strategy, which decides to explore at time $t$ with probability $\mathcal{E}(t)$. $\mathcal{E}(t)$ is chosen in a way such that the exploration probability goes to zero as $t$ goes to infinity. Based on the above idea, we propose an algorithm given in \Cref{algo:bandit}.


% We now assume that our class of policy is restricted only to randomized policy. In other words, we want our bandit algorithm to learn optimum randomized policy given in Section \ref{sec:optimal_randomized_policy}. Hence, our aim is to minimize the regret given by 
% \begin{equation}
%     \regret(t) = \expectation\left(\sum_i \left[\queue_i(t) - \queue^*(t)\right]\right)
% \end{equation}
% where $\queue_i(t)$ and $\queue_i^*(t)$ are the queue length at server $i$ at time $t$ using the bandit policy and optimal randomized algorithm.

% Since, in the beginning the user has no information about the true values of $\mu_i$, the system will have do some exploration to learn the values of $\mu_i$. Every time a job departs from server $i$, the user learns the time taken by the job from server $i$. Since at every time slot,  the departure from a server is decided according to an i.i.d. Bernoulli random variable with parameter $\mu_i$, the service time is distributed according to a geometric random variable. As more and more jobs leave from server $i$, the user can estimate the success probability of server $i$, $\hat{\mu}_i = \frac{n}{\sum_j X_{ij}}$, where $X_{ij}$ is the service time of $j^{th}$ job departing from server $i$.  Define $\hat{\mu}_i(t)$ to be the estimate of $\mu_i$ at time $t$. As, more jobs departs from server $i$, $\hat{\mu}_i(t)$ becomes closer and closer to $\mu_i$, and user have more information about the system. So, in the later stages, the user should exploit the knowledge of the system and explore less often. To maintain a balance between exploration and exploitation, we follow an $\epsilon(t)$ - greedy bandit policy, where at each time $t$, the user decides to explore with probability $\epsilon(t)$ where $\epsilon(t)\rightarrow 0$ as $t\rightarrow \infty$. So, at each time $t$, if the user chooses to explore, it sends any incoming to job to any server at random. However, if the user decides to exploit, it sends the job to server $i$ using the optimal  randomized allocation using the estimates.
% We propose \Cref{algo:bandit} and prove that our algorithm achieves $\order\left(\frac{\left(\ln t\right)^{\frac{3}{2}}}{\sqrt{t}}\right)$.
\begin{algorithm}[H]
\caption{Bandit algorithm}
\label{algo:bandit}
\begin{algorithmic}[1]
\While{$t\geq 0$}
\If{\mbox{a job arrives}}
\State $\explorerandom(t) \sim Ber(\min(1, \frac{K\ln t}{t}))$
\If{$\explorerandom(t) = 1$}
\State{Send to one of the $K$ servers uniformly at random}
\Else
\State{Send to server $i$ with probability  $\hat{p}_i(t)$ where $\hat{p}_i(t)$'s are  optimal probabilities calculated using \eqref{optimal_p} with parameters $\lambda$ and $\hat{\mu}_i(t)$'s}
%\Gauri{Remove $M^*$ from here}
%\Tuhin{Though I removed it, the current algorithm looks stranger. It might be better to define the optimal categorical distribution $\mathcal{M}^*$ for any given $\lambda$ and $\boldsymbol{\mu}$. Let me know what you think!}
\EndIf
\EndIf
\For{$i = 1, 2, \cdots K$}
\If{\mbox{a job departs from server } i}
\State {Update $\hat{\mu}_i(t)$}
\EndIf
\EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}

==> old/old_files/old_analyzing_queue_length.tex <==
\subsection{Analyzing queue length difference}
Note that the difference between $\queue_i(t)$ and $\queue_i^*(t)$ at any time $t$ can be written as follows with any $\tau\le t$:
\begin{align*}%\label{rel:queue_process}
    \queue_i(t) - \queue_i^*(t) &= \queue_i(\tau) - \queue_i^*(\tau)\\
    &\mspace{21mu}+\sum_{\ell = \tau}^{t-1}\left(\arrival_i(\ell) - \departure_i(\ell) - \left(\arrival_i^*(\ell) - \departure_i^*(\ell)\right)\right).
\end{align*}
\Weina{Should the upper limit of the sum be $t-1$ instead of $t$?}
\Weinarevise{Below we will consider a specific $\tau$ that is the last time queue $i$ is empty. Specifically,}
\sout{If the system is stable, one expects to see a cycle of busy  period and idle period at each server. Now the queues at each server resets at the end of each busy period.} define $\busy_i(t)$ as the length of the current busy cycle period as seen at time $t$, i.e.,
% \Gauri{$\busy_i(t)$ is not the start of the busy period -- it is the length of the ongoing busy period at time $t$}
% \Weina{Google how to correctly write ``i.e.''.}
\begin{equation}
    \busy_i(t) = \min\left\{s\ge 0 : \queue_i(t - s) =0\right\}.
\end{equation}
\Weinarevise{Then note that for $\tau = t-\busy_i(t)$, we have $\queue_i(\tau)=0$.}
\Cref{clm:regret_equation}, given below, gives an upper bound on the difference of the queue lengths at any time $t$ based on this recursion.
%\Weina{I added $\ge 0$}
\begin{clm}\label{clm:regret_equation}
\begin{equation}
    \begin{split}
        \queue_i(t) - \queue_i^*(t) \leq  \sum_{\ell = t- \busy_i(t)}^{t-1} \explore_i(\ell) + \\
        \sum_{\ell = t- \busy_i(t)}^{t-1} \indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}}.
    \end{split}
\end{equation}
\end{clm}
\begin{proof}
    \begingroup
    \allowdisplaybreaks
    \begin{align}
        &\queue_i(t) - \queue_i^*(t) \\
        = &\queue_i(t-\busy_i(t)) - \queue_i^*(t - \busy_i(t))\nonumber  \\
        & \qquad + \sum_{\ell = t- \busy_i(t)}^{t-1}\left(\arrival_i(\ell) - \departure_i(\ell) - \left(\arrival_i^*(\ell) - \departure_i^*(\ell)\right)\right)\\
        \leq &\sum_{\ell = t- \busy_i(t)}^{t-1}\left(\arrival_i(\ell) - \arrival_i^*(\ell)\right)  + \sum_{\ell = t- \busy_i(t)}^{t-1}\left(\departure_i^*(\ell) - \departure_i(\ell)\right)\\
        \leq &\sum_{\ell = t- \busy_i(t)}^{t-1} \left(\explore_i(\ell) + \exploit_i(\ell) - \arrival_i^*(\ell)\right)  \nonumber\\
        & \qquad + \sum_{\ell = t- \busy_i(t)}^{t-1} \left(\service_i^*(\ell) - \service_i(\ell) \right)\label{label:align_queue_a}\\
        = &\sum_{\ell = t- \busy_i(t)}^{t-1} \explore_i(\ell) + \sum_{\ell = t- \busy_i(t)}^{t-1} \left(\exploit_i(\ell) - \arrival_i^*(\ell)\right)\label{label:align_queue_b}\\
        &\leq \sum_{\ell = t- \busy_i(t)}^{t-1} \explore_i(\ell) + \sum_{\ell = t- \busy_i(t)}^{t-1} \indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}}.\label{rel:regret_equation}
    \end{align}
    \endgroup
    where, 
    \begin{enumerate}
        \item \eqref{label:align_queue_a} used the fact that \Weinarevise{for all $\ell \in \left[t-\busy_i(t), t-1\right]$, $\departure_i(\ell) = \service_i(\ell)$ since $\queue_i(\ell) > 0$}\sout{since $\queue_i(\ell) > 0, \forall \ell \in \left[t-b(t), t\right]$, $\departure_i(\ell) = \service_i(\ell)$.} and $\departure_i^*(\ell) \leq\service_i^*(\ell)$.
        \item \eqref{label:align_queue_b} uses the fact that \sout{service process is coupled}\Weinarevise{$\service_i^*(\ell) = \service_i(\ell)$ for all $i$ and all $\ell$ by our construction of the coupling}. %\Gauri{In 6.23 we should have an equality because $S^* = S$?}
       % \Tuhin{Done}
    \end{enumerate}
\end{proof}
%\Gauri{Proof of which theorem? Add to number in the title}
%\Tuhin{Done}
The regret  is cumulative difference in the queue lengths of different servers in the two systems. Hence, expected regret can be upper bounded by taking an expectation over the equation given in \Cref{clm:regret_equation} and summing it over all servers. But directly taking an expectation to calculate the expected regret will be difficult to analyze since $\busy_i(t)$ is a random variable which is depends of past arrivals. However, if $\busy_i(t)$ is bounded, then the first term $\left(\sum_{\ell = t- \busy_i(t)}^{t-1} \explore_i(\ell)\right)$ can be easily upper bounded, since $\expectation\left[\explore_i(\ell)\right]$ is known for all time $\ell$.
% \begin{align}\label{rel:regret_equation}
%   \expectation\left[ \queue_i(t) - \queue_i^*(t)\right] &\leq \expectation\left[\sum_{\ell = t- \busy_i(t)}^t \explore_i(\ell)\right] + \expectation\left[\sum_{\ell = t- \busy_i(t)}^t \indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}}\right].
% \end{align}
% \Gauri{We should simplify the first term further by saying that $\expectation[E_i(l)] = K \ln t / t$ so that it is clear that the first term is proportional to the length of the busy period.}
% \Gauri{Adding a couple of more equations here simplifying the terms will also help untangle the web of lemmas that follow.}
%\Gauri{The above result should be a lemma or claim in the coupling section. No need to repeat it here (it breaks the flow of the difference in queue length analysis that you are doing here), just refer to that lemma when you need it. Also, you don't seem to be using it until much later (6.38), so may be talk about it after the align block containing that equation}
%\Gauri{The above equation should be less than equal to}
%\Tuhin{Corrected.}
% \Weina{Unnecessary parentheses around the indicator.}
% \Weina{As Gauri pointed out before, this needs to be proved after you introduce the coupling of the assignment processes.}
% Also, for any $t_1, t_2 \in \left[\frac{t}{2}, t\right]$
% \begin{equation}\label{rel:explore}
%     \expectation\left[\sum_{\ell = t_1}^{t_2} \explore_i(\ell)\right] \leq \frac{1}{2}\left(\ln^2 t_2 - \ln^2 t_1\right) \leq \frac{(t_2 - t_1)\ln t_1}{t_1} \leq \frac{2(t_2 - t_1)\ln t}{t}.
% \end{equation}
%\Gauri{It is unnecessary to write this for a general $t_1$ and $t_2$. Continue the same align block as 6.24 until here to avoid having readers navigate through a mess of scattered equations}
%\Tuhin{I used it twice, hence thought of writing it in general}
%\Gauri{Even if it is used twice, I think it is okay to write it for specific $t_1$ and $t_2$}
%\Gauri{The following statement does not make sense. I suggest deleting it} Notice that if $\busy_i(t)$ is not a random variable, then the term corresponding to exploration is a sum of random variables.
Consider, the event $\eventfive$ given by, 
\begin{equation}
 \label{eqn:event5}
    \eventfive := \left\{\busy_i(t) \leq v_i(t) \triangleq \frac{66\ln t}{\freecapacity_{i}^2},\> \forall i\right\},
\end{equation}
\Weina{We cannot number the first event we consider as event 5.  It needs to be event 1}
where, $\freecapacity_i$ is the residual capacity of server $i$ given by $\freecapacity_i = \mu_i - \lambda p_i^*$. We will prove in \Cref{lem:final_busy_period} that $\eventfive$ is a very likely event and use it further to simplify the \eqref{rel:regret_equation}. 

Now, $\exploit_i(\ell)$ depends on $\hat{p}_i(\ell)$, while $\exploit_i(\ell)$ depends on $p_i^*$. As the estimates $\hat{\bm{\mu}}(t)$ converges to $\bm{\mu}$, the $\hat{\bm{p}}(t)$ will converge to $\bm{p}^*$. Therefore, the second expression which depends on the difference of $\exploit_i(\ell)$ and $\arrival_i^*(\ell)$ can be bound by the difference of $\hat{p}_i(\ell)$ and $p_i^*$. To simplify the second expression in \eqref{rel:regret_equation}, one can use \Cref{clm:regret_equation} to express it as error in the estimation of $p_i^*$. Consider another event $\eventsix$, defined as
\begin{equation}\label{eqn:event6}
    \eventsix := \left\{\left| \hat{p}_i(\tau) - p_i^*\right| \leq k_1\min\left\{\sqrt{\frac{ \ln t}{t}}, p_i^*\right\},\>\> \forall i , \>\forall \tau \in \left[\frac{t}{2}, t\right]\right\}
\end{equation}
where, $k_1$ is a large enough constant specified as follows: $k_1 \geq c\sqrt{\frac{160}{c_g p_{min}^* \lambda}}$ with 
\begin{equation}
    c_g = \min\left\{\min_i\left\{\frac{1}{3(1 - \mu_i)(3 - \mu_i)}\right\}, \frac{1}{8}\right\},
\end{equation}
$c\geq 1$ is a function of $\lambda, \boldsymbol{
\mu}$ and $p_{\min} = \min_{i: p_i^* > 0}p_i$. Similar to $\eventfive$, we will prove in \Cref{lem:tight_bound_p} that $\eventsix$ is a very likely event and use it to simplify the \eqref{rel:regret_equation}. Define $\regret_{\policy \policy^*}^{inst}(t)$ as the instantaneous regret, given by 
\begin{equation}
    \regret_{\policy \policy^*}^{inst}(t) = \sum_{i = 1}^{\numofserver}\left(\queue_i(t) - \queue_i^*(t)\right).
\end{equation}
%\Weina{I revised the wording slightly.}
% \Gauri{When you define an event there can't be a bunch of constants that are undefined. This implies that the definition of $\eventsix$ is incomplete}
%\Tuhin{Changed} \Gauri{The above statement does not make sense at this place in the paper because you are using it much later. State it where you use it}
%\Tuhin{Okay}

Hence, using $\eventfive, \eventsix$ and \Cref{clm:regret_equation}, we have %\Gauri{This statement about $t'$ is also not at the right place. You don't need $t > t'$ until the later part of the following derivation}
%\Tuhin{I deleted it. But is it okay to introduce conditions later in the proofs without introducing them first. I feel that since we are writing all the steps with any break in between, all the conditions should be applied right from the start.}
%\Tuhin{I think this issue is now solved, so we can comment out the commnet.}
%\Gauri{Also, is $t'$ the same as $t_0$? Where is $t'$ defined? Instead of saying there exists some $t'$, we should specify what $t'$ is -- does it scale linearly with $t$ or logarithmically with $t$? The readers will get confused about that}
%\Tuhin{It is not exactly same. $t_0$ satisfies the conditions of $t'$, but it has to satisfy some additional constraints. Also, $t'$ does not scale with $t$. $t' = \inf_{\tau} \left\{\tau:v_i(\tau) \leq \tau/2\right\}$. It is just a constant which depends on system parameters.}
%\Gauri{Would it be okay to just retain $t_0$, since it places stricter conditions than $t'$, and say that the results hold for $t > t_0$? Even if it is less general, it might be more clear to present.}
%\Tuhin{Consider line 43-49 as an alternate line of proof, which resembles more of Sanjay's paper. 42 and then 50-55 was the original proof I considered.}
\Gauri{Write $\sum_{i=1}^{K}$ everywhere instead of $\sum_i$}
\begingroup
\allowdisplaybreaks
\begin{align}
    &\expectation\left[\regret_{\policy \policy^*}^{inst}(t)\right] \\
    =& \sum_i\expectation\left[\queue_i(t) - \queue_i^*(t)\right] \\
    \leq &\sum_i\expectation\left[ \left(\queue_i(t) - \queue_i^*(t)\right)\indicatorofevents\left\{\eventfive\right\} + \left(\queue_i(t) - \queue_i^*(t)\indicatorofevents\left\{
    \eventfive^c\right\}\right)\right] \\
    \leq &\sum_i\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[  \explore_i(\ell) +  \indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}}\right]\nonumber\\
    & \qquad + t\probability\left(\eventfive^c\right)\label{rel:simplified_regret:use_regret_equation}\\
    = & \sum_i\sum_{\ell = t- v_i(t)}^{t-1}\probability\left( \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right) + \nonumber\\
    & \qquad + \sum_i\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\explore_i(\ell)\right] + t\probability\left(\eventfive^c\right)\\
    = & \sum_i\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\probability\left( \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\Big| \hat{p}_i(\ell)\right)\right]   \nonumber\\
    & \qquad + \sum_i\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\explore_i(\ell)\right] + t \probability\left(\eventfive^c\right)\\
    \leq & \sum_i\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\explore_i(\ell)\right]    + \sum_i\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\left| \hat{p}_i(\ell) - p_i^*\right|\right] \nonumber\\
    & \qquad + t \probability\left(\eventfive^c\right)\label{rel:simplified_regret:exploit_to_est_err}\\
    \leq & \sum_i\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\explore_i(\ell)\right]    + \sum_i\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\left| \hat{p}_i(\ell) - p_i^*\right|\Big | \eventsix\right] \nonumber\\
    & \qquad + t \left(\probability\left(\eventfive^c\right) + 2\probability\left(\eventsix^c\right) \right).\label{rel:simplified_regret:exploit_to_est_err_condition}
\end{align}
\endgroup
%\Gauri{ In (48), do you mean $\expectation [|\hat{p}_i(\ell) - p_i^*| \indicatorofevents(\eventsix)]$ instead of  $\expectation [\hat{p}_i(\ell) - p_i^*|\Big | \eventsix]$? The conditioning may be correct. But, please add an explanation of how you got (48) from (47) below in the itemized list of explanations}
where,
\begin{enumerate}
    \item \eqref{rel:simplified_regret:use_regret_equation} uses \Cref{clm:regret_equation} and $\eventfive$.
    \item \eqref{rel:simplified_regret:exploit_to_est_err} uses \Cref{clm:false_exploit_to_p_diff}.
    \item \eqref{rel:simplified_regret:exploit_to_est_err_condition} uses the fact that, 
    \begin{align}
        &\sum_i\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\left| \hat{p}_i(\ell) - p_i^*\right|\right] \\
        =& \sum_i\sum_{\ell = t- v_i(t)}^{t-1} \probability\left(\eventsix\right)\expectation\left[\left| \hat{p}_i(\ell) - p_i^*\right|\Big| \eventsix\right] \nonumber\\
        & \qquad + \probability\left(\eventsix^c\right)\expectation\left[\left| \hat{p}_i(\ell) - p_i^*\right|\Big| \eventsix^c\right] \\
        \leq& \sum_i\sum_{\ell = t- v_i(t)}^{t-1} \expectation\left[\left| \hat{p}_i(\ell) - p_i^*\right|\Big| \eventsix\right] + 2t\probability\left(\eventsix^c\right).
    \end{align}
\end{enumerate}
%\Weina{As I re-read this, I am not sure about the arguments again.  I think $\explore_i(\ell)$ is not independent of $\eventfive, \eventsix$ since the arrivals to queue $i$ at $l$ affects the length of the busy period.  I think we need to think over this again.}
%\Gauri{Got it. You can add these equations to the align block from (54) - (58) above. But note that you are missing some terms. $\left(\eventsix\right)$ does'nt make sense.}
%\Tuhin{I missed the probability. I am using conditional expectation.}
%\Gauri{This is a minor grammatical correction, but since I see this mistake several times in the paper, there should be a space before brackets when you use them in text. For example, equation\eqref{rel:simplified_regret:exploit_to_est_err} should be equation \eqref{rel:simplified_regret:exploit_to_est_err}. }
%\Tuhin{Will take of this in future.}
%\Gauri{Claim 1 does not appear to need $v_i(t) < t/2$. Do you mean another claim, the one that uses Hoeffing's inequality to bound the difference between $\hat{p}$ and $p^*$?}
%\Tuhin{Corrected}
\Weina{The second from the last line in the equation above needs proper parentheses.}
Notice $v_i(t) = \order(\ln t) = o(t)$. Hence, if $v_i(t) \leq t/2$, then \eqref{rel:simplified_regret:exploit_to_est_err_condition} can be further simplified using $\eventsix$. Let $t_0$ be some constant such that $v_i(t) \leq t/2$ for all $t \geq t_0$. Then, for all $t\geq t_0$, the expected instantaneous regret can be further simplified as
\begin{align}
    &\expectation\left[\regret_{\policy \policy^*}^{inst}(t)\right]\\
    \leq &\sum_i\sum_{\ell = t- v_i(t)}^{t-1}\left[\expectation\left[ \explore_i(\ell)\right]\right] +\sum_{i:p_i^*>0} k_1v_i(t) \sqrt{\frac{\ln t}{t}} \nonumber\\
    & \qquad + t \left[\probability\left(\eventfive^c\right) + 2\probability\left(\eventsix^c\right) \right]\\
    \leq  &\sum_i\frac{2v_i(t)\ln t}{t} +  \sum_{i:p_i^*>0} k_1v_i(t) \sqrt{\frac{\ln t}{t}} + t\left(\probability\left(\eventfive^c\right) + 2\probability\left(\eventsix^c\right)\right).\label{rel:simplified_final_regret}
\end{align}
%\Gauri{That's a good idea -- I like this version better. When you are introducing a new assumption like saying $t$ should be greater than $t_0$ then, in fact, you should break the flow. This way the readers know that the next set of equations needs additional constraints or assumptions}\Tuhin{Changed.}
% \begingroup
% \allowdisplaybreaks
% \begin{align}
%   &\expectation\left[ \sum_i\left(\queue_i(t) - \queue_i^*(t)\right)\right] \\
%   \leq& \sum_i\expectation\left[ \queue_i(t) - \queue_i^*(t)\Big| \eventfive, \eventsix\right] + t \left[\probability\left(\eventfive^c\right)\right] + \probability\left(\eventsix^c\right) \\
%   \leq & \sum_i\expectation\left[\sum_{\ell = t- \busy_i(t)}^{t-1} \explore_i(\ell) + \sum_{\ell = t- \busy_i(t)}^{t-1} \indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}}\Big| \eventfive, \eventsix\right] + t \left[\probability\left(\eventfive^c\right) + \probability\left(\eventsix^c\right) \right]\label{rel:simplified_regret:use_regret_equation}\\
%   \leq & \sum_i\expectation\left[\sum_{\ell = t- v_i(t)}^{t-1} \explore_i(\ell) + \sum_{\ell = t- v_i(t)}^{t-1} \indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}}\Big| \eventfive, \eventsix\right] + t \left[\probability\left(\eventfive^c\right) + \probability\left(\eventsix^c\right) \right]\\
%   = & \sum_i\left[\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[ \explore_i(\ell)\right]\right] +  \sum_i \expectation\left[\sum_{\ell = t- v_i(t)}^{t-1}\indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}}\Big| \eventfive, \eventsix\right] + t \left[\probability\left(\eventfive^c\right) + \probability\left(\eventsix^c\right) \right]\label{rel:simplified_regret:explore_independent}\\
%   \leq & \sum_i\frac{2v_i(t)\ln t}{t} +  \sum_i\expectation\left[\sum_{\ell = t- v_i(t)}^{t-1} \expectation\left[\indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}}\Big| \hat{p}_i(\ell)\right]\Big| \eventfive, \eventsix\right] + t \left[\probability\left(\eventfive^c\right) + \probability\left(\eventsix^c\right) \right]\label{rel:simplified_regret:explore_iterate_expec}\\
%   = & \sum_i\frac{2v_i(t)\ln t}{t} +  \sum_i \expectation\left[\sum_{\ell = t- v_i(t)}^{t-1} \probability\left[ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\Big| \hat{p}_i(\ell)\right]\Big| \eventfive, \eventsix\right] + t \left[\probability\left(\eventfive^c\right) + \probability\left(\eventsix^c\right) \right]\\
%   \leq & \sum_i \frac{2v_i(t)\ln t}{t} + \sum_i  \expectation\left[\sum_{\ell = t- v_i(t)}^{t-1} \left| \hat{p}_i(\ell) - p_i^*\right|\Big| \eventfive, \eventsix\right] + t \left[\probability\left(\eventfive^c\right) + \probability\left(\eventsix^c\right) \right]\label{rel:simplified_regret:exploit_to_est_err}\\
%   \leq & \sum_i\frac{2v_i(t)\ln t}{t} +  \sum_{i:p_i^*>0} k_1v_i(t) \sqrt{\frac{\ln t}{t}} + t\left(\probability\left(\eventfive^c\right) + \probability\left(\eventsix^c\right)\right)\label{rel:simplified_final_regret}
% \end{align}
% \endgroup
%\Gauri{Why is the condition w.r.t. $\hat{p}_i(l)$ appearing in 6.32 and 6.33 when it was not there 6.31? Then it is going away again in 6.34}
%\Tuhin{I am using law of iterated expectations in 6.32. Weina discussed this idea in one of the meetings. In 6.34 I used \Cref{lem:bound_busy_period_1}. And for some reason, using cref, claim and lemma is shown as theorem like in the statement above. I think I have to change the definitions of lemma and claims. Also, I saw that you added multiple crefname commands in the beginning. I think there is some flaw in that. The "name" part is not within the command(it is not blue in color)}
%\Gauri{You need to change the label of the theorem to the format "thm:.......", for example \Cref{thm:main} for the cleverref package to work. The crefname commands are fine-- I think it is just a overleaf segmenting issue. I have been using the same for all papers.}
%\Gauri{Please check which of the above equations should have equalities instead of inequalities. I can spot several that should be equalities}
%\Tuhin{Done}
where \eqref{rel:simplified_final_regret} follows from the following fact that for $t\geq t_0$ and $v_i(t) \leq t/2$, we have
%    \Gauri{When you sum over $t-v_i(t)$ to $t$ there are $v_i(t)+1$ elements in the sum, not $v_i(t)$}
 %   \Tuhin{Corrected. Changed the definition of $\busy_i(t)$}
\begin{align}
    &\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\explore_i(\ell)\right] \\
    \leq &\sum_{\ell = t- v_i(t)}^{t-1} \frac{\ln \ell}{\ell}\leq v_i(t) \max_{\ell\in \left[t-v_i(t) + 1, t\right]}\frac{  \ln \ell}{\ell}\\
    = &\frac{ v_i(t) \ln \left( t - v_i(t)\right)}{t - v_i(t)} \\
    \leq &\frac{2 v_i(t) \ln t}{t}.\label{rel:explore}
\end{align}
%\Gauri{In 6.34 and 6.35 you need to condition the first two terms with event $E_5$}
%\Gauri{Why does $E_6$ suddenly appear in 6.36? As we discussed today, can't we condition on both $E_5$ and $E_6$ right from the beginning?}
%\Tuhin{Addressed both the comments.}
%\Weina{Just do this for your specific $t_1$ and $t_2$ in \eqref{rel:regret_equation}.  This is unnecessary generalization.}
%\Tuhin{This relation is used more than once. So, I thought it is better to put it in general.}
%\Gauri{Why don't we substitute the expression of the RHS of 6.9 into all the equations below? Then we can analyze the two terms in 6.12 separately. The expectation of the exploration term will be proportional to $\expectation[\busy_i(t)]$, which we can bound in one of the lemmas. And the expectation of the exploitation term will be proportional to the difference between $\hat{p}_i$ and $p_i$, which we can bound in another lemma}
%\Tuhin{The term corresponding to exploration is not proportional to $\expectation[\busy_i(t)]$ unless we have some information about $\busy_i(t)$. The term corresponding to exploitation is a random sum of random variables. The random variables are not independent how can we separate them? I used $\busy_i(t) \leq t/2$}
%\Gauri{Expectation of a sum of random variables is the sum of the expectations of individual terms, even if they are correlated random variables}
%\Tuhin{Okay, I think I can manage that.}
%\Gauri{What information about  $\busy_i(t)$ do you need? Why is it not proportional to $\expectation[\busy_i(t)]$?}
%\Tuhin{Because the $\frac{ln \ell}{\ell}$ term has its minima at $l=t - \busy_i(t)$.}
%\Gauri{Okay, got it}
%\Weina{This is incorrect.  $\busy_i(t)$ is a random variable.  The first term on the right-hand-side should be $\frac{2\expectation[\busy_i(t)] \ln t}{t}$.  To get this you also need to explain that $\explore_i(\ell)$'s are independent from $\busy_i(t)$.  For the second term on the right-hand-side, I don't know how to separate $\busy_i(t)$ out since it is not independent from the $\exploit_i(\ell)$'s.}
%\Tuhin{I believe this issue is solved.}
% \Gauri{We discussed during the last meeting that the above equation should have a equality}
% \Gauri{Write the above equation in terms of $\exploit_i(\ell)\neq \exploit_i^*(\ell)$}

==> old/old_files/old_coupling.tex <==
\subsection{Coupling with the Optimal Weighted Random Routing}
\Weinarevise{Consider the system that runs the optimal weighted random routing policy $\policy^*$, which we refer to as the \emph{optimal system}.  We will annotate quantities in the optimal system with the superscript $^*$, e.g., $\arrival^*(t)$ denotes the total number of job arrivals at time $t$ to the optimal system, and $\queue_i^*(t)$ denotes the length of queue $i$ under $\policy^*$.  Correspondingly, recall that the regret at time $t$ is defined as
\begin{equation*}
\regret_{\policy \policy^*}(t) = \sum_{\tau = 1}^t \sum_{i = 1}^{\numofserver}\left( \queue_i(\tau) - \queue_i^*(\tau)\right).
\end{equation*}}


%\sout{The queue length at any point of time depends on the past arrivals, departures and the assignment of jobs to the servers. Since the arrival and departure of jobs and assignment of jobs to servers are random, it is not easy to directly analyze the difference in queue lengths of two systems at any time. Hence, we will couple the two systems in a way that makes it easier to analyze the difference in the queue lengths. Assume the following coupling between the systems.}
%\Weina{I think this paragraph is redundant.}
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=60mm]{draft_pics/diagrams/coupling1.pdf}
        \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}  
        \centering
        \includegraphics[width=57mm]{draft_pics/diagrams/coupling2.pdf}
        \caption{}
    \end{subfigure}
    \caption{An illustration of coupling of the assignment process for a multi-server model with $4$ servers for $2$ cases.  \Gauri{Nice figure! But the colors are too bright and jarring. I suggest using lighter pastel colors} \Gauri{I am confused by the equations $R_3 = \hat{R}_2$ and $R_3 = \hat{R}_4$ -- how can $R_3$ be equal to two different things?}}
    \label{fig:dia_coupling}
\end{figure*}

\Weinarevise{We couple the system that runs our proposed $\epsilon_t$-exploration policy with the optimal system in the following way.}
\begin{enumerate}[leftmargin=*, wide = 0pt]
    \item \textit{Arrivals.} %\sout{The arrival process is coupled for both the systems. In other words, if the original system sees an arrival, the optimal system following policy $\policy$ will also see an arrival.}
    \Weinarevise{We couple the arrival processes such that $\arrival(t)=\arrival^*(t)$ for all time $t$.}
    %\Weina{``coupled'' is not a mathematically defined term.}
    
    \item \textit{Service.} %\sout{The service process of the systems are coupled. At each time slot $t$, server $i$ in the original system as well as the optimal system generates a common Bernoulli random variable with parameter $\mu_i$, i.e.,} 
    %\begin{equation}
    %    \service_i(t) = \service_i^*(t) \sim Ber(\mu_i).   
    %\end{equation}
    \Weinarevise{To define the coupling for the job service process, we use the following equivalent description of the queueing dynamics due to the geometrically distributed service times.  For each server~$i$, let $\service_i(t)$ for $t=0,1,2,\dots$ be i.i.d.\ Bernoulli random variables that take the value $1$ with probability $\mu_i$.  We will refer to $\service_i(t)$ as the \emph{service} offered by server $i$ at $t$.  If $\queue_i(t)+\arrival_i(t)>0$, we let $\departure_i(t)=\service_i(t)$, where recall that $\departure_i(t)$ is the number of departures from queue $i$ at $t$; otherwise it is clear that $\departure_i(t)=0$. Similarly, let $\service_i^*(t)$ denote the corresponding service offered in the optimal system.
    We couple the service processes such that $\service_i(t)=\service_i^*(t)$ for all server $i$ and all time $t$.}
    %\Weina{I moved the definition of service to here.}
    
    \item \textit{Assignment process.} %\Gauri{The description below of the coupling process is too long and could be cut down significantly}
    % \Tuhin{I wrote one smaller version in the comment. I kept the original one as I am not sure if my version is over-compact or not.}
    For all time $t$, we generate a random variables $\explorerandom(t) = Ber\left(\frac{\numofserver \ln t}{t}\right)$. The policy explores at time $t$ if and only if $\explorerandom(t) = 1$ and the incoming job will be assigned a server at random in such scenario.
    
    In case the policy is using the optimal weighted random routing with the estimates, we generate a common realization $u$ from the uniform distribution $U[ 0,1]$, which is used to assign an incoming job to one of the $K$ servers. For the original system, we divide the interval $[0,1]$ into $K$ disjoint intervals $\subregion_1(t), \subregion_2(t), \cdots, \subregion_\numofserver(t)$ such that $|\subregion_i(t)| = \hat{p}_i(t)$ and $\cup_{i=1}^{\numofserver} \mathcal{G}_i(t) = [0,1]$. If $u \in \mathcal{G}_i(t)$ then the incoming job at time $t$ is assigned to server $i$. Below, we define the intervals $\subregion_1(t), \subregion_2(t), \dots, \subregion_\numofserver(t)$ for the original system and  and similarly $\subregion^*_1(t), \subregion^*_2(t), \dots, \subregion^*_\numofserver(t)$ for the optimal system respectively.
    
    First, define the common interval length $\commonlength_i(t)$, such that for all $i$, 
    \begin{equation}
        \commonlength_i(t) = \min\left(\hat{p}_i(t), p_i^*\right)
    \end{equation}
    Next, we define the residual interval length $\residuallength_i(t)$ for the original system, such that for all $i$,
    \begin{equation}
        \residuallength_i(t) = \max(0, \hat{p}_i(t) - p_i^*).
    \end{equation}
    For the optimal system, we define the residual interval length $\residuallength_i^*(t)$, such that for all $i$,
    \begin{equation}
        \residuallength_i^*(t) = \max(0, p_i^* - \hat{p}_i(t)).
    \end{equation}
    Now, for the original system, divide the interval $[0, 1]$ into $2\numofserver$-sub intervals $(\common_1(t), \common_2(t), \cdots, \common_\numofserver(t), \residual_1(t), \cdots, \residual_\numofserver(t))$ in the given order such that 
    \Gauri{Not clear what you mean by 'given order'}
    \begin{equation}
        \lvert \common_i(t) \rvert = \commonlength_i(t), \lvert \residual_i(t) \rvert = \residuallength_i(t),
    \end{equation}
    where $\lvert . \rvert$ denotes the length of the interval. 
    Similarly, for the optimal system, we divide the interval $[0, 1]$ into $2\numofserver$-sub intervals $(\common_1(t), \common_2(t), \cdots, \common_\numofserver(t), \residual_1^*(t), \cdots, \residual_{\numofserver}^* (t))$ in the given order such that 
    \Gauri{Not clear what you mean by 'given order'}
    \Gauri{Below, you only defined $\lvert \common_i(t) \rvert$ but did not specify what $\common_i(t)$ is}
    \Gauri{I think you can just write the intervals $G_i$ directly in terms of $\alpha_i$ and $\beta_i$ instead of defining new variables $C_i$ and $R_i$.}
    \begin{equation}
        \lvert \common_i(t) \rvert = \commonlength_i(t), \lvert \residual_i^*(t) \rvert = \residuallength_i^*(t),
    \end{equation} 
    Finally, define $\subregion_i(t) = \common_i(t) \cup \residual_i(t)$ and $\subregion_i^*(t) = \common_i(t) \cup \residual^*_i(t)$. A graphical illustration of the coupling in the assignment process is given in \Cref{fig:dia_coupling} .
    
    
    % -----------------------------------------------------------------------
%     First, we define $\numofserver$ intervals 
%     \begin{align}
%         \common_1(t)&= \left[0, \min(\hat{p}_1(t), p_1^*)\right),\\
%         \common_2(t)&= \left[\min(\hat{p}_1(t), p_1^*),  \sum_{i=1}^{2} \min(p_i(t), p_i^*)\right),\\
%         \vdots \nonumber\\
%         \common_\numofserver(t)&= \left[ \sum_{i=1}^{\numofserver - 1}\min(\hat{p}_i(t), p_i^*), \sum_{i=1}^{\numofserver} \min(p_i(t), p_i^*)\right),
%     \end{align}
%     which we refer to as the common intervals since they are identical for the original system and optimal system. Together $\cup_{i=1}^{\numofserver} \common_i(t) = \left[0, \sum_{i=1}^{\numofserver} \min(p_i, p_i^*)\right)$ covers the first part of the interval $[0,1]$.\\
    
%     Next, we define residual intervals and use them to assign the remaining part of the interval $[0,1]$. For the original system, define for all $i\in \left\{1, 2, \cdots, \numofserver\right\}$
%   % \Gauri{You can just write one equation below for $r_j(t)$}
%   %  \Tuhin{Done.}
%     \begin{equation}
%         r_i(t) = \max(0, \hat{p}_i(t) - p_i^*).
%     \end{equation}
%     Similarly, for the optimal system, define for all $i\in \left\{1, 2, \cdots, \numofserver\right\}$
%   %  \Gauri{You can just write one equation below for $r_j(t)$}
%     \begin{equation}
%         r_i^*(t) = \max(0, p_i^* - \hat{p}_i(t)).
%     \end{equation}
%     Observe that $\sum_{i=1}^{\numofserver} r_i(t) = \sum_{i=1}^{\numofserver} r_i^*(t)$. For the system, the remaining part $\left[\sum_{i=1}^{\numofserver} \min(\hat{p}_i(t), p_i^*), 1\right]$ of the interval $[0,1]$ is divided into sub-intervals $\residual_1(t)$, \dots, $\residual_\numofserver(t)$ which are defined as: 
%     \begin{equation}
%     \begin{split}
%         \residual_j(t)= \Bigg[\sum_{i=1}^{K}\min(\hat{p}_i(t), p_i^*) + \sum_{i=1}^{j-1} r_i(t),\\
%         \sum_{i=1}^{K}\min(\hat{p}_i(t), p_i^*) +  \sum_{i=1}^{j} r_i(t)\Bigg],
%     \end{split}
%     \end{equation}
%     which we refer to as residual intervals. Similarly, for the optimal system, the remaining part $\left[\sum_{i=1}^{\numofserver} \min(\hat{p}_i(t), p_i^*), 1\right]$ of the interval $[0,1]$ is divided into sub-intervals $\residual^*_1(t)$, \dots, $\residual^*_\numofserver(t)$ which are defined as: 
%     \begin{equation}
%     \begin{split}
%         \residual^*_j(t)= \Bigg[\sum_{i=1}^{K}\min(\hat{p}_i(t), p_i^*) + \sum_{i=1}^{j-1} r^*_i(t),\\
%         \sum_{i=1}^{K}\min(\hat{p}_i(t), p_i^*) +  \sum_{i=1}^{j} r^*_i(t)\Bigg],
%     \end{split}
%     \end{equation}
    
%     Now $\subregion_i(t) = \common_i(t) \cup \residual_i(t)$ and $\subregion_i^*(t) = \common_i(t) \cup \residual^*_i(t)$. If $u \in \subregion_i(t)$ then the incoming job at time $t$ is assigned to server $i$ in the original system and if $u \in \subregion_i^*(t)$, then the incoming job at time $t$ is assigned to server $i$ in the optimal system. A graphical illustration of the coupling in the assignment process is given in \Cref{fig:dia_coupling} 
    
    
    % ------------------------------------------------------------------------
    % \Gauri{Drawing a picture to illustrate the intervals of $[0,1]$ and how they are assigned in the two coupled assignments will make this whole explanation much more clear}

 %   \Tuhin{I thought about adding one after the mathematical issues are resolved.}
  %  \Gauri{The math seems good now. You can go ahead and add a figure}
    % \begin{equation}
    %     \common_i(t) = \min\left\{\hat{p}_i(t), p_i^*\right\}.
    % \end{equation}
%    \Gauri{Since the common intervals are the same, you don't need two separate notations $C_i$ and $C_i^*$}
 %   \Tuhin{Changed.}
    % \begin{equation}
    %     \residual_i(t) = \max\left\{\hat{p}_i(t) - p_i^*, 0\right\}.
    % \end{equation}
    % \begin{equation}
    %     \residual_i^*(t) = \max\left\{p_i^* - \hat{p}_i(t), 0\right\}.
    % \end{equation}
%    \Gauri{The total number of servers is $K$. So how can $i$ not be in $[1,K]$? By $[1,K]$ do you mean the set $\{1, K\}$ or the whole set $\{1, 2, \dots K\}$? I interpret $[1,K]$ as  $\{1, 2, \dots K\}$}\Tuhin{$[1, K]$ is $\{1, 2, ..., K\}$. While writing the expression of $\subregion$, I have terms like $\common_0(t)$, which is not defined. So to avoid those confusions, I defined that for all $i\notin [1, K]$, $\common_i, \residual_i = 0$}
%    \Gauri{I see. Please change the notations and the explanations to avoid saying $i\notin [1, K]$ -- it causes unnecessary confusion. I am reading through the rest of this coupling argument carefully and will let you know if I have any ideas of explaining this in a different way} 
%    \Gauri{Also $[1,K]$ actually means the real interval between 1 and K. Use $\{1, 2, \dots K\}$ instead}
   % \Tuhin{Corrected.}
    % For all $i \notin \{1,2, \cdots, \numofserver\}$, assume
    % \begin{equation}
    %     \common_i(t) = \residual_i(t) = \residual_i^*(t) = 0.
    % \end{equation}
    % It is then easy to show that 
    % \begin{equation}
    %     \sum_{i=1}^{\numofserver} \left(\common_i(t) + \residual_i(t)\right) = \sum_{i=1}^{\numofserver}\left( \common_i(t) + \residual_i^*(t)\right) = 1.
    % \end{equation}
%      \Gauri{Since $C_i^*$ and $C_i$ can be replaced by just one common notation, the above equation can just be written as $\sum_{i=1}^{\numofserver}  \residual_i(t) = \sum_{i=1}^{\numofserver} \residual_i^*(t)$}
    % Also, observe that for all $i$,
    % \begin{equation}
    %     \min\left\{\residual_i(t), \residual_i^*(t)\right\} = 0.
    % \end{equation}
    % For system following the optimal policy $\policy^*$, divide the region $[0,1]$ into $2\numofserver$ sub-regions, namely $\subregion_1^*(t), \subregion_2^*(t), \cdots, \subregion_{2\numofserver}^*(t)$ such that 
%    \Gauri{Please don't use words like 'common', 'residual' or 'sub' to denote random variables or constants. Use single-letters such as $U$, $R$, etc.}
%    \Tuhin{Changed.}
    % \begin{equation}
    %     \subregion_i^*(t) := \left[\sum_{j = 0}^{i-1} \common_j(t), \sum_{j = 0}^{i} \common_j(t)\right), \forall i \leq \numofserver,
    % \end{equation}
    % \begin{equation}
    %     \subregion_{\numofserver + i}^*(t) := \left[\sum_{j = 0}^{\numofserver} \common_j(t) + \sum_{j = 0}^{i-1} \residual_j^*(t), \sum_{j = 0}^{\numofserver} \common_j(t) + \sum_{j = 0}^{i} \residual_j^*(t)\right), \forall i \leq \numofserver.
    % \end{equation}
 
    % For any interval $\mathcal{I}$, let $|\mathcal{I}|$ denote the length of the interval. Notice, that for any i,
    % \begin{equation}
    %     \left|\subregion_i^*(t)\right| + \left|\subregion_{\numofserver + i}^*(t)\right| = \min\left\{\hat{p}_i(t), p_i^*\right\} + \max\left\{p_i^* - \hat{p}_i(t), 0\right\} = p_i^*.
    % \end{equation}
    %\Tuhin{How to write length of interval?}
   % \Weina{I think the absolute value you have is a good choice here but you need to add one sentence to define that, e.g., ``let $|\mathcal{I}|$ denote the length of an interval $\mathcal{I}$.''}
   % \Tuhin{Done.}
    % Similarly, for the system following policy $\policy$, divide the region $[0,1]$ into $2\numofserver$ sub-regions, namely $\subregion_1(t), \subregion_2(t), \cdots, \subregion_{2\numofserver}(t)$ such that 
    % \begin{equation}
    %     \subregion_i(t) := \left[\sum_{j = 0}^{i-1} \common_j(t), \sum_{j = 0}^{i} \common_j(t)\right), \forall j \leq \numofserver,
    % \end{equation}
    % \begin{equation}
    %     \subregion_{\numofserver + i}(t) := \left[\sum_{j = 0}^{\numofserver} \common_j^*(t) + \sum_{j = 0}^{i-1} \residual_j(t), \sum_{j = 0}^{\numofserver} \common_j(t) + \sum_{j = 0}^{i} \residual_j(t)\right), \forall i \leq \numofserver.
    % \end{equation}
    % Now, the coupling works as follows, 
    % \begin{enumerate}
    %     \item Every incoming job generates a common random variable $U\sim Unif[0, 1]$.
    %     \item For the system following $\policy^*$, the job is sent to server $i$, if $U\in \subregion_i^*(t)$ or $U\in \subregion_{\numofserver + i}^*(t)$.
    %     \item For the system following $\policy$, the job generates another random variable $\explorerandom(t) \sim Ber\left(\frac{\numofserver \ln t}{t}\right)$. The job is sent to server $i$ through exploitation, if $U\in \subregion_i(t)$ or $U\in \subregion_{\numofserver + i}(t)$ and $\explorerandom(t) = 0$. If $\explorerandom(t) = 1$, the job is sent to any server at random.
    % \end{enumerate}
\end{enumerate}
%\Gauri{You did a great job of editing this section! Well done!}
%\Gauri{I would rewrite the coupling argument as follows: We generate a common realization $u$ from the uniform distribution $U[ 0,1]$, which is used to assign an incoming job to one of the $K$ servers. For the a policy $\mathcal{P}$ we divide the $[0,1]$ into $K$ disjoint intervals $\mathcal{G}_1, \mathcal{G}_2, \dots, \mathcal{G}_K$ such that $|G_i| = p_i$ and $\cup_{i=1}^{K} \mathcal{G}_i = [0,1]$. If $u \in \mathcal{G}_i$ then the incoming job is assigned to server $i$. Below, we define the intervals $\mathcal{G}_1, \mathcal{G}_2, \dots, \mathcal{G}_K$ and $\mathcal{G}^*_1, \mathcal{G}^*_2, \dots, \mathcal{G}^*_K$ for the bandit exploitation and the optimal randomized policies respectively. For these interval definitions we can bound the probability of mismatch between the bandit and the optimal randomized assignments (see \Cref{clm:false_exploit_to_p_diff} below).\\
%First define $K$ intervals $\mathcal{C}_1 = [0, \min(\hat{p}_1, p_1^*))$, $\mathcal{C}_2 = [\min(\hat{p}_1, p_1^*), \min(\hat{p}_1, p_1^*)+\min(\hat{p}_2, p_2^*))$, \dots $\mathcal{C}_K = [ \sum_{i=1}^{K-1}\min(\hat{p}_i, p_i^*), \sum_{i=1}^{K} \min(p_i, p_i^*))$, which we refer to as the common intervals since they are identical for the bandit exploitation and optimal randomized policies. Together $\cup_{i=1}^{K} \mathcal{C}_i = [0, sum_{i=1}^{K} \min(p_i, p_i^*))$ covers the first part of the interval $[0,1]$.\\
%Next, we define residual probabilities which are different for the two policies, and use them to assign the remaining part of the interval $[0,1]$. For the bandit exploitation policy, define $r_1 = \max(0, \hat{p}_1 - p_1^*)$, $r_2 = (\max(0, \hat{p}_2 - p_2^*)$, \dots $r_K = \max(0, \hat{p}_K - p_K^*)$. Similarly, for the optimized randomized policy, let $r^*_1 = \max(0, p_1^*-\hat{p}_1 )$, $r^*_2 = \max(0, p_2^*-\hat{p}_2)$, \dots $r^*_K = \max(0, p_K^*-\hat{p}_K)$. Observe that $\sum_{j=1}^{K} r_j = \sum_{j=1}^{K} r_j^*$. The remaining part $[\sum_{i=1}^{K} \min(p_i, p_i^*), 1]$ of the interval $[0,1]$ is divided into sub-intervals $R_1$, \dots, $R_K$ which are defined as: $\mathcal{R}_j= [\sum_{i=1}^{K}\min(p_i, p_i^*), \sum_{i=1}^{K}\min(p_i, p_i^*) +  \sum_{\ell=1}^{j} r_j]$, which we refer to as residual intervals. \\
%Now $\mathcal{G}_i = \mathcal{C}_i \cup \mathcal{R}_i$ and $\mathcal{G}_i^* = \mathcal{C}_i \cup \mathcal{R}_i$. If $u \in \mathcal{G}_i$ then the incoming job is assigned to server $i$ in the bandit system and if $u \in \mathcal{G}_i^*$, then the incoming job is assigned to server $i$ in the optimal randomized system. }
%\Tuhin{That sounds way cleaner. There is one correction though. The above assignment is only when bandit is exploiting. For exploration, we do not have any coupling strategy. I may have to just re-phrase what you wrote to }
%\Gauri{yes, right. I will write the above argument only for the exploitation case. You can modify it to capture exploration}
%\Gauri{General guidance based on the above rewriting: When you are introducing new notations such as $C$, $R$ etc., first give the reader an idea of why you are doing so and then give the formal definitions. That is why I defined $u$ right at the beginning rather than at the end.}
%\Tuhin{Thanks for the writeup. I will try to take care of this in future.}
With the coupling defined above and given that the estimates $\hat{p}_i(\ell)$'s are known, we can make the following claim on the probability of mismatch in allocation in the two systems.
\begin{clm}
\label{clm:false_exploit_to_p_diff}
    $\probability\left[ \exploit_i(\ell) = 1,  \arrival_i^*(\ell) = 0\Big|  \hat{p}_i(\ell)\right]\leq |\hat{p}_i(\ell) - p_i^*|.$
\end{clm}
% \Gauri{Use the begin proof and end proof environment to write proofs}
% \Tuhin{Thanks for the info. I wasn't aware of this environment}
% \Gauri{Please change it everywhere else as well}
% \Tuhin{Done.}
\begin{proof}
\begin{align}
    & \probability\left[ \exploit_i(\ell) = 1,  \arrival_i^*(\ell) = 0\Big|  \hat{p}_i(\ell)\right]\\
    \leq& \probability\left[u \in \subregion_{i}(\ell), u \notin \subregion_{i}^*(\ell)  \Big|\hat{p}_i(\ell) \right]\\
    \leq& \probability\left(u \in \residual_{i}(\ell)\Big| \hat{p}_i(\ell)\right)\\
    \leq& \residuallength_i(\ell)\\
    \leq& |\hat{p}_i(\ell) - p_i^*|.
\end{align}
\end{proof}

%\Weina{To-do later: we may need to move the paragraph below.  It is easy to miss it here since it is at the end of a section called coupling.}
%\Gauri{My earlier comment was similar to Weina's comment above. So adding it here again}
%\Gauri{There is change of context here and this may be a good place to start a new subsection. Please give the readers a clear roadmap of what the high-level sketch of the proof is going to look like from here onwards.}
%\Tuhin{Changed it.}

Intuitively, \Cref{clm:false_exploit_to_p_diff} suggests that once the estimates $\hat{p}_i(\ell)$'s are close to $p_i^*$'s, the probability of mismatch from optimal weighted random routing is small.

%\Tuhin{The difference in queue length also comes from the coupling of the 2 systems. Creating a subsection after that might be more appropriate.}
%\Gauri{Okay, then it is fine. I will read through the coupling section again to see how it flows}
% \Tuhin{
% Proof Idea to reduce regret to $\order\left(poly(\log)\right)$
%     \begin{align}
%         \queue_i(t) - \queue_i^*(t) &= \queue_i(t-\busy_i(t)) - \queue_i^*(t - \busy_i(t))  + \sum_{\ell = t- \busy_i(t)}^{t-1}\left(\arrival_i(\ell) - \departure_i(\ell) - \left(\arrival_i^*(\ell) - \departure_i^*(\ell)\right)\right)\\
%         &\leq \sum_{\ell = t- \busy_i(t)}^{t-1}\left(\arrival_i(\ell) - \arrival_i^*(\ell)\right)  + \sum_{\ell = t- \busy_i(t)}^{t-1}\left(\departure_i^*(\ell) - \departure_i(\ell)\right)\\
%         &\leq \sum_{\ell = t- \busy_i(t)}^{t-1} \left(\explore_i(\ell) + \exploit_i(\ell) - \arrival_i^*(\ell)\right) +  \sum_{\ell = t- \busy_i(t)}^{t-1} \left(\service_i^*(\ell) - \service_i(\ell) \right)\\
%         &= \sum_{\ell = t- \busy_i(t)}^{t-1} \explore_i(\ell) + \sum_{\ell = t- \busy_i(t)}^{t-1} \left(\exploit_i(\ell) - \arrival_i^*(\ell)\right)\\
%         &\leq \sum_{\ell = t- \busy_i(t)}^{t-1} \explore_i(\ell) + \sum_{\ell = t- \busy_i(t)}^{t-1} \left[\indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}} - \indicatorofevents_{ \left\{ \exploit_i(\ell)=0, \arrival_i^*(\ell) = 1\right\}}\right].
%     \end{align}
%     Then, 
%     \begingroup
% \allowdisplaybreaks
% \begin{align}
%     \regret(t) =& \expectation\left[ \sum_i\left(\queue_i(t) - \queue_i^*(t)\right)\right] \\
%     \leq &\sum_i\expectation\left[ \sum_{\tau_i = 1}^{v_i(t)}\left(\queue_i(t) - \queue_i^*(t)\right)\indicatorofevents\left\{\busy_i(t) = \tau_i\right\} + \left(\queue_i(t) - \queue_i^*(t)\indicatorofevents\left\{
%     \eventfive^c\right\}\right)\right] \\
%     \leq &\sum_i\sum_{\tau_i = 1}^{v_i(t)}\sum_{\ell = t- \tau_i}^{t-1}\expectation\left[  \explore_i(\ell) +  \indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}} - \indicatorofevents_{ \left\{ \exploit_i(\ell)=0, \arrival_i^*(\ell) = 1\right\}}\right]\probability\left(\busy_i(t) = \tau_i\right)  + t\probability\left(\eventfive^c\right)\\
%     \leq &\sum_i\sum_{\tau_i = 1}^{v_i(t)}\sum_{\ell = t- \tau_i}^{t-1}\expectation\left[  \explore_i(\ell) +  \expectation\left[\indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}} - \indicatorofevents_{ \left\{ \exploit_i(\ell)=0, \arrival_i^*(\ell) = 1\right\}}\Big|\hat{p}_i(\ell)\right]\right]\probability\left(\busy_i(t) = \tau_i\right)  + t\probability\left(\eventfive^c\right)\\
%     \leq &\sum_i\sum_{\tau_i = 1}^{v_i(t)}\sum_{\ell = t- \tau_i}^{t-1}\expectation\left[  \explore_i(\ell) +  \expectation\left[\left(\hat{p}_i(\ell) - p_i^*\right)^{+} - \left(p_i^* - \hat{p}_i(\ell)\right)^{+} \Big|\hat{p}_i(\ell)\right]\right]\probability\left(\busy_i(t) = \tau_i\right)  + t\probability\left(\eventfive^c\right)\\
%     \leq &\sum_i\sum_{\tau_i = 1}^{v_i(t)}\sum_{\ell = t- \tau_i}^{t-1}\expectation\left[  \explore_i(\ell) +  \hat{p}_i(\ell) - p_i^*\right]\probability\left(\busy_i(t) = \tau_i\right)  + t\probability\left(\eventfive^c\right)\\
%     \leq &\sum_i\sum_{\tau_i = 1}^{v_i(t)}\sum_{\ell = t- \tau_i}^{t-1}\expectation\left[  \explore_i(\ell)\right]\probability\left(\busy_i(t) = \tau_i\right) + \sum_i\sum_{\tau_i = 1}^{v_i(t)}\sum_{\ell = t- \tau_i}^{t-1}\expectation\left[\hat{p}_i(\ell) - p_i^*\right]\probability\left(\busy_i(t) = \tau_i\right)  + t\probability\left(\eventfive^c\right)\\
%     \leq &\sum_i\sum_{\tau_i = 1}^{v_i(t)}\frac{2\tau_i \ln t}{t}\probability\left(\busy_i(t) = \tau_i\right) + \sum_i\sum_{\tau_i = 1}^{v_i(t)}\sum_{\ell = t- \tau_i}^{t-1}\expectation\left[\hat{p}_i(\ell) - p_i^*\right]\probability\left(\busy_i(t) = \tau_i\right)  + t\probability\left(\eventfive^c\right)\\
%     \leq &\sum_i\frac{2v_i(t) \ln t}{t} + \sum_i\sum_{\tau_i = 1}^{v_i(t)}\sum_{\ell = t- \tau_i}^{t-1}\expectation\left[\hat{p}_i(\ell) - p_i^*\right]\probability\left(\busy_i(t) = \tau_i\right)  + t\probability\left(\eventfive^c\right)
% \end{align}
% \endgroup
% }
% \Tuhin{Now to reduce the second expression we need to upper bound the expression,
% \begin{align*}
%     \expectation\left[\hat{p}_i(\ell) - p_i^*\right] &\leq \expectation\left[\left[\sum_j D_j\hat{p}_i(\ell)\left(\boldsymbol{\mu}\right)\left(\hat{\mu}_j(\ell) - \mu_j\right) + \sum_{k,j} D_{kj}\hat{p}_i(\ell)\left(\boldsymbol{z}\right)\left(\hat{\mu}_j(\ell) - \mu_j\right)\left(\hat{\mu}_k(\ell) - \mu_k\right)\right]\indicatorofevents\left\{\eventone\right\}\right] + \probability\left(\eventone^c\right)\\
%     &\leq \sum_j \left|D_j\hat{p}_i(\ell)\left(\boldsymbol{\mu}\right)\expectation\left[\hat{\mu}_j(\ell) - \mu_j\right]\right| + \sum_{k,j}\left|\expectation\left[ D_{kj} \hat{p}_i(\ell) \left(\boldsymbol{z}\right) \left(\hat{\mu}_j(\ell) - \mu_j\right)\left(\hat{\mu}_k(\ell) - \mu_k\right)\right]\right| + \probability\left(\eventone^c\right)
% \end{align*}
% where $D_j\hat{p}_i(\ell)(\boldsymbol{x}) = \frac{\partial}{\partial \hat{\mu}_j}\hat{p}_i(\ell)\Big|_{\boldsymbol{\hat{\mu}} = \boldsymbol{x}}$ and $D_{kj}\hat{p}_i(\ell)(\boldsymbol{x}) = \frac{\partial^2}{\partial \hat{\mu}_j\partial \hat{\mu}_k}\hat{p}_i(\ell)\Big|_{\boldsymbol{\hat{\mu}} = \boldsymbol{x}}$. Now
% \begin{align}
%     \expectation\left[\hat{\mu}_j(\ell) - \mu_j\right] &\leq  \expectation\left[\sum_{n_j =\frac{p_j^* \lambda t}{32}}^t  (\hat{\mu}_j(\ell) - \mu_j) \indicatorofevents\left\{\sum_{\tau' = 1}^{\ell} \departure_j(\tau') = n_j\right\}\right] + \probability\left(\sum_{\tau' = 1}^{\ell} \departure_j(\tau') < \frac{p_j^* \lambda t}{32}\right)\\
%     &\leq  \sum_{n_j =\frac{p_j^* \lambda t}{32}}^t  \frac{\mu_j}{n_j - 1} \probability\left\{\sum_{\tau' = 1}^{\ell} \departure_j(\tau') = n_j\right\} + \probability\left(\sum_{\tau' = 1}^{\ell} \departure_j(\tau') < \frac{p_j^* \lambda t}{32}\right)\\
%     &\leq  \frac{\mu_j}{\frac{p_j^* \lambda t}{32} - 1} + \probability\left(\eventsix^c\right)
% \end{align}
% Similarly,
% \begin{align}
%     &\expectation\left[\sum_{k,j} D_{kj} \hat{p}_i(\ell) \left(\boldsymbol{z}\right) \left(\hat{\mu}_j(\ell) - \mu_j\right)\left(\hat{\mu}_k(\ell) - \mu_k\right)\right] \\
%     \leq &\expectation\left[\left(\sum_{k,j} D_{kj} \hat{p}_i(\ell) \left(\boldsymbol{z}\right) \left(\hat{\mu}_j(\ell) - \mu_j\right)\left(\hat{\mu}_k(\ell) - \mu_k\right)\right) \indicatorofevents\left(\eventsix\right)\right] + \expectation\left[\left(\sum_{k,j} D_{kj} \hat{p}_i(\ell) \left(\boldsymbol{z}\right) \left(\hat{\mu}_j(\ell) - \mu_j\right)\left(\hat{\mu}_k(\ell) - \mu_k\right)\right) \indicatorofevents\left(\eventsix^c\right)\right] \\
%     \leq & D_{k, j, i}^{\max}\left(k_{11}\sqrt{\frac{\ln t}{t}}\right)k_{11}^2 \frac{\ln t}{t} + \probability\left(\eventsix^c\right)
% \end{align}
% Using all these, the regret can be upper bounded by 
% \begin{align}
%     \regret(t) \leq \sum_iv_i(t)\left( \frac{2 \ln t}{t} + \left(\sum_j D_j\hat{p}_i(\ell)\left(\boldsymbol{\mu}\right)\frac{\mu_j}{\frac{p_j^* \lambda t}{32} - 1}   + \sum_{k, j}D_{k, j, i}^{\max}\left(k_{11}\sqrt{\frac{\ln t}{t}}\right)k_{11}^2 \frac{\ln t}{t}  \right)\right) +  \probability\left(\eventfive^c\right) + \probability\left(\eventsix^c\right)
% \end{align}
% }

%\Tuhin{Yes, I did that only, but the summation is from $\ell = t-\busy_i(t)$ to $\ell =t$. So there are terms like $\frac{\ln (t-B)}{t-B}$}
%\Gauri{Please think about this carefully again. The summation is w.r.t $l$, not $t$}
%\Tuhin{Sorry, I meant $\ell$ only.}
%\Gauri{Again, please think carefully before immediately responding to me here.. I don't see why we need 6.26.}
% \Weina{Use curly brackets for events.  This means all the subscripts of indicators should be inside curly brackets, e.g., $\indicatorofevents_{\{\exploit_i(\ell)\neq \exploit_i^*(\ell)\}}$.}
% \Weina{If you want to put superscript $^*$ on quantities to mean that they are corresponding quantities under the optimal policy, you need to explain this notation system explicitly and clearly.}
%\Gauri{Why do we need to keep switching back and forth between indicators and $A$ above? $A$'s are Bernoulli and indicators are also Bernoulli. In particular, I believe only one of $A^{(explore)}$ and $A^{(exploit)}$ can be positive at a given time for a given server. Can't you write $A = A^{(explore)} + A^{(exploit)}$? Please think carefully and try to condense some of the equations if possible}
%\Tuhin{True, but we need to analyze explore and exploit separately, hence I separated the indicator R.V. I can , but that solve that. I cannot solve bhttps://www.overleaf.com/project/5eb8c89ea4506d000152a4c3oth exploit and explore simultaneously}
%\Gauri{Please think about this a little more}
%\Tuhin{Okay}
%\Tuhin{Also, I am not seeing any switching between indicator and bernoulli, can mention the line?}
%\Gauri{ 6.21 --> 6.22 --> 6.23 --> 6.24}
%\Tuhin{I see, got your point.}
%\Tuhin{I am using the fact that $\frac{\ln \ell}{\ell}$ is a decreasing sequence $\forall \ell \geq e$(consider it is always decreasing for simplicity). Hence $\max_{l\in (t-\busy_i(t), t)} \frac{\ln \ell}{\ell} = \frac{\ln (t - \busy_i(t))}{t - \busy_i(t)}$. This gives us 
% \begin{equation*}
%     \sum_{\ell = t - \busy_i(t)}^{t} \frac{\ln \ell}{\ell} \leq \sum_{\ell = t - \busy_i(t)}^{t} \frac{\ln \left(t - \busy_i(t)\right)}{t - \busy_i(t)} \leq \frac{ \busy_i(t) \ln \left( t - \busy_i(t)\right)}{t - \busy_i(t)}
% \end{equation*}
% Now, I do not know how to interpret $\frac{ \busy_i(t) \ln \left( t - \busy_i(t)\right)}{t - \busy_i(t)}$, but if $\busy_i(t) \leq t/2$, then the numerator is upper bounded by $\ln t$ and denominator is lower bounded by $t/2$, thus giving the bound. \\
% In the above comments, you wrote $\expectation(\explore_i(\ell)) = \frac{\ln t}{t}$, it should be $\frac{\ln \ell}{\ell}$, let me know if this is clear now.}
%\Gauri{I don't get why we need $\busy_i(t) \leq t/2$ for the above equation to hold.}
%\Tuhin{Do I need to show the math, it is a simple calculation. Basically I am using the concave nature of $log^2$. Hence, difference in function value is less than gradient times}
%\Gauri{Yes, please show the math, in particular, where exactly you need $\busy_i(t) \leq t/2$}
%\Tuhin{Okay}
%\Tuhin{Is this enough?}
%\Gauri{Okay, please add this explanation to the above equations.}
%\Gauri{Won't the assumption $\busy_i(t) \leq t/2$ affect the rest of your proof? Where does it fit into the main skeleton of the proof?}
%\Tuhin{Yes, it does. Infact, that is why for all the lemma's I mentioned that the lemma is true for all $t\geq t_0$. I choose the $t_0$ in such a way that $v_i(t)  = O(\ln t)< t/2$. Others things are not a concern.}
%\Gauri{I think this is related to the term $v_i(t)$ that you are introducing later on. Maybe you can just stop the above derivation at 6.24? Because you are starting from 6.24 in equation 6.33. Equation 6.25 does not seem to be used later on}
%\Tuhin{Agreed. I will change it.}
%\Gauri{Okay, great! There are several references to 6.25 in the next part of the proof. I believe those can be replaced by 6.24 then. And if you don't need 6.25, you don't need to add 6.26 either.}
%\Tuhin{I think I will shift the entire B(t) related argument after good events are mentioned. Basically stop at equation 6.24 like you mentioned.}
%\Gauri{Sounds good! :)}
% Hence, taking an expectation would give us, 
%\Gauri{Can merge the equations below with the above align block for better clarity}
%\Tuhin{Done}

==> old/old_files/old_optimal_system.tex <==
\subsection{Optimal system, Departure process and Notation}
\Weina{Notation is an uncountable noun.  Google for the correct usage.}
To analyze the system, we will first define a few notations. Recall, $\arrival_i(t)$ and $\departure_i(t)$ denote the number of arrivals to queue $i$ and the number of departures from queue $i$ at time $t$ respectively in the original system. Since a job can enter the system through either $\epsilon$-exploration or exploitation, we refer $\explore_i(t)$ and $\exploit_i(t)$ as the number of jobs arriving through exploration and exploitation respectively at queue $i$ at time $t$. Hence, for all $t$, and for all $i$,
\begin{equation}
    \arrival_i(t) = \explore_i(t) + \exploit_i(t).
\end{equation}
\Weina{The superscripts need to be shorter.}
\Weina{The subscripts for $\explore_i$ and $\exploit_i$ look very weird.  You need to figure out how to put the $i$ as a subscript of $A$ rather than a subscript of $\explore$.}
%\Weina{Can we just define $\arrival_i(t)$ and $\departure_i(t)$ to be the number of arrivals and departures instead of indicator random variables?  This way the notation may generalize to non-geometric distributions for interarrival and service times.}
%\Tuhin{Did that.}
%\Weina{I think $E$ looks too much like expectation and $I$ looks too much like a generic indicator function.  How about we use $\arrival^{(\text{E})}$ and $\arrival^{(\text{I})}$?}
%\Gauri{Good idea! We could even write something like  $\arrival^{(\text{Explore})}$ and $\arrival^{(\text{Exploit})}$ for better clarity.}

The departure process works as follows. At each time slot, server $i$ offers a service with probability $\mu_i$ and denies service with probability $(1-\mu_i)$. There is a departure from queue $i$ if queue $i$ is non-empty and server $i$ offers a service. Let $\service_i(t)$ denotes the offered service by server $i$ at time $t$, i.e, $\service_i(t) = 1$, if server $i$ offers a service at time $t$, and $0$ otherwise. 
\Weina{Need to mention how this is related to the dynamics in Section 2.1.}

Now, consider an alternate system which is a replica of our original system, except that the dispatcher has full information of the service rates of different servers and is using the optimal policy $\policy^*$ to dispatch the jobs. We refer to the system as the \textit{optimal system}. Now, the regret analysis essentially boils down to comparing the queue length of our original system and the optimal system at each time.

We will use the superscript $(*)$ to denote the corresponding associated variables with the optimal system. For example, $\arrival_i^*(t)$ denotes the number of arrival to server $i$ at time $t$ in the optimal system while $\service_i^*(t)$ denotes the service offered by server $i$ at time $t$ in the optimal system.


% Then for our system,  $\service_i(t) \sim Ber( \mu_i)$, and $\departure_i(t) = \service_i(t)$ if $\queue_i(t) > 0$ and $\departure_i(t) = 0$ otherwise. From the definition, clearly 
% \begin{equation*}
%     \sum_t \departure_i(t) \leq \sum_t\service_i(t),\>\forall i.
% \end{equation*}

 With the terminologies defined above, the regret $\regret_{\policy \policy^*}(t)$ can be expressed as
\begin{equation}
    \regret_{\policy \policy^*}(t) \sum_{\tau = 1}^t \sum_{i = 1}^\numofserver \left(\queue_i(t) - \queue^*(t)\right).
\end{equation}

\Weina{There are several typos in this formula.  @Tuhinangshu, you need to proof read.}

\Weina{This subsection put several different things together without clear purposes.  I suggest to eliminate this section and integrate the content into the next section and call that section ``Coupling with the optimal system''.}

% A summary of all the parameters and notations is given in table \ref{tab:parameter_description} and \ref{tab:notation}.
% \begin{table*}
% \centering
% \caption{System parameters}
% \begin{tabular}{ccl}
% \toprule
% Parameter & Description \\
% \midrule
% $\numofserver$   &   Number of servers    \\
% $\lambda$   &   Arrival rate of jobs    \\
% $\mu_i$     &   Departure rate of jobs from $i^{th}$ server \\
% $p_i^*$       & Probability of sending job to server $i$ according to optimal randomized policy   \\
% $\freecapacity_i$       & residual capacity of server $i$ given by $\mu_i - \lambda p_i^*$   \\
% $\Delta_{support}$    &   Optimal support vector gap  \\
% \bottomrule
% \end{tabular}
% \label{tab:parameter_description}
% \end{table*}
% \begin{table*}
% \centering
% \caption{Variable description}
% \begin{tabular}{ccl}
% \toprule
% Symbol & Description \\
% \midrule
% $\arrival_i(t)$    &   Number of jobs arriving at server $i$ at time t     \\
% $\departure_i(t)$    &   Number of jobs departing from server $i$ at time t     \\
% $\service_i(t)$    &   Indicator random variable denoting service offered by server $i$ at time t      \\
% $\explore_i(t)$    &   Number of jobs arriving at server $i$ at time t through exploration     \\
% $\exploit_i(t)$    &   Number of jobs arriving at server $i$ at time t through exploitation   \\
% $Q_i(t)$    &   Number of jobs queued at server $i$ at time $t$     \\
% $\hat{\mu}_i(t)$ & Estimate of $\mu_i$ at time $t$   \\
% $\hat{p}_i(t)$ & Probability of sending job to server $i$ at time $t$ estimated using $\hat{\mu}_1(t), \hat{\mu}_2(t),\cdots \hat{\mu}_\numofserver(t)$   \\
% \bottomrule
% \end{tabular}
% \label{tab:notation}
% \end{table*}
% Unless specified any normal script is used to denote parameters or variables of the bandit policy and $(.)^*$ is used to define the parameters or variables of the optimal policy
%-------------------------------------Section showing all the lemmas---------------------------------------------%
%\Gauri{Unfortunately, all the notations are currently hard-coded -- no macros. It will be very tedious to change them, and I think we will definitely need to change some of the notation...}
%\Tuhin{Did not get which notation you are referring to}
%\Gauri{All the notations in the paper such as $K$, $p$, $A$, $D$, $S$ etc.}
% Lemma to show the convergence of p with the convergence of p

==> old/old_files/old_proof_theorem.tex <==
\subsection{Important Lemmas, Proof of Theorem \ref{thm:main}}

% -------------------------------------------------------------------
% \include{plot}
\begin{figure*}
    \centering
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[scale = 0.35]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_1.pdf}
        \caption{$\lambda = 0.1$}
    \end{subfigure}
    \begin{subfigure}{0.33\linewidth}  
        \centering 
        \includegraphics[scale = 0.35]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_2.pdf}
        \caption{$\lambda = 0.2$}
    \end{subfigure}
    \begin{subfigure}{0.33\linewidth}  
        \centering 
        \includegraphics[scale = 0.35]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_4.pdf}
        \caption{$\lambda = 0.4$}
    \end{subfigure}
    \caption{Regret vs time for various policies. The shaded region represent $\pm2\sigma$ boundary of the mean regret. TS and UCB performs well in load load regime, while $K/t$-greedy exploration policy performs well in higher traffic regimes. Our policy moderately in very low load regime and performs well in higher traffic regimes. \Weina{Need to replace the ``-greedy'' with ``-exploration'' to be consistent with Section~4.} \Gauri{Reorder the plots such that our policy is either the first or the last in the legend. Also, in the legend, say 'Proposed $\numofserver \log t/t$-exploration policy'. Adding the word proposed will further avoid confusion about which one of our policy}}
    \label{fig:regret_policies}
\end{figure*}
% -------------------------------------------------------------------

Hence, to bound the expected queue-regret, we need to bound $2$ quantities with high probability, mainly
% \Gauri{Specify the events and lemmas corresponding to each of the items in the following list}
\begin{enumerate}
    \item Length of the busy period of all servers $\left(\eventfive\right)$.
    \item Error in the estimate of $p_i^*$'s $\left(\eventsix\right)$
\end{enumerate}
\Cref{lem:tight_bound_p} and \Cref{lem:final_busy_period} provide bounds on the probability of $\eventsix$ and $\eventfive$ respectively.
% \begin{enumerate}
%     \item Length of the busy period $\left(\eventfive\right)$.  %\Gauri{Space before brackets} \Tuhin{Changed.} 
%     This is small if 
%      \begin{enumerate}
%          \item arrival rate of jobs in queues is less than the departure rate - Proved in \Cref{lem:p_wt}.
%          \item queue length is not too large at later stages - Proved in \Cref{lem:bound_q_length}, \Cref{lem:bound_busy_period_1} and \Cref{lem:tighter_queue_length}.
%      \end{enumerate}
%     \item %\Gauri{Space before brackets} \Tuhin{Changed.}
%     Number of false exploitations in a busy period $\left(\eventfive, \eventsix\right)$ - This is small if
%          \begin{enumerate}
%              \item the estimate $\hat{p}_i(t)$ is close to $p_i^*$ - Proved in \Cref{lem:tight_bound_p}.
%              \item To show the convergence of the estimate, we need the number of arrivals to queue $i$ to be linear in time $t$ which is true if arrival rate of jobs into queues is at least some positive constant - Proved in \Cref{lem:p_wt}.
%          \end{enumerate}
% \end{enumerate}
Define 
\begin{equation}\label{eq:t_0}
    \begin{multlined}
        t_0 = \inf_\tau \Bigg\{\tau \in \mathbb{R}:\frac{\lambda \ln w(\tau)}{w(\tau)} \leq \min_i\frac{\freecapacity_i}{4},  \min_i \freecapacity_{i} w(\tau) \geq 48 \ln \tau, \\
        \max_i \frac{66 \ln \tau}{\freecapacity_i^2} + \frac{10 \ln \tau}{ \freecapacity_i} \leq \frac{\tau}{2} , 42\leq w(\tau) \leq \frac{\tau}{4},\\
        \min_i\frac{\mu_i w(\tau)}{2} \geq\frac{4\ln \tau}{c_g \Delta_0^2}  + \sqrt{2w(\tau)\ln t} , \frac{k_1}{c}\sqrt{\frac{\ln\tau/2}{\tau/2}} \leq \Delta,\\
        \frac{2}{9} w(\tau) \geq 4 \ln \tau, \frac{32 w(\tau)}{3} \leq \frac{\tau}{4} \Bigg\},
    \end{multlined}
\end{equation}
where
\begin{equation}\label{eq:w(t)}
    w(\tau) = 2\exp\left(\frac{1}{\Delta_0}\sqrt{\frac{16 \ln \tau}{c_g\lambda}}\right)
\end{equation}
and $\Delta_0$ and $\Delta$ are constants depending on system parameters given by 
\begin{equation}\label{eq:delta0}
    \Delta_0 = \min\left\{\Delta, \min_i\{\mu_i(1 - \mu_i)\}, \frac{\min_{i:p_i^* > 0}p_i^*}{3c}, \sqrt{\frac{\freecapacity_{min}}{3}}\right\},
\end{equation}
\begin{equation}\label{eq:delta)}
    \Delta = \min \left\{\frac{\tilde{\mu}}{2}, \frac{\freecapacity_{min}}{||\support(\bm{\mu}, \lambda)||_1}, \frac{\freecapacity_{min}}{2c\lambda}, \Delta_{support}\right\},
\end{equation}
  and $\tilde{\mu} = \min_i \{\min \{\mu_i, 1- \mu_i\}\}, \freecapacity_{min} = \min_i \freecapacity_i$, and $\Delta_{support}$, the \textit{tolerance gap} of the system, is given by,
\begin{equation}\label{def_optimal_support_set}
\begin{split}
     \Delta_{support} = \sup \Big\{\delta \geq 0 \>:\>\support\left(\boldsymbol{\mu} - \boldsymbol{\kappa}, \lambda\right) = \support(\bm{\mu}, \lambda),\\
     \>\forall \boldsymbol{\kappa} \mbox{ s.t. } \left|\left|\boldsymbol{\kappa}\right|\right|_{\infty}\leq \delta\Big\}.   
\end{split}
\end{equation}
% \Gauri{We used $\freecapacity_i$ already to denote $\mu_i - \lambda p_i^*$. These $\freecapacity$'s are different from that, right?}
% \Tuhinrevise{\eqref{def_optimal_support_set} implies that if $\left|\left|\hat{\bm{\mu}}(t) - \bm{\mu}\right|\right|_\infty \leq \Delta_{support}$ then $\hat{\support}(t) = \support$. Intuitively, $\Delta_{support}$ denotes the maximum error that is allowed in the estimate of service rate vectors that still allows the use of servers in the optimal support set.}. %\Weina{8/3: $\Delta_0$ and $\Delta$ haven't been introduced yet.} \Tuhin{Changed.} 
% For the above lemma to hold, we need at least $\order(t)$ number of departure of jobs from each server. For this we want our arrival rate of jobs into each queue to be some positive constant. \Cref{lem:p_wt} will show that the queue $i$ will see arrival rate of some positive constant. Meanwhile, to upper bound the expected regret, we showed that we need to bound the length of busy cycle as seen at time $t$. \Cref{lem:final_busy_period} given below gives a bound on the probability that the busy period length exceeds a certain quantity.
\begin{lem}
\label{lem:final_busy_period}
For the event $\eventfive := \left\{\busy_i(t) \leq v_i(t) \triangleq \frac{66\ln t}{\freecapacity_{i}^2},\> \forall i\right\}$ about the busy period length $\busy_i(t)$, as defined in \eqref{eqn:event5}, we have
\begin{equation}
    \probability\left(\eventfive^c\right) \leq \numofserver\left( \frac{8}{t^{7}} + \frac{4k_2}{t^3} + \frac{5}{t^4}\right)
\end{equation}
%\Gauri{I repeated the definition of $\eventfive$ above to avoid making readers go back to find it}
%\Tuhin{Sounds good.}
for any $t \geq t_0$ with $t_0$ defined in \eqref{eq:t_0}. %\Gauri{When you mention $t_0$, please cite the equation where you defined it}
%\Tuhin{Done}
\end{lem}
\begin{proof}
    Given in Appendix \ref{prf_lem:final_busy_period}.
\end{proof}
\begin{lem}
For the event 
\begin{equation}
    \eventsix := \left\{\left| \hat{p}_i(\tau) - p_i^*\right| \leq k_1\min\left\{\sqrt{\frac{ \ln t}{t}}, p_i^*\right\},\>\> \forall i , \>\forall \tau \in \left[\frac{t}{2}, t\right]\right\}
\end{equation}
about the estimation error of $\hat{p}_i(t)$'s, as defined in \eqref{eqn:event6}, we have
\label{lem:tight_bound_p} 
\begin{equation}
\begin{split}
     \probability\left(\eventsix^c\right) \leq \numofserver\left(\frac{1}{t^7} + \frac{k_2}{t^3}\right) +\sum_{i: p_i^*>0}\Bigg(\frac{1}{t^3} + t \exp\left(-\frac{p_i^*\lambda t}{128}\right) + \\
     t\exp\left(-\frac{\freecapacity_i^2 t}{4}\right)\Bigg)   
\end{split}
\end{equation}
for any $t \geq t_0$ with $t_0$ defined in \eqref{eq:t_0}, and $ k_2 = \frac{1}{1 - \exp\left( -c_g\Delta_0^2 \right)}$.% \Gauri{When you mention $t_0$, please cite the equation where you defined it}
%\Tuhin{Done}
\end{lem}
\begin{proof}
    Given in Appendix \ref{prf_lem:tight_bound_p}.
\end{proof}
%\Gauri{Use the proof environment}
%\Tuhin{Done}
\begin{proof}[Proof of \Cref{thm:main}]
    \begin{align}
        &\expectation\left[\regret_{\policy \policy^*}(t)\right]\\
        = &\sum_{\tau = 1}^t \expectation\left[\regret_{\policy \policy^*}^{inst}(\tau)\right]\\
        =& \sum_{\tau = 1}^{t_0} \expectation\left[\regret_{\policy \policy^*}^{inst}(\tau)\right] + \sum_{\tau = t_0}^t \expectation\left[\regret_{\policy \policy^*}^{inst}(\tau)\right]\\
        \leq &t_0 + \sum_{\tau = t_0}^t \sum_{i=1}^{\numofserver}\frac{132 \ln^2 \tau}{\freecapacity_i^2 \tau} + \sum_{\tau = t_0}^t\sum_{i: p_i^* > 0} k_1 \frac{66\ln \tau}{\freecapacity_i^2}\sqrt{\frac{\ln \tau}{\tau}}  \nonumber\\
        & \qquad + \numofserver\sum_{\tau = t_0}^t \left( \frac{10}{\tau^{6}} + \frac{6k_2}{\tau^2} + \frac{5}{\tau^3}\right)\nonumber\\
        & \qquad + 2\left(\sum_{\tau = t_0}^t\sum_{i: p_i^*>0}\left(\frac{1}{\tau^2} + \tau^2\exp\left(-\frac{p_i^*\lambda \tau}{128}\right) + \tau^2\exp\left(-\frac{\freecapacity_i^2 \tau}{4}\right)\right)\right)\\
        \leq &\sum_{\tau = t_0}^t\left(\sum_{i=1}^{\numofserver}\frac{132 \ln^2 \tau}{\freecapacity_i^2 \tau} + \sum_{i: p_i^* > 0} k_1 \frac{66\ln \tau}{\freecapacity_i^2}\sqrt{\frac{\ln \tau}{\tau}}\right)  + \left(t_0 + \order\left(1\right)\right).
    \end{align}
% Using the \Cref{lem:tight_bound_p} and \Cref{lem:final_busy_period} and \eqref{rel:simplified_final_regret}, for all $t\geq t_0$, we have  
% \begin{equation*}\label{calc:regret_simplification}
%     \regret(t)\leq \sum_{i=1}^{\numofserver}\frac{132 \ln^2 t}{\freecapacity_i^2 t} + \sum_{i: p_i^* > 0} k_1 \frac{66\ln t}{\freecapacity_i^2}\sqrt{\frac{\ln t}{t}}  + \numofserver\left(\frac{9}{t^{6}} + \frac{5k_2}{t^2} + \frac{5}{t^3}\right) + \sum_{i: p_i^*>0}\left(\frac{1}{t^2} + t^2 \exp\left(-\frac{p_i^*\lambda t}{128} + \exp\left(-\frac{\freecapacity_i^2 t}{4}\right)\right)\right)
% \end{equation*}
\end{proof}

Notice, that if the policy is following the optimal weighted random routing policy, then the rate of arrival of jobs in servers, which form the optimal support set, is some positive. So, as the policy emulates the optimal policy better, one would expect $\left(\order\left(t\right)\right)$  number of arrivals in the those servers. Now, the central idea behind \Cref{lem:tight_bound_p} is that if number of arrivals into optimal servers is $\order\left(t\right)$, then error estimate would be in order of $\sqrt{\frac{1}{t}}$ with high probability. Another, idea behind the \Cref{lem:tight_bound_p} is that once the estimates of $\hat{\mu}_i(t)$ is close $\mu_i$, the optimal support vector using the estimates of service rates would coincide with the true optimal support vector $\support$. That would ensure that policy would allocate $0$ probability for the servers which are not in the optimal support set, even though the estimation error of the service rates for these servers is not vanishing at the rate $\order\left(\sqrt{\frac{1}{t}}\right)$. 

Similarly, in the optimal weighted random routing, the queue length process for server $i$ experience a negative drift of $\freecapacity_i$. Recall, $\freecapacity_i = \mu_i - \lambda p_i^*$, was defined as the residual capacity of server $i$. So, the central idea behind \Cref{lem:final_busy_period} is that once the estimates of service rates become better, queue length of process at server $i$ would experience a negative drift of at least $\frac{\freecapacity_i}{2}$ and this would result in a bounded busy period length. 

In short, the key concept behind \Cref{lem:tight_bound_p} and \Cref{lem:final_busy_period} is that as the estimates become better, the policy behaves in some good sense. By good sense, we mean that the policy is ensuring steady rate of arrivals in the servers constituting the optimal support set, diminishing rate of arrival into remaining servers and stabilizing the queue. \Cref{lem:p_wt}, given below, proves that after some time $w(t)$, the system reflects the properties described above and is a key step in proving \Cref{prf_lem:final_busy_period} and \Cref{lem:tight_bound_p}. 


Recall, $\support$ denotes the optimal support set for a system with arrival rate $\lambda$ and departure rate $\bm{\mu} = (\mu_1, \mu_2, \cdots, \mu_\numofserver)$. Since, our policy performs weighted-random routing using the estimates $\hat{\bm{\mu}}(t) = (\hat{\mu}_1(t), \hat{\mu}_2(t), \cdots, \hat{\mu}_\numofserver(t))$, we denote $\support\left(\lambda, \hat{\bm{\mu}}(t)\right)$ as the  \textit{estimated optimal support set} at time $t$. For the ease of notation, we use $\hat{\support}(t)$ to denotes $\support\left(\lambda, \hat{\bm{\mu}}(t)\right)$.
\begin{lem}
\label{lem:p_wt}
Define the event $\eventone$ as 
\begin{equation}\label{event1}
    \eventone := \mathcal{E}_{11} \cap \mathcal{E}_{12}
\end{equation} where
\begin{enumerate}
    \item $\mathcal{E}_{11}:=\left\{\hat{\support}(t) = \support(\bm{\mu}, \lambda),\>\>\forall \tau \in \left[w(t), t\right]\right\}$,
    \item $\mathcal{E}_{12}:= \left\{\frac{\lambda p_i^*}{2} \leq
            \expectation\left(\arrival_i(\tau) \Big| \hat{p}_i(\tau)\right) \leq \mu_i - \frac{\freecapacity_i}{2},\>\>\forall i,\forall \tau \in \left[w(t)), t\right]\right\}$.
\end{enumerate}
% \Weina{What is $\Delta$?}
% \Tuhin{I do not see where it is used. May be because of change in lemma.}
Then, $\forall t\geq t_0$ 
\begin{equation}
    \probability\left(\eventone^c\right)\leq \numofserver\left(\frac{2}{t^{7}} + \frac{k_2}{t^3}\right)
\end{equation}
where $k_2$ is given in \Cref{lem:tight_bound_p}.
\end{lem}
\begin{proof}
    Given in Appendix \ref{prf_lem:p_wt}.
\end{proof}
% For the above lemma to hold, we need at least $\order(t)$ number of departure of jobs from each server. For this we want our arrival rate of jobs into each queue to be some positive constant. \Cref{lem:p_wt} will show that the queue $i$ will see arrival rate of some positive constant. Meanwhile, to upper bound the expected regret, we showed that we need to bound the length of busy cycle as seen at time $t$. \Cref{lem:final_busy_period} given below gives a bound on the probability that the busy period length exceeds a certain quantity. 
%\Weina{Change to a lower-case letter.  It is a good practice to use upper-case letters for random variables and lower-case letters for non-random variables.  You can have exceptions for indexing integers like $K$, $N$, etc.}
%\Tuhin{Changed.}
% \Weina{I suggest that we eliminate the definitions of many of the events and write them out directly.  The number of indexed events is just too large.  It is impossible to memorize the events.  If we do not need to do complicated unions or intersections, we do not need to give the event a symbol.  For example, the following lemma can be rewritten as follows.
% \begin{lem}
% For any $t\ge t_0$ with $t_0$ defined in \eqref{eq:t_0}, it holds that
% \begin{equation}
% \probability\left(Q_i(t - v_i(t)) > q_i \right)\leq \numofserver\left(\frac{6}{t^{7}} + \frac{3k_2}{t^3} + \frac{4}{t^4}\right).
% \end{equation}
% \end{lem}
% Later when you need to use the event $\eventfour$, just write out $Q_i(t - v_i(t)) > q_i$.
% This is just an example and I think we should do this also for at least $\eventfive$, $\eventthree$, $\eventtwo$.  You need to think carefully about which ones to keep and keep as few as possible.}
% \Tuhin{Done. I have kept only the main events, i.e., $\eventone, \eventfive, \eventsix$. $\eventtwo, \eventthree, \eventfour$ are intermediate events and I removed them from the main document. Kept it in the appendix though to simplify the expressions written.}
% From the service times of the departed jobs, the system can learn the $\mu_i$'s. Since $\expectation\left(\hat{\mu}_i(t)\right) \neq \mu_i$ and geometric random variable is unbounded, standard hoeffding bounds cannot be used to bound the estimation error. \Cref{lem:conc_geoemtric} provides a relation to bound the error in the estimate $\hat{\mu}_i(t)$. However, the ultimate goal of the system is to learn $p_i^*$. Since $\hat{p}_i(t)$ is a function of $\hat{\mu}_i(t)$, we want a relation between the estimation error of $\mu_i$ and $p_i^*$ for all $i$. \Cref{lem:relation_p_mu} provides a relation between the estimation error of $\mu_i$ and $p_i^*$ for all $i$. 

==> old/old_files/optimal-weighted-routing.tex <==

%\Gauri{No need to introduce the notation $\mathcal{M}$, directly define $p_i$. Make sure to remove $\mathcal{M}$ from all other places where you have used it in the paper}
%\Tuhin{Corrected.}
%\Weina{Did we agree on ``Weighted Random Routing''?}

%\sout{A policy follows a \textit{weighted routing algorithm} if every incoming job is allocated to one of the servers according to some fixed probability distribution; i.e., every incoming job is sent to server $i$ with probability $p_i$ independent of other jobs, where $p_i$'s satisfy the property $\sum_{j=1}^{\numofserver} p_j=1$. We call the probability vector $\bm{p} = \left(p_1, p_2, \cdots, p_\numofserver \right)$ the \emph{routing vector}. Then, $\left\{\bm{\queue}(t): t\in \mathbb{Z_+}\right\}$ forms a DTMC, where $\bm{\queue}^{\policy}(t) = \left(\queue_1(t), \queue_2(t), \cdots, \queue_\numofserver(t) \right)$.}
%\Gauri{Removing the above paragraph because we already defined weighted random routing in Section 2}

We define \textit{optimal weighted random routing (OWR) policy} as the weighted random routing policy that minimizes the mean response time of jobs in steady state or equivalently, the policy that minimizes the cumulative steady-state queue length $\mathbb{E}[\sum_{i=1}^{\numofserver} Q_i(\infty)]$. Let $\bm{p}^* = \left(p_1^*, p_2^*, \cdots, p_\numofserver^* \right)$ be the routing vector corresponding to the optimal weighted routing policy as a function of arrival rate and the service rates and we will refer to it as the \textit{optimal routing vector}.

For a $Geo/Geo/1$ queueing system with arrival rate $\lambda'$ and departure rate $\mu'$, the expected steady-state queue length, $\expectation\left[\queue(\infty)\right]$, is given by (see \citep{srikant2014communication}~Chapter~3 for the derivation)
\begin{equation}
    \expectation\left[\queue (\infty)\right] = \frac{\lambda'(1-\mu')}{\mu' - \lambda'}.
\end{equation}
Now, for our system with arrival rate $\lambda$ and service rates $\mu_i$'s, if every incoming job is assigned to server $i$ with probability $p_i$, the system can be viewed as $\numofserver$ $Geo/Geo/1$ queues each with arrival rate $p_i\lambda$ and service rate $\mu_i$ respectively. Hence, the steady state queue length of the system is given by
\begin{equation}
    \expectation\left[\sum_{i=1}^{\numofserver}\queue_i(\infty)\right] = \sum_{i=1}^{\numofserver}\expectation\left[\queue_i(\infty)\right] = \sum_{i=1}^{\numofserver} \frac{p_i\lambda(1-\mu_i)}{\mu_i-\lambda p_i}.
\end{equation}
Hence, the optimal routing vector would be the solution to the following optimization problem:
\begin{align}
\min_{p_1, p_2, \cdots, p_\numofserver} \quad &  \sum_{i = 1}^\numofserver \frac{p_i\lambda(1-\mu_i)}{\mu_i-\lambda p_i}\\
\textrm{s.t.} \quad & \sum_{i=1}^{\numofserver} p_i = 1\\
\quad  & p_i \geq 0 , %\> \forall i\\
  \quad  p_i \lambda < \mu_i,  \> \forall i,
\end{align}
%\Tuhin{I did not get what you mean by waterfilling solution.}
where the constraint $p_i \lambda < \mu_i $ ensures stability of the queue $i$ and the remaining constraints ensures that $p_i$ forms a valid routing vector. We show in \secondversion{\Cref{prf_optimal_p}}{\cite{choudhury2020job}} that the optimal routing vector is given by $\bm{p}^* = f(\lambda, \bm{\mu})$, where $f:[0,1]^{\numofserver+1} \rightarrow [0,1]^{\numofserver}$ is a function given by
%\Weina{Change $p^*$ to $p$ in the optimization problem above}
%\Gauri{You haven't defined what the objective of this optimization problem represents -- is it the mean response time, or the sum of the queue lengths?}
%\Gauri{Define $\support(\mathbf{\mu}, \lambda)$ as a function of $\mathbf{\mu}$ and $\lambda$, where $\mathbf{\mu}$ is the vector of service probabilities... and $\lambda$ is the arrival probability...}
%\Gauri{Don't use $\bar{\lambda}$ to denote a scalar. Just $\lambda$}
%\Tuhin{I already used $\lambda$, is it okay to use it once more?}
%\Gauri{Directly define $SUP$ in terms of  $\lambda$ and $\mu$}
\begin{multline}\label{optimal_p}
f(\lambda, \bm{\mu})(i) \\
=  \begin{cases} 
      \frac{\mu_i}{\lambda} - \frac{\sqrt{\mu_i(1-\mu_i)}}{\sum_{j\in \support\left(\lambda,\boldsymbol{\mu}\right)} \sqrt{\mu_j(1-\mu_j)}}\left( \frac{\sum_{j\in \support\left(\lambda,\boldsymbol{\mu}\right)} \mu_j}{\lambda} - 1\right), & \text{if }i\in \support(\lambda, \bm{\mu}), \\
      0, & \text{if }i\notin \support(\lambda, \bm{\mu}). 
   \end{cases}
\end{multline}
where $\support(\lambda, \bm{\mu})$ is a subset of servers which we refer to as the \textit{optimal support set} such that $i\in \support\left(\lambda, \bm{\mu}\right)$ if and only if $p_i^*>0$.

% Define $\support\left(\boldsymbol{\mu}, \lambda\right)$ to be the \textit{optimal support set} such that $i\in \support\left(\boldsymbol{\mu}, \lambda\right)$ if and only if $p_i^*>0$.

In \secondversion{\Cref{prf_optimal_p}}{\cite{choudhury2020job}}, we formally prove that if $\mu_i \geq \mu_j$, then $p_i^* \geq p_j^*$. Therefore, only the slowest servers are excluded from the support set $\support(\lambda, \bm{\mu})$, and the support set has to be $ [1, \dots, i ]$ for some $i \in \{ 1, 2, \dots \numofserver\}$. To find the optimal set $\support(\lambda, \bm{\mu})$ and the optimal routing vector $\bm{p}^*$ we can use the iterative algorithm given below.
%\Gauri{I have changed the support vector to the support set. Please check and update the appendix accordingly}
\begin{enumerate}[label=(\roman*)]\label{algo:find_support}
    \item Initialize the support set $\support(\lambda, \bm{\mu}) = \{1, 2, \dots, \numofserver\}$.
    \item \label{alg:support:2} Calculate $p_i^*$ according to \eqref{optimal_p}.
    \item \label{alg:support:3} If $p_i^* < 0$ for any $i \in \{1, \dots, \numofserver\}$, then remove the slowest server $\arg \min_{i \in \support\left(\lambda,\boldsymbol{\mu}\right)} \mu_i$ from the support set and repeat from Steps \ref{alg:support:2} and \ref{alg:support:3}.
\end{enumerate}
The proof of the correctness of the above algorithm is also given in~\secondversion{\Cref{prf_optimal_p}.}{\cite{choudhury2020job}.} 
%For ease of notation, in the remainder of the paper, we denote $\support\left(\lambda,\boldsymbol{\mu}\right)$ as $\support$ and $\support\left(\lambda, \hat{\bm{\mu}}(t)\right)$ as $\hat{\support}(t)$.

%\Weina{I propose that we don't introduce new notation and just keep $\support\left(\lambda,\boldsymbol{\mu}\right)$ and $\support\left(\lambda, \hat{\bm{\mu}}(t)\right)$, at least in the main body of the paper.}
%\Gauri{That is a good idea. Let me try and make this notation change everywhere in the main paper}
%\Gauri{Add a picture to illustrate the waterfilling solution}
\begin{figure}[t]
    \centering
    \includegraphics[width=75mm]{draft_pics/diagrams/waterfilling.pdf}
    \caption{An illustration of the optimal weighted random routing policy. The job arrival rate is $\lambda$ is split and there are $4$ servers with service rates $\mu_1, \dots, \mu_{4}$ respectively such that $\mu_1\geq \mu_2\geq \mu_3\geq \mu_{4}$.}
    \label{fig:waterfilling_policy}
   % \Gauri{Very nice figure!! Could you please replace 'speed of the server' by 'increasing service rate'?}
\end{figure}


==> old/old_files/optimal_random.tex <==
\section{Optimal Static policy}\label{sec:optimal_randomized_policy}
We consider the class of policies where every incoming job is assigned to server according to some fixed probability distribution.  In other words, for a system with arrival rate and departure rates given by $\lambda$, $\mu_i$'s respectively, consider a distribution $\mathcal{M}\left(\lambda, \mu_1, \mu_2, \cdots, \mu_{\numofserver}\right)$ such that $C\sim \mathcal{M}\left(\lambda, \mu_1, \mu_2, \cdots, \mu_{\numofserver}\right)$ implies
$$C = i \> \> \mbox{with probability } p_i,$$
where $\sum_j p_j = 1.$ Every time a job comes into the system, it is assigned to server $C$, where $C$ is independently sampled from the distribution $\mathcal{M}\left(\lambda, \mu_1, \mu_2, \cdots, \mu_{\numofserver}\right)$. In such a scenario, $p_i^*$ corresponding to the optimal probability distribution $\mathcal{M}^*\left(\lambda, \mu_1, \mu_2, \cdots, \mu_{\numofserver}\right)$ will be the solution to following optimization problem
\begin{align*}
\min_{p_1^*, p_2^*, \cdots, p_\numofserver^*} \quad &  \sum_{i = 1}^\numofserver \frac{p_i^*\lambda(1-\mu_i)}{\mu_i-\lambda p_i^*}\\
\textrm{s.t.} \quad & \sum_i p_i^* = 1\\
\quad &  p_i^* \lambda < \mu_i , \> \forall i\\
  & p_i^* \geq 0 , \> \forall i    \\
\end{align*}
Observe, that the objective function is to minimize the sum of the mean queue length of the system. Minimizing the sum of mean queue length is equivalent to minimizing the mean response time of the server.
\Weina{Change $p^*$ to $p$ in the optimization problem above}
\Gauri{You haven't defined what the objective of this optimization problem represents -- is it the mean response time, or the sum of the queue lengths?}
\Gauri{Define $\support(\mathbf{\mu}, \lambda)$ as a function of $\mathbf{\mu}$ and $\lambda$, where $\mathbf{\mu}$ is the vector of service probabilities... and $\lambda$ is the arrival probability...}
Let $\support$ be a function defined as $\support: (0, 1)^{\numofserver + 1} \rightarrow \{0, 1\}^\numofserver$ such that for any input $X = \{x_1, x_2, \cdots, x_{\numofserver + 1}\} \in \mathbb{R}^{\numofserver + 1}$, $\support(X)$ satisfies the following property.
\begin{enumerate}
    \item Property 1\label{rel:support_monotonic}
    \begin{equation}
        x_i \geq x_j \implies \support(X)_i \geq \support(X)_j,\>\forall i, j \in [1, \cdots, \numofserver]
    \end{equation}
    \item Property 2\label{rel:support_positive}
    \begin{equation}
        \support(X)_i = 1 \implies \frac{x_i}{x_{\numofserver + 1}} - \frac{\sqrt{x_i(1-x_i)}}{\sum_{j:\support(X)_j = 1}\sqrt{x_j(1-x_j)}}\left(\frac{\sum_{} x_j}{x_{\numofserver + 1}} - 1\right) \geq 0
    \end{equation}
    \item Property 3\label{rel:support_maximal}
    \begin{equation}
        \nexists V\in \{0, 1\}^{\numofserver}\mbox{ s.t. }\left|\left| V\right|\right|_1 > \left|\left|\support(X)\right|\right|_1\mbox{ and } V \mbox{satisfy the property \ref{rel:support_monotonic}, \ref{rel:support_positive}.}
    \end{equation}
\end{enumerate}
where $\support(X)_i$ is the $i^{th}$ index of the vector $\support(X)$. It is shown in the Appendix \ref{prf_optimal_p} that the optimal solution to the above optimization problem is given by
\begin{equation}\label{optimal_p}
p_i^* =   \begin{cases} 
      \frac{\mu_i}{\lambda} - \frac{\sqrt{\mu_i(1-\mu_i)}}{\sum_{j\in \support^*} \sqrt{\mu_j}(1-\mu_j)}\left( \frac{\sum_{j\in \support^*} \mu_j}{\lambda} - 1\right) & i\in \support^* \\
      0 & i\notin \support^* 
   \end{cases}
\end{equation}
where $\support^* = \support\left(\mu_1, \mu_2, \cdots, \mu_\numofserver, \lambda\right)$. Here $\support^*$ is defined as the optimal support vector. In other words the optimal policy uses server $i$ iff $\support^*_i =1$. The proof of optimality is given in the Appendix \ref{prf_optimal_p}. The algorithm to find $\support^*$ and $p_i^*$ is given in algorithm \ref{find_support}
% \Gauri{Typo in the above equation -- $\sqrt{\mu}$ should be $\mu$ in the last term}
% \Gauri{There is a chicken-and-egg problem in the above equation -- you need $S^*$ in order to determine $p_i^*$, whereas you need $p_i^*$ in order to determine $S^*$}
% \Tuhin{That is why we need to iterate over all set. Algorithm \ref{find_support} precisely does that.}
%\Gauri{What is $S^*$ in the above equation? Is it supposed to be $\support^*$?}
%\Tuhin{Corrected}
%\Gauri{Do you mean $\support^*$ instead of $\support^*$ here?}
%\Tuhin{Did not understand issue}
\Gauri{Are we going to use these properties later on in the proofs?}

\begin{algorithm}[H]
\caption{Finding the optimal support vector}
% \Gauri{What is $k$ in Line 1?}\Tuhin{I was using the previous version, which had the notation issues. Corrected it.} \Gauri{I don't understand the role of the loop over $i$ here}\Tuhin{Since we assumed initially that $\mu_i$ is monotonically increasing, it means $p_i$ has to monotonically increasing. So at $i^{th}$ step we look at $p_i$ to see if it is negative or not. If it is negative, then $i\notin \support^*$, else $i\in \support^*\implies p_j \geq 0,\> \forall j\geq i \implies$ we found $\support^*$}
\Gauri{We discussed during a previous meeting that we should come up with a way to avoid writing an algorithm to find the optimal support vector.}
\label{find_support}
\begin{algorithmic}[1]
\State Initialize $\support^*_i = 1, \> \forall i$
\For{$i\in \{1,2,\cdots, \numofserver - 1\}$}
\For{$j\in \{1,2,\cdots, \numofserver\}$}
\If{$j\in \support^*$}
\State $p_j^* = \frac{\mu_j}{\lambda} - \frac{\sqrt{\mu_j(1- \mu_j)}}{\sum_{k: \support_k^* = 1} \sqrt{\mu_k(1-\mu_k)}}\left(\frac{\sum_{k: \support_k^* = 1} \sqrt{\mu_k}}{\lambda} - 1\right)$ 
\Else
\State $p_j^* = 0$ 
\EndIf
\EndFor
\State $\hat{i} = \argmin_i \mu_i,\> s.t. \> \support_i^* = 1$
\If{$p_{\hat{i}}\geq 0$}
\State Break
\Else
\State $\support_{\hat{i}}^*  = 0$ 
\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}
Since, the above algorithm finds a distribution for which the queues are stable. We can find $\epsilon_i> 0$, for all $i$ satisfying $\support_i^* = 1$ such that $\epsilon_i = \mu_i - \lambda p_i^*$
\subsection{Properties of Optimal policy}
\Gauri{Are we going to use these properties later on in the proofs?}

\begin{enumerate}
    \item \textbf{Scale Invariance:} Replacing $\lambda, \mu_1, \cdots\mu_k$ with $c\lambda, c\mu_1, \cdots c\mu_k, \> c > 0$ does not change $B^*$
    \item \textbf{Monotonocity: }
    \begin{itemize}
        \item $\mu_i \geq \mu_j \implies p_i^* \geq p_j^*, \> \forall i, j$
        \item $\mu_j = \mu_j', \> \forall j\neq i$, then $\mu_i \geq \mu_i' \implies p_i^* \geq p_i^{*'}$ and $\mu_i \leq \mu_i' \implies p_i^* \leq p_i^{*'}$
        \item $\mu_j = \mu_j', \> \forall j\neq i$, then $\mu_i \geq \mu_i' \implies p_j^* \leq p_j^{*'}$ and $\mu_i \leq \mu_i' \implies p_j^* \leq p_j^{*'}, \> \forall j\neq i$
    \end{itemize}
\end{enumerate}

==> old/old_files/problem_setup.tex <==
\section{Problem Setup} \label{sec prob}
%\Gauri{You are using $k$ to denote the number of servers here, and the notation is changed to $K$ later on. Please define a macro to make it easier to change the notation later, as Weina also suggested}
In this section,  we will formally define the problem. We consider the multi-server model on a discrete-time system. There are $\numofserver$ servers and queues assigned to each server. Let $\queue_i(t)$ represents queue size at server $i$ at time $t$. We assume $\queue_i(0) = 0, \> \forall i$ i.e the system starts with empty queues. At each time $t$, a job arrive at the system according to a Bernoulli random variable with parameter $\lambda$. We also assume that $\lambda < \sum_i \mu_i$ for the system to be stable. Every time a job arrives, the system assign the job to a server according to some policy $\policy$. The decision of policy $\policy$ can depend on the present and past state of the system. Service time for jobs in server $i$ are independently sampled from a geometric random variable with success probability $\mu_i$, independent of any previous sample. Without loss of generality, assume that $\mu_i \geq \mu_j, \forall i < j$, i.e. server $1$ is the fastest server while, server $\numofserver$ is the slowest server on average. \Gauri{Don't say that without loss of generality the servers are ordered. We consider the ordering only to find the static optimal policy, not in the bandit policy or when you are coupling. When you find the static optimal policy, you can use denote the ordered service rates as $\mu_{(1)} \geq \mu_{(2)} \geq \dots \geq \mu_{(k)}$ to distinguish them from $\mu_1$, $\mu_2$, \dots $\mu_k$, which need not be ordered}  We assume a non-preemptive FCFS scheduling policy for each queue i.e. service of a job will start when all jobs ahead of it are serviced. Initially, the system, does not know $\mu_i$'s, however it can learn about the rates as more and more job departs from the system. Every time a job departs from server $i$, the system gets the service time of the job and it can use that to estimate  the parameter $\mu_i$. Let $X_1, X_2, \cdots, X_n$ be the service time of the $n$ jobs departed from server $i$ so far. Then, the estimate $\hat{\mu}_i$ of $\mu_i$ can be estimated as 
\begin{equation}
    \hat{\mu}_i = \frac{n}{\sum_{j=1}^n X_j}
\end{equation}
\Gauri{Whenever you write $\hat{\mu}_i$, I suggest always adding an index $t$ to denote the time at which it is calculated, or $n$ to denote the number of samples used to calculate this estimate. }
\Weina{Do not use $i$ both as the subscript for the estimate and the dummy variable for the sum.  Also please write out the range of the sum.  You can omit the range of the sum later when it is totally clear from the context, say, in the middle of a proof after you write the sum many times.}
As our estimates of $\mu_i$'s become better, we should be able to make a more informed decision. Our aim is to minimize the expected queue length. Consider a policy $\policy^*$, which is the optimal algorithm to minimize the expected queue length. We define regret $\regret(t)$ as 
\begin{equation}
    \regret(t) = \expectation\left(\sum_{i=1}^\numofserver \left[\queue_i(t) - \queue_i^*(t)\right]\right),
\end{equation}
\Gauri{Why are we using instantaneous regret and not cumulative regret?}
\Weina{Write out the range of the summation.  Add subscript to $\queue^*$.  Fix the punctuation throughout the paper.}
where $\queue_i^*(t)$ is the queue length of server $i$ at time $t$, when following the optimal policy $\policy^*$. One can understand regret as the expected penalty received because of not following the optimal policy. Since, $\policy^*$ is optimal, minimizing  expected queue length is equivalent to minimize  the $\regret(t)$.
% \Gauri{Need to define the performance metric of interest}

==> old/old_files/staticvsdynamic.tex <==
\section{Consideration of static policies}
% \Gauri{Formulate the search for the static policy as an optimization problem in terms of the performance metric defined in the problem setup section, and show the derivation of $p_i^*$ here}
We define a policy $\policy^*$ to be \textbf{optimal} if for all other policy $\policy$,
$$\expectation\left[\sum_{i=1}^{\numofserver} \queue_i^*(\infty)\right] \leq \expectation \left[\sum_{i=1}^{\numofserver} Q_i (\infty)\right]$$
Consider a system where the policy has the knowledge of $\lambda$ and $\mu_i$ for all $i$. Any such policy can be categorized into class of two policies given as:
\begin{itemize}
    \item Dynamic: Assignment of jobs to server $i$ at time $t$ depends on $\queue_i(t)$
    \item Static: Assignment of jobs to server $i$ at time $t$ is independent of $\queue_i(t)$
\end{itemize}
\Weina{You have used $\queue^*$ to differentiate the queue lengths under the optimal policy from those under other policies.  You need to stick to that notation instead of putting the policies as subscripts of the expectations.}
The simplest example of a dynamic policy is JSQ (Join the shortest queue), where the incoming job is pushed to the server with the smallest queue. Intuitively, at any point in time the dynamic policy can do at-least as good as the static policy, the mean queue length for dynamic policy is usually better as compared to static polices.
\begin{figure}[H]
    \centering
    \includegraphics[scale = 0.5]{plots/plot_condor2.pdf}
    \caption{Response time for various policies}
    \label{fig:rt_policy}
\end{figure}
Figure \ref{fig:rt_policy} shows the response time of the system according to various dynamic and static policies. One can clearly observe that the dynamic policies outperform the static policies by huge margin. By little's law, one can also argue that a system which minimizes the mean response time, also minimizes the mean queue length. However, a major issue with dealing in dynamic policies is that the state space is very complicated. Hence, it is difficult to solve the system, and only numerical approximation exists. Even in the simplest case of JSQ, the mean response time of the system is not known, though some close approximation exists. Since, we are dealing with bandit version of queueing policies, it can be expected that solving a bandit version of a dynamic policy would be more difficult. Also, difficulty in solving the system for a dynamic policy makes it harder to prove optimality for any policy. Hence, for the ease of solving we will consider on static policies as of now.

==> old/old_files2/algorithm.tex <==
\section{Proposed Job Dispatching Policy For Unknown Service Rates}
\label{sec:algorithm}

Recall that we consider a dispatcher who does not know the service rate vector $\bm{\mu}=(\mu_1,\dots,\mu_{\numofserver})$ and thus relies on the estimated service rate vector $\bm{\hat{\mu}}(t)=\left(\hat{\mu}_1(t),\dots,\hat{\mu}_{\numofserver}(t)\right)$. Our goal is to design a dispatching policy $\policy$ that minimizes the expected regret $\mathbb{E}\left[\regret_{\policy \policy^*}(t)\right]$ with respect to the optimal weighted random routing policy $\policy^*$. 

In order to asymptotically converge to $\policy^*$, it is important for the dispatching policy to correctly identify the optimal support set $\support(\lambda,\bm{\mu})$ for which $p_i^* > 0$. If a server with $p_i^* > 0$ is excluded from the estimated support set, then the dispatcher will not send any jobs to it and hence cannot converge to the optimal policy $\policy^*$. In this section we first demonstrate that it is necessary to explore (that is, send jobs to all $\numofserver$ servers) infinitely often for achieving a reasonable regret in Section~\ref{subsec:exploration}. We then present our policy in Section~\ref{subsec:algorithm}.
%% May want to change $\support$ to $\support\left(\lambda,\boldsymbol{\mu}\right)$

\subsection{The Necessity of Exploration}\label{subsec:exploration}
It is well-known that for stochastic multi-armed bandits problems, it is necessary to explore infinitely often to achieve an optimal regret.  Interestingly, there are recent results showing that no explicit exploration is needed for achieving an optimal regret in some queueing systems with unknown parameters \citep{krishnasamy2018learningcu}. There the exploration comes for free when running a stabilizing policy.  However, for the job dispatching problem we consider in this paper, we demonstrate below that infinitely often exploration is still necessary.

A naive dispatching policy may dedicate a constant amount of time at the beginning to exploration to obtain a good estimate of the service rate vector.  Then after the initial exploration phase, the policy uses the estimate $\hat{\bm{\mu}}(t)$ at every time slot $t$ to compute the routing vector and dispatches arriving jobs accordingly, while keeping updating the estimate $\hat{\bm{\mu}}(t)$ using the service times of completed jobs.  We will construct an example to demonstrate that this can lead to a situation where a server in the optimal support set $\support(\lambda,\bm{\mu})$ is forever excluded from the estimated optimal set, which will incur a linear regret.

% \sout{Now, a naive dispatching policy may use the estimate $\hat{\bm{\mu}}(t)$ at every time to compute the routing vector and assign \sout{the}\Weinarevise{an arriving} job to \sout{different}\Weinarevise{one of the} servers accordingly. However, this can lead to a situation where an optimal server is not included in the support vector because of bad estimation. The best way to get over this issue is to force \textit{exploration} of the servers, where the policy ensures that it has sufficient samples of service times from each server before rejecting it. One way to do this is given as follows:}
% \Weina{Just a comment: you wrote ``the best way to get over this issue...'', but what you described below is not the best way to get over this issue.}


% \sout{However, this type of policy is also not enough to ensure that the policy achieves a sub-linear regret w.r.t. time. Consider the example given below that illustrates the issue of this type of policy. }

Consider a two-server system with $\lambda = 0.05$ and  $\bm{\mu} = (0.5, 0.5)$. One can verify that the optimal routing vector is $\left(0.5, 0.5\right)$. Suppose for the first $n$ time slots, the dispatching policy assigns an arriving job to one of the two servers chosen uniformly at random. We consider an event $\mathcal{E}$ defined by the scenario below. 

Suppose that there are $k$ job arrivals during the first $n$ time slots to server $1$. Let $t'$ be the earliest time by which all the $k$ %\sout{jobs within the first $n$} 
jobs that are assigned to server~$1$ have departed. Then we consider the scenario where
the estimated service rates satisfy that $\hat{\mu}_1(t) \leq 0.1$ for all time $t$ with $t\le t'$ and $\hat{\mu}_2(t) \geq 0.2$ for all time $t$. 


We first argue that under the event $\mathcal{E}$, the regret scales linearly with time.
Note that under $\mathcal{E}$, for any time $t$ with $n<t\le t'$, the routing vector is $(0,1)$ since $\hat{\mu}_1(t) \leq 0.1$ and $\hat{\mu}_2(t) \geq 0.2$. 
At time $t=t'+1$, we still have that $\hat{\mu}_1(t) \leq 0.1$ since no new job is sent to server~$1$ and that $\hat{\mu}_2(t) \geq 0.2$ by the definition of event $\mathcal{E}$, which makes the routing vector remain $(0,1)$.  Repeating this argument for all the time slots after $t'+1$ we can see that for rest of the time no job will be sent to server~$1$ at all. Now the expected steady-state queue length when using only server $2$ is $1/18$, while the expected steady-state queue length using the optimal routing vector is $1/19$. Thus the regret scales roughly as $t/342$, which is linear in $t$.


We next show that the event $\mathcal{E}$ happens with a strictly positive probability:
    % \Weina{The hat symbol should only be over $\mu$}
    \begin{align}
        %\probability(\mathcal{E}) &\geq \left(\sum_{k = 1}^n {n \choose k}(0.5)^n \left((0.5)^{10}\right)^k\right) \probability\left(\cap_{t = 1}^{\infty}\left\{\hat{\mu}_2(t) \geq 0.2\right\}\right)\\
        \probability(\mathcal{E}) &= \left(\sum_{k = 1}^n {n \choose k}(0.5\lambda)^n \probability\left(\substack{\text{all $k$ jobs to server $1$}\\ \text{have service time $\ge 10$}}\right)\right)\nonumber\\
        &\mspace{23mu}\cdot\probability\left(\cap_{t = 1}^{\infty}\left\{\hat{\mu}_2(t) \geq 0.2\right\}\right)\\
        &\geq \left(1 -  \sum_{t = 1}^{\infty}\probability\left(\hat{\mu}_2(t) < 0.2\right)\right) \sum_{k = 1}^n {n \choose k}(0.5\lambda)^n \left((0.5)^{10}\right)^k\\
        &\geq \frac{1}{3} \sum_{k = 1}^n {n \choose k}(0.5\lambda)^n \left((0.5)^{10}\right)^k\label{eq:counter_example},
    \end{align}
which is strictly positive, where \eqref{eq:counter_example} is due to Chernoff bound.
% \Weina{Question: should this probability be multiplied by $\lambda^n$?  Is the first inequality supposed to be equality?}
% \Weina{Question: should we mention Sanjay's paper where no exploration is needed?}

% \Weina{Can you give a short, clear argument on why this gives a linear regret?}

\subsection{An \texorpdfstring{$\epsilon_t$}{et}-Exploration Policy}
\label{subsec:algorithm}

%\sout{Hence, one would like never to stop exploration, but reduce the amount of exploration over time. This is to ensure that one does not overdo exploration, which would also lead to a higher regret.}

As demonstrated in Section~\ref{subsec:exploration},
exploring for a fixed amount of time can lead to a linear regret. To ensure enough exploration, we propose an $\epsilon_t$-exploration policy, which explores with probability $\epsilon_t = \frac{\numofserver \ln t}{t}$ at each time slot $t$. When not exploring, the policy treats the estimated service rates as if they were the actual service rates and calculates the optimal routing probabilities based on them; i.e., when not exploring, the policy uses $\hat{\bm{p}}(t) = (\hat{p}_1(t), \hat{p}_2(t), \cdots, \hat{p}_\numofserver(t))$ to make a routing decision at time $t$. The pseudo-code is presented in~\Cref{poli:bandit}.
%
%In \Cref{sec:simulation} we compare this policy with variants of upper confidence bound (UCB) and Thompson sampling (TS). 
%\sout{One way to do this is to use the $\mathcal{E}(t)$-greedy exploration strategy, which decides to explore at time $t$ with probability $\mathcal{E}(t)$. $\mathcal{E}(t)$ is chosen in a way such that the exploration probability goes to zero as $t$ goes to infinity. Based on the above idea, we propose an algorithm given in %\Cref{algo:bandit}.}



% We now assume that our class of policy is restricted only to randomized policy. In other words, we want our bandit algorithm to learn optimum randomized policy given in Section \ref{sec:optimal_randomized_policy}. Hence, our aim is to minimize the regret given by 
% \begin{equation}
%     \regret(t) = \expectation\left(\sum_i \left[\queue_i(t) - \queue^*(t)\right]\right)
% \end{equation}
% where $\queue_i(t)$ and $\queue_i^*(t)$ are the queue length at server $i$ at time $t$ using the bandit policy and optimal randomized algorithm.

% Since, in the beginning the user has no information about the true values of $\mu_i$, the system will have do some exploration to learn the values of $\mu_i$. Every time a job departs from server $i$, the user learns the time taken by the job from server $i$. Since at every time slot,  the departure from a server is decided according to an i.i.d. Bernoulli random variable with parameter $\mu_i$, the service time is distributed according to a geometric random variable. As more and more jobs leave from server $i$, the user can estimate the success probability of server $i$, $\hat{\mu}_i = \frac{n}{\sum_j X_{ij}}$, where $X_{ij}$ is the service time of $j^{th}$ job departing from server $i$.  Define $\hat{\mu}_i(t)$ to be the estimate of $\mu_i$ at time $t$. As, more jobs departs from server $i$, $\hat{\mu}_i(t)$ becomes closer and closer to $\mu_i$, and user have more information about the system. So, in the later stages, the user should exploit the knowledge of the system and explore less often. To maintain a balance between exploration and exploitation, we follow an $\epsilon(t)$ - greedy bandit policy, where at each time $t$, the user decides to explore with probability $\epsilon(t)$ where $\epsilon(t)\rightarrow 0$ as $t\rightarrow \infty$. So, at each time $t$, if the user chooses to explore, it sends any incoming to job to any server at random. However, if the user decides to exploit, it sends the job to server $i$ using the optimal  randomized allocation using the estimates.
% We propose \Cref{algo:bandit} and prove that our algorithm achieves $\order\left(\frac{\left(\ln t\right)^{\frac{3}{2}}}{\sqrt{t}}\right)$.
\begin{algorithm}[t]
\caption{%Bandit algorithm
An $\epsilon_t$-Exploration Policy for Learning Optimal Weighted Random Routing}
\label{poli:bandit}
\begin{algorithmic}[1]
\While{$t\geq 0$}
\If{\mbox{a job arrives}}
\State $\explorerandom(t)\gets$a Bernoulli sample with mean $\min\left\{1, \frac{K\ln t}{t}\right\}$
\If{$\explorerandom(t) = 1$}
\Comment{Explore}
\State{Dispatch to one of the servers uniformly at random}
\Else
\Comment{Exploit}
\State{Compute routing vector $\hat{\bm{p}}(t) = f(\lambda, \hat{\bm{\mu}}(t))$}
\State{Dispatch to server $i$ with probability $\hat{p}_i(t)$
%$\hat{p}_i(t)$ where $\hat{p}_i(t)$'s are  optimal probabilities calculated using \eqref{optimal_p} with parameters $\lambda$ and $\hat{\mu}_i(t)$'s
}
%\Gauri{Remove $M^*$ from here}
%\Tuhin{Though I removed it, the current algorithm looks stranger. It might be better to define the optimal categorical distribution $\mathcal{M}^*$ for any given $\lambda$ and $\boldsymbol{\mu}$. Let me know what you think!}
\EndIf
\EndIf
\For{$i = 1, 2, \cdots K$}
\If{\mbox{a job departs from server $i$}}
\State {Update $\hat{\mu}_i(t)$ using \eqref{eqn:mu_estimate}}
\EndIf
\EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}

%\Gauri{I suggest adding some discussion here qualitatively comparing the proposed policy with the variants of UCB and Thompson sampling applied to queueing bandits}

==> old/old_files2/conclusion.tex <==
\section{Concluding Remarks}
In this paper, we study the problem of job dispatching policies in a system with unknown service rates and unknown queue length information. We propose a bandit-based $K \ln t/t$-exploration policy, which uses online estimate of the service rates to dispatch jobs, and asymptotically converges to the optimal weighted random (OWR) routing policy. We characterize the finite-time regret of this policy and present simulation results to demonstrate that it performs well in all load regimes. % as compared to other bandit-based dispatching policies. 

% Since this is one of the few works applying bandit algorithms to job dispatching in queueing systems, 
There are substantial open directions for future work. 
%
An immediate open challenge is to prove a matching lower bound on the regret. Unlike typical bandit problem where every wrong decision incurs a penalty, characterization of this penalty is difficult in our queueing setting. % Any policy which is optimal in the steady-state might not be optimal at every individual state. As a result of which any sub-optimal policy might outperform the optimal policy in particular states. For e.g., in a $2$ server system with $\lambda = 0.5$ and $\bm{\mu} = (0.5, 0.5)$, the optimal routing vector is $(0.5, 0.5)$. However, if the current queue length is $\bm{\queue} = (2, 7)$, any routing vector which has more weight for the first server will outperform the OWR for that state.
%
Another open direction is extending the work to characterize of regret for classes of policies that has access to the queue length information like JSQ, SED etc. The analysis of these policies is far more complicated than random routing policies, where the difference in the queue length can be characterized by the difference in the routing probabilities.%, the evolution of queues in policies, that uses queue length to dispatch jobs, is far more complicated.

%\Gauri{I suggest shifting the paragraph below to the end of the regret analysis section rather than highlighting it in the conclusion}
%\sout{Finally, our proof technique used the absolute difference in the routing probabilities to analyze the difference in queue length. However, a tighter regret upper bound might be proved by considering the actual difference in routing probabilities. But the analysis has to handle the dependencies between the busy period and routing decision of the algorithm.}

==> old/old_files2/intro.tex <==
\section{Introduction}
\label{sec:intro}

%\Gauri{Don't we have to list the authors' email IDs somewhere in the template?}

%\Gauri{If you have some other candidate paper titles in mind, please add them to the comments below}
%\title{Scheduling to Queues with Unknown Service Rates using Bandit Exploration}
%\title{Bandit-based Scheduling Algorithms for Multi-server Queueing Systems}
% \title{Job Dispatching Policies for Queueing Systems with Unknown Service Rates}

%\Gauri{Proposed Outline for the Introduction: 1) Scheduling in Queueing Systems and the standard assumption that service rates are known. 2) In practice (in data-center computing or crowdsourcing appllications), the service rates may be unknown or time-varying, which precludes the use of traditional scheduling policies, 3) Bandit algorithms are suitable for this problem of simultaneously estimating the service rates and scheduling jobs. However very few works have explored this intersection of online learning and scheduling. Add a review of previous works here. 4) Summarize the contributions of our paper along with stating the organization.}

%Multi-arm bandit and Queueing theory have been one of the most extensively researched areas over the last century. The traditional queueing problem studied the relation of system metrics like response time and expected queue length concerning server speed and job arrival rate. Change in the metrics is also studied w.r.t scheduling of jobs. However, in most of the settings, people assumed that they have full knowledge about the system, i.e., service time and job arrival rate are known. These assumptions simplify the system by a great extent. However, in real life, it is difficult to know the parameters beforehand. The problem studied in this paper is an example of such a case. 
% \Weina{Do not use line break at the end of a paragraph.}

%\textbf{Job Dispatching in Multi-server Systems.} 
Traditional queueing models \citep{mor_book, srikant2014communication} such as M/M/1, M/G/k, G/G/k consist of a single central queue holding incoming jobs and one or more servers that are used to serve those jobs. However, in many applications such as supermarket or airport queues, it is more practical for each server to maintain a separate queue consisting of jobs that are assigned to it. This paradigm calls for the design of job dispatching policies such as join-the-shortest queue (JSQ), shortest expected delay (SED) and least-work-left (LWL) that seek to emulate the delay performance of systems with a single central queue by making the most efficient assignments of jobs to server queues. For example, the JSQ dispatching policy polls the queue lengths at the servers and assigns each job to the shortest queue. In large-scale systems such as computing clusters with tens of thousands of servers, an important consideration is that it can be practically infeasible to poll and maintain status information of all the queues. Therefore, alternatives to join-the-shortest-queue such as the power-of-$d$-choices (Po$d$) policy \citep{mitzenmacher1996load, mitzenmacher2001power, vvedenskaya1996queueing} obtain queue length information of only a randomly chosen subset of servers in order to reduce the communication and memory cost.

A common assumption in all the the policies described above is that the service rates at which jobs assigned to each server are served are known to the job dispatcher, or are to be homogeneous across servers, which precludes the need for the dispatcher to know them. In emerging applications such as cloud computing and crowd-sourcing, the servers may not be dedicated to jobs assigned by the dispatcher and may encounter interruptions and service slowdown due to background workload. Therefore, the service rate experienced by the assigned jobs can be unknown, highly variable across servers, and also changing over time. Traditional service-rate-agnostic policies are not effective in such systems and service-rate-aware policies such as join-the-fastest-shortest-queue (JFSQ) cannot be used due to the service rates being unknown.

\subsection{Main Contributions and Organization} In this paper, we propose a job dispatching policy that learns the unknown service rates of the servers, while simultaneously seeking to minimize the queueing delay experienced by jobs. This problem is at the %scarcely explored 
intersection of queueing systems and online learning. It sheds light on a novel exploration-exploitation trade-off where the job dispatching policy needs to strike a balance between assigning jobs to all servers in order to better estimate their service rates (exploration) and preferentially sending jobs to the faster servers to minimize the queueing delay experienced by jobs (exploitation).

%%Weina's revision
Unlike classic multi-armed bandits (MABs) where only one of the actions is optimal, in the queueing setting considered in this paper, an optimal policy would typically use several fast servers.  Therefore, it is necessary to perform exploration in order to identify the subset of servers that should continue receiving jobs asymptotically.  However, more importantly, only identifying this optimal subset of servers is \emph{not enough} for learning an optimal job dispatching policy.  We need to also accurately estimate the service rates of servers in this subset.
Interestingly, we are able to achieve this by virtue of some special properties of queueing systems. 
%This illustrates an interesting phenomenon in the considered queueing setting: exploration and exploitation can happen simultaneously.
In particular, after we identify the optimal subset of servers, we exploit by dispatching jobs only to this subset of servers.  But meanwhile, since we keep obtaining service time samples from the jobs dispatched to these servers, we also continue to improve the learning accuracy of the service rates.  Therefore, exploitation and improvement in estimation are taking place simultaneously in this queueing system.
%The fractions of jobs we dispatch to each server can be suboptimal due to the inaccuracy in the learnt service rates.  But even with the suboptimal fractions, we still dispatch jobs to all servers in this subset and thus keep obtaining service time samples to improve the learning accuracy of service rates.

The rest of the paper is organized as follows. In \Cref{sec:prob_formu} we describe the system model and formulate the problem concretely. In \Cref{sec:optimal_randomized_policy}, we find the optimal weighted random routing policy, which serves as the performance baseline. In \Cref{sec:algorithm} we propose a bandit-based $\epsilon_t$-exploration algorithm. The distinction between multi-armed bandits and our queueing setting leads to very different regret analysis, presented in \Cref{sec:regret_analysis}.
%Unlike classic multi-armed bandits (MABs) where only one of the actions is optimal and pure exploitation policies will always choose that action, in the queueing setting considered in this paper, a pure exploitation policy would typically use several fast servers, and thus implicitly perform some exploration. However, in \Cref{sec:algorithm}, we show that in regimes where there is a significant gap between the service rates of the fastest and slowest servers, it is indeed necessary to perform exploration in order to identify the subset of servers that should continue receiving jobs asymptotically. We then propose the $\epsilon_t$-exploration dispatching policy.
%In \Cref{sec:regret_analysis} we provide a regret upper bound, and 
In \Cref{sec:simulation} we demonstrate the effectiveness of the proposed policy via simulations. \secondversion{ }{Due to lack of space, we mainly present proof sketches here, and provide the full proofs in the technical report  \citep{choudhury2020job} available online.} 

\subsection{Related Work}
Bandits have had a rich history, both from an optimal control perspective (see \cite{mate08} for a survey) and a finite-time regret perspective (see \cite{lattimoreszepesvari2020banditbook} for a survey). Our paper focuses on bandits in queueing settings -- while this intersection has had a rich history (starting from the Klimov's model \cite{kli74} focusing on optimal control), our focus is on a finite-time regret formulation. At a high-level, the regret perspective formulates queueing problems with unknown statistics (e.g., of the service or arrival processes), with the goal of characterizing the loss/regret in performance of a resource allocation (with learning) algorithm with respect to a genie-policy that has access to the complete statistics. Such regret formulations have recently been introduced both in the adversarial setting \cite{walton13} and the stochastic setting \cite{krishnasamy2016learning}. \citet{walton13} has shown that in an adversarial setting, the queue regret (difference between the queue-length induced by a learning algorithm with respect to a static optimal policy) increases at most sublinearly in time. On the other hand, in a stochastic setting, \citet{krishnasamy2016learning} have shown that the expected regret in fact decreases with time (roughly as $\tilde{O}(1/t)$). 

Starting from the above studies, there has been increasing interest in the regret of algorithms in various queueing settings  \citep{krishnasamy2018learningcu, cayci2017learning,stahlbuhk2018learningalgorithm,liu2020pond,fbnmh20}. \citet{krishnasamy2018learningcu} studied the problem of scheduling jobs using the $c\mu$ rule with unknown service rates and showed that the cumulative queue regret (i.e., sums of queue regret over time) is $\order(1)$. \citet{liu2020pond} studied the problem of distributing different job classes across servers with unknown rewards for each job class-server pair and proves a reward regret of $\order(\sqrt{t})$. Bandits problems of similar flavour are also studied in the communication system settings, where \citet{cayci2017learning} studied channel allocation in wireless downlink systems with unknown channel statistics,
with an objective to identify the optimal number of channels to activate and proposed an UCB-based index policy that achieves $\order(\ln t)$ regret. The task of selecting the optimal channel in a wireless system with a single transmitter/receiver and multiple channels was studied by \citet{stahlbuhk2018learningalgorithm}, and they derived queue length based policies that achieve $\order(1)$ cumulative queue regret by exploiting samples acquired during the idle time of queues. Finally, \citet{fbnmh20} studied regret from an age of information viewpoint. 

Unlike these studies, our setting is one where the queues are not centrally located at the dispatcher. Instead, jobs are dispatched to individual queues based on partial information; this setting requires both learning a discrete support set and an  estimation of dispatch weights (over continuous parameters).%, thus highlighting new regret scaling properties.

% \Tuhinrevise{\citep{walton13} studied the queueing problem for a non-stochastic setting and proved the existence of an online algorithm that stabilizes the queue and achieves $o(t)$ queue regret. Bandit problem in the stochastic queueing system was studied in \citep{krishnasamy2016learning} with the task of determining the optimal matching between job classes and servers and they proved a queue regret bound of $\order(poly(\ln t)/t)$. 


% Although there is extensive prior work on multi-armed bandit algorithms \citep{bubeck2012regret, auer2002finite, lattimoreszepesvari2020banditbook} and their analysis, these online learning methods have only recently been used in queueing systems \citep{walton13,krishnasamy2016learning, krishnasamy2018learningcu, cayci2017learning, stahlbuhk2018learningalgorithm,liu2020pond}.
%
%
% are seldom applied to queueing systems. 
% This is because unlike the standard multi-armed bandit setting where the rewards obtained by pulling an arm are i.i.d. and stationary, in the queueing settings, the response times of jobs are non-stationary. There is also some work in queueing bandits in communication system \citep{cayci2017learning, stahlbuhk2018learningalgorithm}. Only a handful of recent works such as \citep{krishnasamy2016learning, krishnasamy2018learningcu} have proposed the use of multi-armed bandit algorithms, or more generally reinforcement learning methods, to queueing systems. Both these works consider that incoming jobs are held at the single central queue (or multiple centralized queues in the case where jobs belong to different priority classes), where each server receives a new job only when it is idle. The dispatching policy considers a bipartite graph consisting of links connecting the priority queues to the servers and chooses which of the links should be activated in each slot. Because there are no queues at the servers, this setting resembles more closely to the standard multi-armed bandit setting.

%\textbf{Job Dispatching in Queueing Systems.}

%\textbf{Multi-armed Bandit Algorithms.}

%\textbf{Bandit Policies for Queueing Systems.}

%A traditional MAB problem consists of $k$-arms. Arm $i$, when pulled give reward randomly sampled from a random variable with mean $\mu_i$. The problem is to identify the arm with the highest expected reward. Under this setting, many algorithms have been derived to determine the best-arm. \citep{jamieson2014lil} proposes a lil' UCB algorithm to identify the best arm. Another version of the problem is regret minimization. Regret is the difference between reward received from the algorithm and reward received if one only pulls the optimal arm.\citep{garivier2011kl}, \citep{auer2002finite}, \citep{agrawal2012analysis} gives some algorithm to minimize the regret over finite or infinite time-horizons. The problem that we are studying is a direct map to the MAB problem with regret minimization where regret corresponds to mean response time of the system. A similar setup  was studied in \citep{krishnasamy2016learning}; however, they assumed a single queue multi-server model, unlike the multi-queue multi-server model,  where multiple servers can remain active at a particular+ instance.

%\Gauri{I suggest avoiding using 'static' and 'dynamic' to indicate whether a policy uses queue length information. Our proposed algorithm can also be thought of as dynamic, although it does not use queue length information}
%Now, there is an extensive set of literature analyzing different load balancing policies for the multi-server system. Some of the popular queue-length-aware policies are JSQ, JFSQ, SED, Power-of-$2$ etc. A policy is called \textit{static} if it does not use queue length information to schedule the jobs. In this paper, we assume that the scheduler follows a static policy called \textit{weighted routing policy (WR)}. The policy works as follows; each server is assigned a weight, and any incoming job is randomly routed to one of the servers with probability proportional to its weight. Usually, a dynamic policy performs better than a static policy. This is because using queue length information balances the load is well across different servers. It has already been shown that JSQ is optimal in the stochastic order sense \citep{weber1978optimal}. Heavy traffic delay optimality of JSQ was proved in \citep{eryilmaz2012asymptotically}. \citep{weng2020optimal} shows that JFSQ in asymptotically optical in mean response time in the large server limit. In the large server limit, it has been shown that queue delay is significantly less for Po$2$ policy (\citep{mitzenmacher1996load, mitzenmacher2001power, vvedenskaya1996queueing}). \citep{banawan1992comparative} showed that SED performs really well in low-load and heavy load regime. Heavy traffic optimality of SED is shown in \citep{foschini1977heavy}.


%\subsection{Organization of the paper}


==> old/old_files2/plot.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[scale = 0.30]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_1.pdf}
        \caption{$\lambda = 0.1$}
    \end{subfigure}
    \begin{subfigure}{0.33\linewidth}  
        \centering 
        \includegraphics[scale = 0.30]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_2.pdf}
        \caption{$\lambda = 0.2$}
    \end{subfigure}
    \begin{subfigure}{0.33\linewidth}  
        \centering 
        \includegraphics[scale = 0.30]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_4.pdf}
        \caption{$\lambda = 0.4$}
    \end{subfigure}
    \caption{Regret vs time for various policies}
    \label{fig:regret_policies}
\end{figure*}

==> old/old_files2/prob_formu.tex <==

%\Gauri{This may be a major notation change.. But I think we should change the server index $i$ to $k$. Right now we use $i$ and $j$ interchangeably}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{draft_pics/diagrams/policy.pdf}
    \caption{Our system model with job arrival rate $\lambda$ and $\numofserver$ servers with service rates $\mu_1, \dots, \mu_{\numofserver}$ respectively. The dispatching policy $\policy$ assigns each job to one of $K$ queues. The service rates and queue lengths are unknown to the dispatcher; it only observes the service times of departed jobs.
    %\vspace{-0.5cm}
    }
    \label{fig:dia_policy}
\end{figure}

\subsection{System Model, Arrivals and Departures}\label{subsec:sysmodel_arr_dep}

We consider a multi-server discrete-time\footnote{Although we use the discrete-time assumption for the regret analysis presented in this paper, the proposed policy can be used in continuous time systems. We conjecture that the regret analysis is extendable to continuous time systems as well, but this extension is beyond the scope of this paper and is left for future work.} queueing system consisting of $\numofserver$ servers, with one queue at each server storing the unfinished jobs that are dispatched to it, as illustrated in \Cref{fig:dia_policy}. Jobs arrive into the system according to a Bernoulli process with arrival rate $\lambda$, where $0<\lambda<1$. Specifically, let $\arrival(t)$ denote the number of job arrivals at the beginning of time slot $t$.  Then $\arrival(t)=1$ with probability $\lambda$ and $\arrival(t)=0$ with probability $1-\lambda$. 
%
Incoming jobs are dispatched to one of the  the $\numofserver$ servers according to a scheduling policy $\policy$. Once dispatched, the job joins a first-come-first-served queue with an infinite buffer size at that server. The $\numofserver$ servers have geometrically distributed service times with parameter $\mu_i$. That is, after a job reaches the head of the queue at server $i$, it departs at the end of the next time slot with probability $\mu_i$. With the arrival rate $\lambda$ and the service of the $i$-th server being $\mu_i$, the system is stable only if $\lambda < \sum_{i=1}^{\numofserver} \mu_i$, a condition that we assume to be true. 

Let $\arrival_i(t)$ and $\departure_i(t)$ denote the number of arrivals to queue~$i$ and the number of departures from queue $i$ respectively during time slot $t$. Let $\queue_i(t)$ represent the length of queue~$i$ at the beginning of slot $t$, including the job that is currently in service. We assume that the system starts with empty queues, i.e.,  $\queue_i(0) = 0$, for all $i$. Then the queue evolution process is given by
%\Gauri{Replace $\arrival_i(t)$ by $\arrival_i(t)$ similarly for $Q$ and $D$}
\begin{equation}
    \queue_i(t + 1) = \queue_i(t) + \arrival_i(t) - \departure_i(t).
\end{equation}
%\Gauri{The queue length is measured at the beginning of time slot $t+1$, right? Added that to the definition of the queue evolution process above}
We use $X_{i,n}$ to denote the service time of the $n$-th job that departs from server $i$. It is the time since the job reaches the head of its queue and starts service until it departs from the system. $X_{i,n}$ is geometrically distributed with success probability $\mu_i$, that is, $\Pr(X_{i,n} = x) = (1-\mu_i)^{x-1} \mu_i$ for $x \in \{1, 2, \dots \}$.

% \Gauri{Don't say that without loss of generality the servers are ordered. We consider the ordering only to find the static optimal policy, not in the bandit policy or when you are coupling. When you find the static optimal policy, you can use denote the ordered service rates as $\mu_{(1)} \geq \mu_{(2)} \geq \dots \geq \mu_{(k)}$ to distinguish them from $\mu_1$, $\mu_2$, \dots $\mu_k$, which need not be ordered}  We assume a non-preemptive FCFS scheduling policy for each queue, i.e., service of a job will start when all jobs ahead of it are serviced. Initially, the system, does not know $\mu_i$'s, however it can learn about the rates as more and more job departs from the system. Every time a job departs from server $i$, the system gets the service time of the job and it can use that to estimate  the parameter $\mu_i$. Let $X_1, X_2, \cdots, X_n$ be the service time of the $n$ jobs departed from server $i$ so far. Then, the estimate $\hat{\mu}_i$ of $\mu_i$ can be estimated as 
%\Gauri{Whenever you write $\hat{\mu}_i$, I suggest always adding an index $t$ to denote the time at which it is calculated, or $n$ to denote the number of samples used to calculate this estimate. }
%\Weina{Do not use $i$ both as the subscript for the estimate and the dummy variable for the sum.  Also please write out the range of the sum.  You can omit the range of the sum later when it is totally clear from the context, say, in the middle of a proof after you write the sum many times.}


\subsection{Information Available to the Dispatcher}
%\Gauri{I have switched the order of Sections 2.2 and 2.3 for now. Trying to rewrite to make this order work..}


\vspace{0.1cm} \textbf{Service Rates and Queue Lengths are Unknown.} Job dispatching policies for the multi-server setting described above have been extensive studied in previous literature \citep{mor_book, srikant2014communication}. However, most prior works assume that the dispatcher knows the service rates $\mu_1, \dots, \mu_K$, and it also has either full or partial information about the queue lengths $Q_i(t)$. For example, for homogeneous systems where $\mu_1 =  \dots = \mu_K = \mu$, the join-the-shortest-queue (JSQ) policy has full queue information and sends each incoming job to the server $i^* \in \arg \min Q_i(t)$, i.e., the shortest queue, with ties broken at random. Power-of-$d$-choice (Po$d$) policies \citep{mitzenmacher1996load, mitzenmacher2001power, vvedenskaya1996queueing} reduce the cost of querying queue lengths by sampling $d$ queues uniformly at random and dispatching the incoming job to the shortest queue. For heterogeneous service rates, JSQ can be generalized to the join-the-shortest-fastest-queue (JSFQ) \citep{weber1978optimal,eryilmaz2012asymptotically,weng2020optimal}, which breaks ties in favor for the queue with the fastest server. Other policies for systems with heterogeneous servers such as shortest expected delay (SED) \citep{banawan1992comparative,foschini1977heavy} also use some form of queue length information to make job dispatch decisions. In contrast, in this work, we consider that the service rates $\mu_1$, $\mu_2$, \dots,  $\mu_{\numofserver}$ of the $\numofserver$ servers are \emph{heterogeneous and unknown} to the dispatcher. Similarly, the queue lengths $Q_i(t)$ for $i = 1, \dots, \numofserver$ are also \emph{unknown} to the dispatcher.

%This is because, in modern applications such as job scheduling cloud data centers (need citations), we have thousands of servers without a centralized queue of jobs coming from different applications. The servers may be running background workload or higher jobs coming from other dispatchers. As a result, the service rate $\mu_i$ of server $i$ as seen by a job dispatcher is actually the service rate remaining after accounting for this external workload. It is difficult for a dispatcher to monitor the external workload at each server and obtain (even partial) queue length information due to two reasons: 1) privacy concerns -- if a server reveals its total queue length $Q_i(t)$ to one of the dispatcher, it may compromise the privacy of other dispatchers by revealing information about how many jobs they sent to that queue and 2) even if privacy is not a concern, due to large communication delays incurred when a dispatcher queries the queue length of a server, the queue length information may become stale by the time the job is assigned. Therefore, we consider that service rates $\mu_i$ and the queue lengths $Q_i(t)$ are unknown to the dispatcher. \footnote{In practice, the effective service rates may also vary over time depending on the external workload. For tractability of the analysis, we do not consider time-varying service rates $\mu_i$. However, our proposed algorithm can account for time-varying service rates by modifying the estimates of $\mu_i$ in \eqref{eqn:mu_estimate} to discount older service time observations.}
 
%Similarly, we consider that the queue lengths $Q_i(t)$ for $i = 1, \dots, \numofserver$ are also \emph{unknown} to the dispatcher. This is because in large-scale systems it is prohibitively expensive for a job dispatcher to keep track of the queue lengths $Q_i(t)$ at each server $i$. However, in large-scale systems with multiple job sources, each server's queue receives jobs from many dispatchers. In this setting, it would be infeasible to obtain queue length information due to two reasons: 1) privacy concerns -- if a server reveals its total queue length $Q_i(t)$ to one of the dispatcher, it may compromise the privacy of other dispatchers by revealing information about how many jobs they sent to that queue and 2) even if privacy is not a concern, due to large communication delays incurred when a dispatcher queries the queue length of a server, the queue length information may become stale by the time the job is assigned. Therefore, we assume that the queue lengths $Q_i(t)$ are unknown to the dispatcher. 

\vspace{0.1cm} \noindent \textbf{Dispatcher Observes Service Times of Departed Jobs.} In lieu of service rates and queue lengths, we consider that the dispatcher observes service times $X_{i1}$, \dots $X_{iN_i(t)}$ of the $N_i(t)$ jobs that depart from server $i$ by time $t$. In practice, this information can be made available to the dispatcher by having the server send  the dispatcher a notification when a job reaches the head of its queue and begins service and another notification when it departs. The dispatching policy $\policy$ can use this information to estimate the service rates $\mu_1$, \dots $\mu_{\numofserver}$. For example, it can estimate the service rate vector $\hat{\bm{\mu}}(t) = \left(\hat{\mu}_1(t), \hat{\mu}_2(t), \cdots, \hat{\mu}_\numofserver(t)\right)$ at time $t$, where $\hat{\mu}_i(t)$ is given by 
\begin{equation}
    \hat{\mu}_i(t) = \frac{N_i(t)}{\sum_{j=1}^{N_i(t)} X_{i,j}} \label{eqn:mu_estimate},
\end{equation}
and use it to make job dispatch decisions. For instance, it can dispatch a larger fraction of jobs to server $i$ if it has a higher service rate estimate $\hat{\mu}_i(t)$.

\subsection{Weighted Random Routing Policies}
\label{sec:weighted_random_routing}

The service rate estimate $\hat{\mu}_i(t)$ can be used by the dispatcher in a variety of ways to make job dispatch decisions. Among all the possible scheduling policies, we focus on the class of \textit{weighted random routing policies}, which are defined as follows.

\begin{defn}[Weighted Random Routing $\policy$]
\label{defn:weighted_random_routing}
In time slot $t$, the dispatcher associates a probability $\hat{p}_i(t)$ with server $i$, where $\hat{p}_i(t)$'s satisfy the property $\sum_{j=1}^{\numofserver} \hat{p}_j(t)=1$. We call the probability vector $\hat{\bm{p}}(t) = \left(\hat{p}_1(t), \hat{p}_2(t), \cdots, \hat{p}_\numofserver (t)\right)$ the \emph{routing vector}. A job that arrives at time $t$ is dispatched to server $i$ with probability $\hat{p}_i(t)$, independent of other jobs. The routing vector $\hat{\bm{p}}(t) = f(\lambda, \hat{\bm{\mu}}_i(t))$, where $f:[0,1]^{\numofserver+1} \rightarrow [0,1]^{\numofserver}$ is a fixed, deterministic function.
\end{defn}

The uniform random routing policy corresponds to setting $\hat{\bm{p}}(t) = \left(1/\numofserver, \cdots, 1/\numofserver \right)$. Since the routing vector $\hat{\bm{p}}(t)$ is a fixed, predetermined function of $\hat{\mu}_i(t)$, policies such as round-robin dispatching that retain a memory of where past jobs were dispatched are not included in this class of weighted random routing policies. 

\vspace{0.1cm} \noindent \textbf{Optimal Weighted Random Routing.} Consider a genie system where the dispatcher knows the service rates $\mu_1, \dots, \mu_{\numofserver}$. Then the optimal weighted routing policy $\policy^*$ is defined as the policy that chooses the optimal $\bm{p}^* = f(\lambda, \bm{\mu})$, that minimizes the expected steady-state queue length $\mathbb{E}[\sum_{i=1}^{\numofserver} Q_i(\infty)]$, which is equivalent to minimizing the mean response time experienced by incoming jobs. 
We will derive $\bm{p}^*$ in \Cref{sec:optimal_randomized_policy}.

\subsection{Measuring Performance in terms of Regret}
We seek to design a weighted random routing policy $\policy$ that starts with no knowledge of the service rates and converges to the optimal random routing policy $\policy^*$. To evaluate the transient performance of $\policy$ in terms of how quickly it learns $\policy^*$, we define a performance metric $\regret_{\policy \policy^*}(t)$, referred to as the regret of $\policy$. In \Cref{sec:regret_analysis}, we analyze the performance of our proposed dispatching policy in terms of the expected regret $\mathbb{E}[\regret_{\policy \policy^*}(t)]$.

\begin{defn}[Regret of a Dispatching Policy]
\label{defn:regret}
The regret $\regret_{\policy \policy^*}$ of a dispatching policy $\policy$ with respect to the optimal baseline $\policy^*$ is
\begin{equation}
    \regret_{\policy \policy^*}(t) \triangleq \sum_{\tau = 1}^t \sum_{i = 1}^{\numofserver}\left( \queue_i(\tau) - \queue_i^{*}(\tau)\right),
\end{equation}
where $\queue_i^*(t)$ represent the queue length at server $i$ at time $t$ when following policy $\policy^*$. 
\end{defn}

The $\regret_{\policy \policy^*}(t)$ represents the cost of using policy $\policy$ instead of $\policy^*$ in terms of cumulative queue length till time $t$. Note that the cumulative queue length is the total time spent by all jobs that arrived before time $t$, including the jobs that have departed. Hence, regret represents the additional time jobs stayed in the system when using policy $\policy$ instead of $\policy^*$. It is the penalty the policy $\policy$ has to pay for the lack of knowledge the service rates system.

\vspace{0.1cm} \noindent \textbf{Difference from the Regret used in Multi-armed Bandits.} Although similar, the regret considered in this paper and its analysis is fundamentally different from the multi-armed bandit setting \citep{bubeck2012regret,lattimoreszepesvari2020banditbook,lai1985asymptotically}. In the multi-armed bandit setting with $K$ arms, asymptotically optimal algorithms pull the best arm (with the highest mean reward) $O(t)$ times and pull all the $K-1$ sub-optimal arms $O(\log t)$ times. In our queueing setting, the optimal random routing policy generally sends $O(t)$ jobs to all servers with $p_i^*> 0$ and not just the fastest server with the highest service rate $\mu_i$. We seek fast convergence of the routing vector $\hat{\bm{p}}(t)$ to the optimal $\bm{p}^*$ so as to dispatch the optimal fraction $p_i^*$ of incoming jobs to each server $i$.

%\Weina{Mention expected regret here?}

%and achieves a low expected regret $\expectation\left[\regret_{\policy \policy^*}(t)\right]$

%\Gauri{Write a formal definition of regret here, pointing the readers to the formal definition of the optimal randomized policy, which we use as the baseline}
%\Weina{Justify why this is the right regret definition -- the total time spent by all the jobs that arrived before time t (including the jobs that have already departed)}

%\Weina{The regret definition should be separated from the previous paragraph.  I don't think we need to mention multi-armed bandits here.  Regret also appears in reinforcement learning and online optimization.  We should mention the connection to multi-armed bandit problems in the introduction.  But rather, we should explain why we define regret based on queue lengths.  I'm thinking of either mentioning job response time or holding costs.}

\subsection{Justification for Focusing on Weighted Random Routing Policies}

In this section, we justify why we choose to focus on the class of weighted random routing policies. First, we explain why service rates and queue lengths are unknown in the large-scale systems envisioned in this work. Furthermore, we show that even if partial or delayed queue length information is available, using it and performing join-the-shortest-queue (JSQ) or join-the-fast-shortest-queue (JFSQ) dispatching does not give a large performance improvement over weighted random routing.

\vspace{0.1cm} \noindent \textbf{Why the Service Rates are Unknown.} Traditionally, multi-server queueing systems consisted on dedicated servers and a single source of incoming jobs. However, in modern applications such as cloud data centers, a server may be receiving jobs from several different applications. For instance, it may be running background workload such as check-pointing and garbage collection, or higher priority jobs coming from other sources \citep{dean2013tail}. As a result, the effective service rate $\mu_i$ of server $i$ as seen by the dispatcher of any one application depends on the external workload. Due to privacy constraints and communication delays, it is infeasible for each dispatcher to know and keep track of the external workload at each server. Therefore, we consider that service rates $\mu_i$ are unknown to the dispatcher.% do not explicitly consider multiple job sources and instead .
\footnote{In practice, the effective service rates may vary over time depending on the external workload. For tractability of the analysis, we do not consider time-varying service rates $\mu_i$. However, the estimates in \eqref{eqn:mu_estimate} can be modified to discount older service time observations in order to account for time-varying service rates.}

%\Gauri{Randomized --> Random -- DONE for this section}
%\Gauri{Assign --> Dispatch -- DONE for this section}

\vspace{0.1cm} \noindent \textbf{Why Queue Lengths are Unknown.} In large-scale systems with multiple job sources, each server's queue receives jobs from many dispatchers. In this setting, it is difficult to obtain queue length information due to two reasons: 1) privacy concerns -- if a server reveals its total queue length $Q_i(t)$ to one of the dispatcher, it may compromise the privacy of other dispatchers by revealing information about how many jobs they sent to that queue and 2) even if privacy is not a concern, due to large communication delays incurred when a dispatcher queries the queue length of a server, the queue length information may become stale by the time the job is dispatched. Therefore, we consider that the queue lengths $Q_i(t)$ are unknown to the dispatcher.

 
%\sout{Apart from the user's arrival of jobs, each server $i$ has an additional external arrival according to a Poisson process of rate $\lambda_i^{ext}$. This kind of situation can be seen in computing clusters where multiple people are simultaneously using the same set of clusters. Although our model is different , this type of setting can be relevant to our model. Note that from the user's perspective, the effective rate of server $i$ is $\left(\mu_i - \lambda_i^{ext}\right)$. Now, if the external arrival rate is unknown while the true service rate of servers are known, then a good scheduling policy essentially boils downs to estimating the effective service rate.}

%\sout{However, numerical evidence shows that under certain circumstances, the weighted routing algorithm outperforms policies like JSQ and JFSQ. Consider another multi-server setting as described in Subsection \ref{subsec:sysmodel_arr_dep}. Apart from the user's arrival of jobs, each server $i$ has an additional external arrival according to a Poisson process of rate $\lambda_i^{ext}$. This kind of situation can be seen in computing clusters where multiple people are simultaneously using the same set of clusters. Although our model is different , this type of setting can be relevant to our model. Note that from the user's perspective, the effective rate of server $i$ is $\left(\mu_i - \lambda_i^{ext}\right)$. Now, if the external arrival rate is unknown while the true service rate of servers are known, then a good scheduling policy essentially boils downs to estimating the effective service rate. In this setting, consider the following two situations.} 

% \begin{enumerate}
%     \item \textit{Privacy of queues} - The user has no information on the queue length corresponding to external arrival because of privacy issues, however it knows how many of its own job are there in each queue. 
%     \item \textit{Communication delay} - The queue length information is updated with a delay and the user has access to the last updated queue length information. This kind of situation can be expected in a large cluster where updating the queue length information of all the queues all the time can be costly.
% \end{enumerate}

\vspace{0.1cm}
\noindent \textbf{Limited Utility of Partial or Delayed Queue Length Information.}
In \Cref{fig:compare}, we consider a system of $6$ servers with service rates $\mu_i$ such that $\mu_i = 2^{i-1} \mu_1$, and $\sum_{i=1}^{6} \mu_i = 0.99$. We show a comparison of the mean response times (waiting time in queue plus service time) for optimal weighted random (OWR) routing, which knows the service rates $\mu_i$ but does not use queue length information, with JSQ and JFSQ, which use queue length information to make job dispatching decisions. Our goal is to demonstrate that when the queue length information is partial or delayed, a queue-length-agnostic policy such as OWR performs nearly as well as JSQ and JFSQ. %\Gauri{Need to be more precise in the above sentences. Please check the edited version above}

To model partial and delayed queue length information, we consider that apart from the rate $\lambda$ job arrivals at the dispatcher, server $i$ has external Poisson arrivals at rate $\lambda_i^{ext}$ that are not visible to the dispatcher. For \Cref{fig:compare_privacy} and \Cref{fig:compare_communication}, we choose $\lambda_i^{ext} = \mu_i/2$, while for \Cref{fig:compare_privacy_heavy_arrival} and \Cref{fig:compare_communication_heavy_arrival}, we choose $\lambda_i^{ext} = 4\mu_i/5$. In \Cref{fig:compare_privacy_combined}, we consider that due to privacy concerns, the dispatcher only has queue length information about the jobs that it sent to each queue, but not about the external arrivals. In \Cref{fig:compare_communication_combined}, we consider the case of delayed queue lengths, where the dispatcher receives updated queue length information (including both its jobs and the external arrivals) with probability $1/3$. For OWR, we assumed that the policy does not know $\mu_i$ or $\lambda_i^{ext}$ but knows the difference $(\mu_i - \lambda_i^{ext})$ and uses the routing vector $f(\lambda, \bm{\mu} - \bm{\lambda}^{ext})$ to dispatch jobs. All the simulations are averaged over $40$ trials of $10^7$ job departures each. %\Gauri{There should always be a space before brackets} 
For both these cases, observe in \Cref{fig:compare} that in the low to moderate load regimes (load $= (\lambda + \sum_{i=1}^{K} \lambda_i^{ext})/\sum_{i=1}^{K} \mu_i)$), the optimal weighted random routing (OWR) policy is comparable to JFSQ and better than JSQ in terms of the mean response time. %, where response time is the wait time in queue plus the service time.
Moreover, observe that as the external arrival rate $\lambda_i^{ext}$ increased from $\mu_i/2$ to $4\mu_i/5$, the load beyond which OWR performs worse than JFSQ shifted from $0.8$ to $0.9$ roughly. This is because at heavy load, the cost of a sub-optimal allocation of job using a partial or delayed information is more than using no information at all. We conjecture that OWR becomes more and more useful as the cross traffic load increases.


%\Gauri{Tuhin, can you please edit the above paragraph and specify all the parameters that you used in the simulations? Need to mention in a sentence that response time is the waiting time in queue plus service rate. Also, need to define the load mathematically in terms of $\lambda$ and $\lambda_i^{ext}$.}
%\Tuhin{Done.}

As a result of these observations, we choose to focus on the class of weighted random routing policies that do not take into account of queue lengths when making job dispatching decisions, and seek to design a dispatching policy that can learn unknown service rates while simultaneously minimizing the regret (see \Cref{defn:regret}). Another reason is that for this class of policies, the optimal policy $\policy^*$ that minimizes the steady-state cumulative queue length is clearly defined, as we show in \Cref{sec:optimal_randomized_policy} below. In contrast, the optimal policy is not known in the case where queue lengths are considered for job assignment decisions. Although policies such as JSQ and JFSQ perform well in practice and have been shown to be optimal in the heavy-traffic regime, it is unclear which policy is optimal in other regimes.
%JSQ and JFSQ used the queue length information available to the user while OWR used the effective service rate of the servers. The simulation setup considered a system of $6$ servers where the service rates forms a geometric progression and communication delay is geometrically distributed.

% \begin{enumerate}
%     \item \textit{Privacy of queues} - The user has no information on the queue length corresponding to external arrival because of privacy issues, however it knows how many of its own job are there in each queue. 
%     \item \textit{Communication delay} - The queue length information is updated with a delay and the user has access to the last updated queue length information. This kind of situation can be expected in a large cluster where updating the queue length information of all the queues all the time can be costly.
% \end{enumerate}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{1\linewidth}
        \begin{subfigure}[b]{0.49\linewidth}
            \centering
            \renewcommand\thesubfigure{a1}
            \includegraphics[width=48mm]{plots/simulation/justify_opt_random/data_privacy_geo_discrete.pdf}
            \caption{$\lambda_i^{ext} = \frac{\mu_i}{2}$}
            \label{fig:compare_privacy}
        \end{subfigure}
        \hfill
        \centering
        \begin{subfigure}[b]{0.49\linewidth}  
            \centering
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{a2}
            \includegraphics[width=48mm]{plots/simulation/justify_opt_random/data_privacy_geo_discrete_heavy_arrival.pdf}
            \caption{$\lambda_i^{ext} = \frac{4\mu_i}{5}$}
            \label{fig:compare_privacy_heavy_arrival}
        \end{subfigure}
        \addtocounter{subfigure}{-1}    
        \caption{Partial Queue Length Information (excluding external workload)}
        \label{fig:compare_privacy_combined}
    \end{subfigure}
    \hfill
    \centering
    \begin{subfigure}[b]{1\linewidth}
        \begin{subfigure}[b]{0.49\linewidth}
            \centering
            \renewcommand\thesubfigure{b1}
            \includegraphics[width=48mm]{plots/simulation/justify_opt_random/comm_cost_geo_discrete.pdf}
            \caption{$\lambda_i^{ext} = \frac{\mu_i}{2}$}
            \label{fig:compare_communication}
        \end{subfigure}
        \hfill
        \centering
        \begin{subfigure}[b]{0.49\linewidth}  
            \centering
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{b2}
            \includegraphics[width=48mm]{plots/simulation/justify_opt_random/common_cost_geo_discrete_heavy_arrival.pdf}
            \caption{$\lambda_i^{ext} = \frac{4\mu_i}{5}$}
            \label{fig:compare_communication_heavy_arrival}
        \end{subfigure}
        \addtocounter{subfigure}{-1}    
        \caption{Delayed Queue Length Information (including external workload)}
            \label{fig:compare_communication_combined}
    \end{subfigure}
    \caption{%Performance comparison of $3$ policies under different traffic regimes. 
    OWR performs better than JSQ and similar to JFSQ in the middle and low traffic regime. In the heavy traffic regime, both JSQ and JFSQ performs better than OWR. OWR performs better as the external workload increases.
    %\Gauri{Write an information caption describing the main message of this figure}
    % \Gauri{Remove the relative load axis} 
    % \Gauri{Make the axis label fonts bigger}
    \vspace{-0.5cm}
    }
    \label{fig:compare}
\end{figure}

%\sout{We assume that the scheduler has no prior information about the system parameters at the beginning. Now, with complete system information, the scheduler can make a more informed decision. E.g. if the scheduler knows that $\mu_1 \geq \mu_2$, it knows that it is better to send more jobs to server $1$ as compared to server 2 on average to achieve a better response time. However, every time a job departs from any server $i$, the scheduler learns the service time of the job.  As more and more jobs leave the system, the scheduler can estimate the service rates of the different servers from the service time of the departed jobs. At any time $t$, the policy $\policy$ has access to only service time of jobs that departed from the system till time $t$. Using this information, the policy $\policy$ can choose a weighted routing algorithm to schedule } %\Weina{The part may be easier to write after justifying why we consider the static optimal policy.}

%\Gauri{Weina, is 'job assignment' a better term than 'job routing'? We should choose one of these and consistently use it throughout the paper}



==> old/old_files2/prooflemma2backup.tex <==
We first utilize the event $\eventfive$ to further upper bound the queue length difference based on the upper bound in \eqref{rel:regret_equation}. Specifically, recall that $\eventfive$ is the event where  $B_i(t)\le v_i(t)=\frac{66\ln t}{\freecapacity_{i}^2}$ for all server $i$.  Then based on \eqref{rel:regret_equation}, we have
\begin{align}
&\mspace{21mu}\sum_{i=1}^K\expectation\left[\queue_i(t) - \queue_i^*(t)\right]\nonumber\\
&=\expectation\left[\left(\sum_{i=1}^K\left(\queue_i(t) - \queue_i^*(t)\right)\right)\cdot (\indicatorofevents_{\eventfive} + \indicatorofevents_{\left(\eventfive\right)^c} ) \right]\nonumber\\
%&\mspace{21mu}+\expectation\left[\left(\sum_{i=1}^K\left(\queue_i(t) - \queue_i^*(t)\right)\right)\cdot \indicatorofevents_{\left(\eventfive\right)^c}\right]\nonumber\\
&\le \expectation\left[\left(\sum_{i=1}^K\sum_{\ell = t- \busy_i(t)}^{t-1} \explore_i(\ell)\right)\cdot\indicatorofevents_{\eventfive}\right]\nonumber\\
&\mspace{21mu}+ \expectation\left[\sum_{i=1}^K\left(\sum_{\ell = t- \busy_i(t)}^{t-1} \indicatorofevents_{\left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}}\right)\cdot\indicatorofevents_{\eventfive}\right]\nonumber\\
&\mspace{21mu}+ t\probability\left(\left(\eventfive\right)^c\right)\label{eq:bound-eventfive-temp1}\\
&\le \expectation\left[\sum_{i=1}^K\sum_{\ell = t- v_i(t)}^{t-1} \explore_i(\ell)\right]\nonumber\\
&\mspace{21mu}+ \expectation\left[\sum_{i=1}^K\sum_{\ell = t- v_i(t)}^{t-1} \indicatorofevents_{\left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}}\right]+t\probability\left(\left(\eventfive\right)^c\right)\label{eq:bound-eventfive-temp2}\\
&\le \sum_{i=1}^K\frac{2v_i(t)\ln t}{t}+\sum_{i=1}^K\sum_{\ell = t- v_i(t)}^{t-1}\probability\left(\exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right)\nonumber\\
&\mspace{21mu}+t\probability\left(\left(\eventfive\right)^c\right),\label{eq:bound-eventfive-temp3}
\end{align}
where \eqref{eq:bound-eventfive-temp1} uses \eqref{rel:regret_equation} and the fact that $\sum_{i=1}^K\left(\queue_i(t)-\queue^*_i(t)\right)\le t$ since there are at most $t$ arrivals before time $t$; \eqref{eq:bound-eventfive-temp2} is due to the property $\busy_i(t)\le v_i(t)$ given by the indicator $\indicatorofevents_{\eventfive}$; and \eqref{eq:bound-eventfive-temp3} is because $v_i(t)\le t/2$ for large enough $t$.

Next, it suffices to bound $\probability\left(\exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right)$ using event $\eventsix$. Using Lemma~\ref{lem:mismatch} for  $\hat{\bm{p}}(t)=f(\lambda, \hat{\bm{\mu}})$, the routing probability vector computed from the estimated service rates, we have
\begin{align}
&\mspace{21mu}\sum_{i=1}^K\sum_{\ell = t- v_i(t)}^{t-1}\probability\left(\exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right)\nonumber\\
&=\sum_{i=1}^K\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\probability\left(\exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\mmiddle\hat{p}_i(t)\right)\right]\nonumber\\
&\le \sum_{i=1}^K\sum_{\ell = t- v_i(t)}^{t-1}\expectation\left[\left|\hat{p}_i(t)-p_i^*\right|\right]\label{eq:bound-eventsix-temp1}\\
&=\expectation\left[\left(\sum_{i=1}^K\sum_{\ell = t- v_i(t)}^{t-1}\left|\hat{p}_i(t)-p_i^*\right|\right)\cdot\indicatorofevents_{\eventsix}\right]\nonumber\\
&\mspace{23mu}+\expectation\left[\left(\sum_{i=1}^K\sum_{\ell = t- v_i(t)}^{t-1}\left|\hat{p}_i(t)-p_i^*\right|\right)\cdot\indicatorofevents_{\left(\eventsix\right)^c}\right]\nonumber\\
&\le \sum_{i:p_i^*>0} k_1v_i(t) \sqrt{\frac{\ln t}{t}} + 2t\probability\left(\left(\eventsix\right)^c\right),\label{eq:bound-eventsix-temp2}
\end{align}
where \eqref{eq:bound-eventsix-temp1} is due to Lemma~\ref{lem:mismatch}; \eqref{eq:bound-eventsix-temp2} uses the definition of the event $\eventsix$, the fact that $v_i(t)\le t/2$ for large enough $t$, and the fact that $\sum_{i=1}^K\left|\hat{p}_i(t)-p_i^*\right|\le 2$ for the second summand.  Inserting \eqref{eq:bound-eventsix-temp2} back to \eqref{eq:bound-eventfive-temp3} completes the proof.\qed

==> old/old_files2/regret_analysis.tex <==
\section{Regret Analysis}\label{sec:regret_analysis}
In this section, we prove an upper bound on the expected regret $\expectation\left[\regret_{\policy \policy^*} (t)\right]$ of the $\epsilon_t$-exploration policy.

To state our upper bound, we first define a quantity $\Delta_{\support}$ that we refer to as the \emph{tolerance gap}, which is analogous to the suboptimality gap for multi-armed bandits.  Specifically, let
\begin{equation}\label{eq:gap}
\begin{split}
\Delta_{\support} &:= \sup\left\{\delta \geq 0\colon \support\left(\lambda,\bm{\mu}'\right) = \support(\lambda,\bm{\mu})\right.\\
&\mspace{111mu}\left.\forall\bm{\mu}'\mathrm{ s.t.\ } \left|\mu'_i-\mu_i\right|\leq \delta,\forall i\right\},
\end{split}
\end{equation}
where recall that $\support(\lambda,\bm{\mu})$ is the optimal support set computed from arrival rate $\lambda$ and service rate vector $\bm{\mu}$.

The tolerance gap $\Delta_{\support}$ quantifies how much error in the service rates can be tolerated without incurring a discrepancy in the support set.  We can think of the $\bm{\mu}'$ in \eqref{eq:gap} as the estimated service rate vector.  If $\Delta_{\support}=0$, then even a slight imprecision in the estimated service rates would make the estimated support set deviate from the optimal support set, indicating hardness of the problem.  Therefore, we make the assumption that $\Delta_{\support}>0$ in our upper bound.  We comment that from a practical perspective, this is a very mild assumption since only a small set (with zero measure) in the parameter space $\left\{(\lambda,\bm{\mu})\in\mathbb{R}_+^{K+1}\colon \lambda<\sum_{i=1}^K \mu_i\right\}$ will violate this assumption.


\begin{thm}[Upper Bound on Expected Regret]
\label{thm:main}
Consider a system with arrival rate $\lambda$ and service rate vector $\bm{\mu}$ and assume that $\Delta_{\support}>0$.
Then there exists a constant $k_1$ and a $t_0$ such that for all $t \geq t_0$, the $\epsilon_t$-exploration policy (\Cref{poli:bandit}) has an expected regret $\expectation\left[\regret_{\policy \policy^*} (t)\right]$ that admits the following upper bound:
\begin{multline}
\expectation\left[\regret_{\policy \policy^*} (t)\right]\\
\le \sum_{\tau = t_0}^{t-1}\left(\sum_{i: p_i^* > 0}\frac{66k_1\ln \tau}{\freecapacity_i^2}\sqrt{\frac{\ln \tau}{\tau}}+\sum_{i=1}^{\numofserver}\frac{132 \ln^2 \tau}{\freecapacity_i^2 \tau}\right) + \order\left(1\right),
\end{multline}
where $\freecapacity_i$ is the residual capacity of server $i$ under the optimal weighted random routing given by $\freecapacity_i = \mu_i - \lambda p_i^*$.
\end{thm}

In the regret upper bound in Theorem~\ref{thm:main} above, the first summand $\sum_{\tau = t_0}^{t-1}\sum_{i: p_i^* > 0}\frac{66k_1\ln \tau}{\freecapacity_i^2}\sqrt{\frac{\ln \tau}{\tau}}$ is the dominant term and it comes from the estimation error in the estimated routing probability vector $\bm{\hat{p}}(t)$, and the second summand $\sum_{\tau = t_0}^{t-1}\sum_{i=1}^{\numofserver}\frac{132 \ln^2 \tau}{\freecapacity_i^2 \tau}$ results from the exploration used by the $\epsilon_t$-exploration policy.  We note that this regret bound becomes smaller in low to moderate traffic regimes where the residual capacities $\freecapacity_i$'s are large and the size of the optimal support set $\support\left(\lambda,\bm{\mu}\right)=\{i\colon p_i^*>0,i=1,2,\dots,K\}$ is small.


%\Gauri{Add discussion on 1) the dominant term in the regret bound and that it comes from the error in estimating $p$'s, 2) the second dominant term which comes from exploration, 3) the regret bound becomes smaller in low to moderate traffic regimes where $r_i$ is large and the size of the support set is smaller, and 4) how this regret bound differs from the regret analysis of traditional multi-armed-bandit algorithms and that in Sanjay's queueing bandits papers}

In the following subsections, we first couple our system with the system that runs the the optimal weighted random routing policy in Section~\ref{subsec:coupling} to facilitate the regret analysis.  We then prove Theorem~\ref{thm:main} in Section~\ref{subsec:proof-regret-bound}, using several lemmas whose proof sketches are given in Section~\ref{subsec:proof-sketch-lemmas}.


\subsection{Coupling with the Optimal Weighted Random Routing}\label{subsec:coupling}
Consider the system that runs the optimal weighted random routing policy $\policy^*$, which we refer to as the \emph{optimal system}.  We will annotate quantities in the optimal system with the superscript $^*$, e.g., $\arrival^*(t)$ denotes the total number of job arrivals at time $t$ to the optimal system, and $\queue_i^*(t)$ denotes the length of queue $i$ under $\policy^*$.  Correspondingly, recall that the regret at time $t$ is defined as
\begin{equation*}
\regret_{\policy \policy^*}(t) = \sum_{\tau = 1}^{t-1} \sum_{i = 1}^{\numofserver}\left( \queue_i(\tau) - \queue_i^*(\tau)\right).
\end{equation*}
We assume that the optimal system also starts from empty queues, i.e., $\queue_i^*(0)=0$ for all $i$.



We couple the system that runs our proposed $\epsilon_t$-exploration policy with the optimal system in the following way.

\vspace{0.1cm} \noindent {\textbf{Arrivals.}}
We couple arrivals such that $\arrival(t)=\arrival^*(t)$ for all time $t$.
    
\vspace{0.1cm} \noindent {\textbf{Service.}}
%To define the coupling for the job service processes, we use the following equivalent description of the queueing dynamics due to the geometrically distributed service times. 
For each server~$i$, let $\service_i(t)$ for $t=0,1,2,\dots$ be i.i.d.\ Bernoulli random variables that take the value $1$ with probability $\mu_i$.  We will refer to $\service_i(t)$ as the \emph{service} offered by server $i$ at $t$.  If $\queue_i(t)+\arrival_i(t)>0$, we let $\departure_i(t)=\service_i(t)$, where recall that $\departure_i(t)$ is the number of departures from queue $i$ at $t$; otherwise it is clear that $\departure_i(t)=0$. Similarly, let $\service_i^*(t)$ denote the corresponding service offered in the optimal system.
We couple the service processes such that $\service_i(t)=\service_i^*(t)$ for all server $i$ and all time $t$.
    
\vspace{0.1cm} \noindent {\textbf{Assignment process.}}
Recall that in the $\epsilon_t$-exploration policy, for each time slot $t$, with probability $\frac{\numofserver \ln t}{t}$ we explore and otherwise we dispatch the arriving job according to the routing vector $\hat{\bm{p}}(t)$. We couple the dispatching decision generated from $\hat{\bm{p}}(t)$ with the dispatching decision generated from the optimal routing vector $\bm{p}^*$ in the optimal system as follows.

For simplicity, we can assume that for each time slot $t$, we generate a dispatching decision from $\hat{\bm{p}}(t)$, although this dispatching decision is needed only when there is a job arrival at $t$ and the $\epsilon_t$-exploration policy chooses to exploit.  Let the dispatching decision generated from $\hat{\bm{p}}(t)$ be represented by the server that an arriving job will be dispatched to, denoted as $\dispdecision(t)$.  Then $\dispdecision(t)$'s pmf is $\hat{\bm{p}}(t)$.  Similarly, let $\dispdecision^*(t)$ be the dispatching decision in the optimal system, and then $\dispdecision^*(t)$'s pmf is $\bm{p}^*$. Then we couple $\dispdecision(t)$ and $\dispdecision^*(t)$ such that they have the following joint pmf:
\begin{multline}
\probability(\dispdecision(t)=i,\dispdecision^*(t)=j)\\
=
\begin{cases}
\min\{\hat{p}_i(t),p^*_i\} & \textrm{ if }i=j,\\
\frac{\left(\hat{p}_i(t)-\min\left\{\hat{p}_i(t),p^*_i\right\}\right)\left(p^*_j(t)-\min\left\{\hat{p}_j(t),p^*_j\right\}\right)}{d_{TV}(\hat{\bm{p}}(t), \bm{p}^*)} & \textrm{ if }i\neq j,
\end{cases}
\end{multline}
where $d_{TV}(\hat{\bm{p}}(t), \bm{p}^*)$ is the total variation distance between $\hat{\bm{p}}(t)$ and $\bm{p}^*$ and $d_{TV}(\hat{\bm{p}}(t), \bm{p}^*) =\sum_{j=1}^K\left(p^*_j(t)-\min\left\{\hat{p}_j(t),p^*_j\right\}\right)$ for the job routing distributions. This coupling is known as the \emph{maximal coupling} (see, e.g., \citep{RosPek_07}) and it guarantees that $\probability(\dispdecision(t)\neq\dispdecision^*(t))=d_{TV}(\hat{\bm{p}}(t), \bm{p}^*)$. %\sout{We illustrate this coupling in Figure~.}

%\Gauri{The above description looks great! After reading this, I don't think it is necessary to add a figure showing the coupling. The description is already very clear.}

With this coupling, we can quantify the probability for a mismatched dispatching decision between our system and the optimal system.  In our system, recall that $\arrival_i(t)$ denotes the number of jobs dispatched to server~$i$ at time $t$.  We now make a finer distinction between jobs dispatched through exploration and through exploitation under the $\epsilon_t$-exploration policy.  Let $\explore_i(t)$ and $\exploit_i(t)$ denote the numbers of jobs dispatched to server $i$ through exploration and exploitation, respectively.  Then $\arrival_i(t) = \explore_i(t) + \exploit_i(t)$.  Lemma~\ref{lem:mismatch} below upper-bounds the probability for the mismatch that $\exploit_i(t) = 1,  \arrival_i^*(t) = 0$ with the distance $\left|\hat{p}_i(t) - p_i^*\right|$, implying that once the estimates $\hat{p}_i(t)$'s are close to $p_i^*$'s, the probability of such a mismatch is small.
\begin{lem}\label{lem:mismatch}
For any time slot $t$ and any server $i$,
\begin{equation*}
\probability\left[\exploit_i(t) = 1,  \arrival_i^*(t) = 0 \Bigm|  \hat{p}_i(t)\right]\leq \left|\hat{p}_i(t) - p_i^*\right|.
\end{equation*}
\end{lem}
Proof of the lemma is given in \secondversion{\Cref{prf_lem:mismatch}.}{\cite{choudhury2020job}.}
\subsection{Proof of Regret Bound (Theorem~\ref{thm:main})}\label{subsec:proof-regret-bound}
In this section we prove the upper bound in Theorem~\ref{thm:main} on the expected regret $\expectation\left[\regret_{\policy \policy^*}(t)\right] = \expectation\left[\sum_{\tau = 1}^{t-1} \sum_{i = 1}^{\numofserver}\left( \queue_i(\tau) - \queue_i^*(\tau)\right)\right]$ based on several lemmas.
Proof sketches of these lemmas will be given in Section~\ref{subsec:proof-sketch-lemmas}, and the detailed proofs are presented in \secondversion{Appendices~\ref{prf_lem:inst-regret}, \ref{prf_lem:final_busy_period}, \ref{prf_lem:tight_bound_p} and \ref{prf_lem:p_wt} respectively.}{\cite{choudhury2020job}.}


We first note that the difference between $\queue_i(t)$ and $\queue_i^*(t)$ can be written in the following recursive form for any $t$ and $\tau\le t$:
\begin{align*}%\label{rel:queue_process}
    \queue_i(t) - \queue_i^*(t) &= \queue_i(\tau) - \queue_i^*(\tau)\\
    &\mspace{21mu}+\sum_{\ell = \tau}^{t-1}\left(\arrival_i(\ell) - \departure_i(\ell) - \left(\arrival_i^*(\ell) - \departure_i^*(\ell)\right)\right).
\end{align*}
In this proof, we will consider a specific $\tau$ that is the last time queue~$i$ is empty. In particular, define $\busy_i(t)$ as the length of the current busy cycle period as seen at time $t$, i.e.,
\begin{equation}
    \busy_i(t) = \min\left\{s\ge 0 : \queue_i(t - s) =0\right\}.
\end{equation}
Then it is easy to see that for $\tau = t-\busy_i(t)$, we have $\queue_i(\tau)=0$ and $\queue^*_i(\tau)\ge 0$.  In addition, for any $\ell$ with $\tau\le\ell\le t-1$, we have $\departure_i(\ell)=\service_i(\ell)$ since $\queue_i(\ell)>0$.
Based on this choice of $\tau$, the queue length difference can be bounded as follows:
\begin{align}
\mspace{21mu}\queue_i(t) - &\queue_i^*(t)\nonumber
= \queue_i(t-\busy_i(t)) - \queue_i^*(t - \busy_i(t)) + \nonumber  \\
&\mspace{21mu} \sum_{\ell = t- \busy_i(t)}^{t-1}\left(\arrival_i(\ell) - \departure_i(\ell) - \left(\arrival_i^*(\ell) - \departure_i^*(\ell)\right)\right)\nonumber\\
&\leq \sum_{\ell = t- \busy_i(t)}^{t-1}\left(\arrival_i(\ell) - \arrival_i^*(\ell)\right)  + \sum_{\ell = t- \busy_i(t)}^{t-1}\left(\departure_i^*(\ell) - \departure_i(\ell)\right)\nonumber\\
&\le \sum_{\ell = t- \busy_i(t)}^{t-1} \left(\explore_i(\ell) + \exploit_i(\ell) - \arrival_i^*(\ell)\right)\nonumber\\
&\mspace{21mu}+ \sum_{\ell = t- \busy_i(t)}^{t-1} \left(\service_i^*(\ell) - \service_i(\ell) \right)\label{eq:align_queue_a}\\
&= \sum_{\ell = t- \busy_i(t)}^{t-1} \explore_i(\ell) + \sum_{\ell = t- \busy_i(t)}^{t-1} \left(\exploit_i(\ell) - \arrival_i^*(\ell)\right)\label{eq:align_queue_b}\\
&\leq \sum_{\ell = t- \busy_i(t)}^{t-1} \explore_i(\ell) + \sum_{\ell = t- \busy_i(t)}^{t-1} \indicatorofevents_{ \left\{ \exploit_i(\ell)=1, \arrival_i^*(\ell) = 0\right\}},\label{rel:regret_equation}
\end{align}
where \eqref{eq:align_queue_a} uses the facts that $\arrival_i(\ell)=\explore_i(\ell) + \exploit_i(\ell)$, $\departure^*_i(\ell)\le \service^*_i(\ell)$, and $\departure_i(\ell)= \service_i(\ell)$; \eqref{eq:align_queue_b} is due to our coupling $\service_i(\ell)=\service^*_i(\ell)$.


In the upper bound \eqref{rel:regret_equation} on the queue length difference, the first summand comes from exploration.  Since we know that by our $\epsilon_t$-exploration, we have $\expectation[\explore_i(\ell)]=\frac{K\ln \ell}{\ell}$, this summand can be properly bounded if we obtain a suitable upper bound on $\busy_i(t)$.  The second summand in \eqref{rel:regret_equation} comes from exploitation, and it can be bounded with the estimation error through Lemma~\ref{lem:mismatch}.  To formalize the above intuition, we define the following events:
\begin{equation}\label{eqn:event5}
\eventfive := \left\{\busy_i(t) \leq v_i(t),\forall i\right\},\textrm{ where }v_i(t)=\frac{66\ln t}{\freecapacity_{i}^2}, \text{ and}
\end{equation}
\begin{equation}\label{eqn:event6}
\eventsix := \left\{\left| \hat{p}_i(\tau) - p_i^*\right| \leq k_1\min\left\{\sqrt{\frac{ \ln t}{t}}, p_i^*\right\},\forall \tau \in \left[\frac{t}{2} + 1, t\right],\forall i\right\},
\end{equation}
where $k_1$ is a properly chosen constant.
Utilizing these two events, Lemma~\ref{lem:inst-regret} below establishes an upper bound on the expected queue length difference, which enables us to further bound the regret by analyzing the busy period and the estimation error in service rates.
%
\begin{lem}\label{lem:inst-regret}
There exists a $t_0$ such that for any time $t\ge t_0$, the total expected queue length difference can be bounded as
\begin{multline}
\sum_{i=1}^K\expectation\left[\queue_i(t) - \queue_i^*(t)\right]
\le\sum_{i=1}^K\frac{2v_i(t)\ln t}{t} \\
+ \sum_{i:p_i^*>0} k_1v_i(t) \sqrt{\frac{\ln t}{t}} + t\probability\left(\left(\eventfive\right)^c\right) + 2t\probability\left(\left(\eventsix\right)^c\right).
\end{multline}
\end{lem}


\begin{figure}
    \centering
    \includegraphics[width=80mm]{draft_pics/diagrams/timeline.pdf}
    \caption{Time structure of lemmas in proof of Theorem~\ref{thm:main}.}
    \label{fig:dia_timeline}
\end{figure}
With Lemma~\ref{lem:inst-regret}, to bound the expected regret, now it suffices to bound the probabilities $\probability\left(\left(\eventfive\right)^c\right)$ and $\probability\left(\left(\eventsix\right)^c\right)$, which are established in Lemmas~\ref{lem:final_busy_period} and \ref{lem:tight_bound_p} below.  We demonstrate the time structure of the lemmas in Figure~\ref{fig:dia_timeline}.
\begin{lem}[Busy Period Bound]\label{lem:final_busy_period}
There exist a constant $k_2$ and a $t_0$ such that for any $t\ge t_0$, the event $\eventfive$ defined in \eqref{eqn:event5} satisfies
\begin{equation}
\probability\left(\left(\eventfive\right)^c\right) \leq 4\numofserver\left( \frac{1}{t^{7}} + \frac{k_2 + 1}{t^3} + \frac{1}{t^4}\right).
\end{equation}
\end{lem}
\begin{restatable}[Estimation Error Bound]{lem}{lemERRORestimate}
\label{lem:tight_bound_p}
There exist a constant $k_2$ and a $t_0$ such that for any $t\ge t_0$, the event $\eventsix$ defined in \eqref{eqn:event6} satisfies  
\begin{multline}
\probability\left(\left(\eventsix\right)^c\right) \leq \numofserver\left(\frac{1}{t^7} + \frac{k_2 + 1}{t^3}\right) \\+\sum_{i: p_i^*>0}\left(\frac{1}{t^3} + t \exp\left(-\frac{p_i^*\lambda t}{128}\right) +
t\exp\left(-\frac{\freecapacity_i^2 t}{4}\right)\right).
\end{multline}
\end{restatable}

Finally, we choose a common $t_0$ for Lemmas~\ref{lem:inst-regret}--\ref{lem:tight_bound_p} and a common $k_2$ for Lemmas~\ref{lem:final_busy_period} and \ref{lem:tight_bound_p}, and put Lemmas~\ref{lem:inst-regret}--\ref{lem:tight_bound_p} together to get
\begin{align}
&\mspace{21mu}\expectation\left[\regret_{\policy \policy^*}(t)\right]\nonumber\\
&= \sum_{\tau = 1}^{t_0-1}\sum_{i=1}^K \expectation\left[\queue_i(\tau)-\queue^*_i(\tau)\right] + \sum_{\tau = t_0}^{t-1} \sum_{i=1}^K \expectation\left[\queue_i(\tau)-\queue^*_i(\tau)\right]\nonumber\\
&\le t_0^2 + \sum_{\tau = t_0}^{t-1} \sum_{i=1}^K\frac{2v_i(\tau)\ln \tau}{\tau}
+\sum_{\tau = t_0}^{t-1}\sum_{i:p_i^*>0} k_1v_i(\tau) \sqrt{\frac{\ln \tau}{\tau}}\nonumber\\
&\mspace{21mu}+\sum_{\tau = t_0}^{t-1}\tau\cdot \numofserver\left(\frac{4}{\tau^{7}} + \frac{4k_2 + 4}{\tau^3} + \frac{4}{\tau^4}\right)+\sum_{\tau = t_0}^{t-1}2\tau\cdot \numofserver\left(\frac{1}{\tau^{7}} + \frac{k_2 + 1}{\tau^3}\right)\nonumber\\
&\mspace{21mu}+\sum_{\tau = t_0}^{t-1}2\tau\cdot\sum_{i: p_i^*>0}\left(\frac{1}{\tau^3} + \tau\exp\left(-\frac{p_i^*\lambda \tau}{128}\right) +\tau\exp\left(-\frac{\freecapacity_i^2 \tau}{4}\right)\right)\\
& = t_0^2 + \sum_{\tau = t_0}^{t-1} \sum_{i=1}^{\numofserver}\frac{132 \ln^2 \tau}{\freecapacity_i^2 \tau} + \sum_{\tau = t_0}^{t-1}\sum_{i: p_i^* > 0} \frac{66k_1\ln \tau}{\freecapacity_i^2}\sqrt{\frac{\ln \tau}{\tau}}  \nonumber\\
&\mspace{21mu} + \numofserver\sum_{\tau = t_0}^{t-1} \left( \frac{6}{\tau^{6}} + \frac{6k_2 + 6}{\tau^2} + \frac{4}{\tau^3}\right)\nonumber\\
&\mspace{21mu} + 2\sum_{\tau = t_0}^{t-1}\sum_{i: p_i^*>0}\left(\frac{1}{\tau^2} + \tau^2\exp\left(-\frac{p_i^*\lambda \tau}{128}\right) + \tau^2\exp\left(-\frac{\freecapacity_i^2 \tau}{4}\right)\right)\\
&=\sum_{\tau = t_0}^{t-1}\left(\sum_{i: p_i^* > 0} \frac{66k_1\ln \tau}{\freecapacity_i^2}\sqrt{\frac{\ln \tau}{\tau}}+\sum_{i=1}^{\numofserver}\frac{132 \ln^2 \tau}{\freecapacity_i^2 \tau}\right) +  \order\left(1\right),\nonumber
\end{align}
which completes the proof of Theorem~\ref{thm:main}.\qed

\begin{remark*}
Our proof techniques used the \emph{absolute} difference in the routing probabilities to analyze the difference in queue lengths.
We comment that it might be possible for one to prove a tighter regret upper bound by considering the actual difference in routing probabilities, but the analysis will become much more challenging.  Specifically, inaccurate routing probabilities can actually instantaneously benefit the queues whose $\hat{p}_i(t)$ is smaller than the optimal $p^*_i$.  This is a phenomenon not seen in multi-armed bandit problems, and it is worth further investigation.
\end{remark*}

\subsection{Proof Sketches of Lemmas~\ref{lem:inst-regret}--\ref{lem:tight_bound_p}}\label{subsec:proof-sketch-lemmas}
% -------------------------------------------------------------------
% \include{plot}
\begin{figure*}
    \centering
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[scale = 0.35]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_1.pdf}
        \caption{$\lambda = 0.1$}
    \end{subfigure}
    \begin{subfigure}{0.33\linewidth}  
        \centering 
        \includegraphics[scale = 0.35]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_2.pdf}
        \caption{$\lambda = 0.2$}
    \end{subfigure}
    \begin{subfigure}{0.33\linewidth}  
        \centering 
        \includegraphics[scale = 0.35]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_3.pdf}
        \caption{$\lambda = 0.4$}
    \end{subfigure}
        \centering
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[scale = 0.35]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_5.pdf}
        \caption{$\lambda = 0.5$}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.33\linewidth}  
        \centering 
        \includegraphics[scale = 0.35]{plots/simulation/policy_compare/transient_regret_compare_servicetime_coupled_memory_manypolicy_var_timestep10000_run12000_7.pdf}
        \caption{$\lambda = 0.7$}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.33\linewidth}  
        \centering 
        \raisebox{1cm}{\includegraphics[scale = 0.9, trim={2mm 2mm 1mm 2mm}, clip]{plots/simulation/policy_compare/legend.pdf}}
    \end{subfigure}
    \caption{Regret vs time for various policies. The shaded region represent $\pm2\sigma$ boundary of the mean regret. TS and UCB performs well in load load regime, while $K/t$-greedy exploration policy performs well in higher traffic regimes. Our policy moderately in very low load regime and performs well in higher traffic regimes. %\Weina{Need to replace the ``-greedy'' with ``-exploration'' to be consistent with Section~4.} \Gauri{Reorder the plots such that our policy is either the first or the last in the legend. Also, in the legend, say 'Proposed $\numofserver \log t/t$-exploration policy'. Adding the word proposed will further avoid confusion about which one of our policy}
    %\Gauri{This figure looks great! To save space, is it possible to make a vertical legend and put it alongside the second row of plots?}
    %\Gauri{A minor comment -- the color of the TS curve looks very similar to green. Maybe change it to a magenta or pink color?}
    %\Tuhin{number format}
    %\Tuhin{Changed number format, legend and the colours}
    }
    \label{fig:regret_policies}
\end{figure*}
% -------------------------------------------------------------------------------


% -------------------------------------------------------------------

The detailed proofs of Lemmas~\ref{lem:inst-regret}, \ref{lem:final_busy_period}, \ref{lem:tight_bound_p} and \ref{lem:p_wt} are presented in \secondversion{Appendices~\ref{prf_lem:inst-regret}, \ref{prf_lem:final_busy_period}, \ref{prf_lem:tight_bound_p} and \ref{prf_lem:p_wt} respectively.}{\cite{choudhury2020job}.}

\Cref{lem:inst-regret} can be proven using a series of conditioning on event $\eventfive$, event $\eventsix$ and also the estimated  $\hat{\bm{p}}(t)$.  Then the construction of $\eventfive$ gives an upper bound on the busy period, \Cref{lem:mismatch} helps translate the number of mismatches into the error in estimation, and finally the construction of $\eventsix$ upper bounds the estimation error.

Next for Lemmas~\ref{lem:final_busy_period} and \ref{lem:tight_bound_p}, we will just highlight a key lemma used in their proofs, presented as Lemma~\ref{lem:p_wt}.  
Lemma~\ref{lem:p_wt} below states that for any large enough time $t$, the estimated optimal support set, $\support\left(\lambda, \hat{\bm{\mu}}(t)\right)$, is correct (i.e., equal to the true optimal support set $\support\left(\lambda, \bm{\mu}\right)$) for a period of time $[w(t),t]$ with high probability, where $w(t)=2\exp\left(\Theta\left(\sqrt{\ln t}\right)\right)$.  Moreover, during this period of time, the rate at which we dispatch jobs to each server~$i$ lies between $\lambda p^*_i/2$ and $\mu_i-\freecapacity_i/2$; i.e., the arrival rate to each server is no smaller than half of the rate under the optimal weighted random routing, but still leaves at least half of residual capacity under the optimal weighted random routing.  We call the period of time $[w(t),t]$ the \emph{quick learning period} since we have ``locked'' the correct support set and spend all exploitation jobs on learning the service rates of servers in the correct support set.  This time structure of Lemma~\ref{lem:p_wt} is also illustrated in Figure~\ref{fig:dia_timeline}.

\begin{restatable}[Quick Learning Period]{lem}{restateLEMMApWT}
\label{lem:p_wt}
Define the event $\eventone$ as 
\begin{equation}\label{event1}
    \eventone := \eventoneone \cap \eventonetwo, \text{ where}
\end{equation} 
\begin{align*}
\eventoneone&:=\left\{\support\left(\lambda, \hat{\bm{\mu}}(\tau)\right) = \support(\lambda,\bm{\mu}),\forall \tau \in \left[w(t) + 1, t\right]\right\},\\
\eventonetwo&:= \left\{\frac{\lambda p_i^*}{2} \leq
\expectation\left(\arrival_i(\tau) \mmiddle \hat{p}_i(\tau)\right) \leq \mu_i - \frac{\freecapacity_i}{2},\forall i,\forall \tau \in \left[w(t) + 1, t\right]\right\}.
\end{align*}
Then there exist a constant $k_2$ and $t_0$ such that for all $t\geq t_0$,
\begin{equation*}
    \probability\left(\left(\eventone\right)^c\right)\leq \numofserver\left(\frac{1}{t^{7}} + \frac{k_2 + 1}{t^3}\right).
\end{equation*}
\end{restatable}
Based on Lemma~\ref{lem:p_wt}, Lemmas~\ref{lem:final_busy_period} and \ref{lem:tight_bound_p} can be proven through the following outline.  The bound on the busy period in Lemma~\ref{lem:final_busy_period} relies on the property that $\expectation\left(\arrival_i(\tau) \mmiddle \hat{p}_i(\tau)\right) \leq \mu_i - \frac{\freecapacity_i}{2}$ in the event $\eventonetwo(t)$, which leads to a negative drift in the queue length.  For the bound on the estimation error in Lemma~\ref{lem:tight_bound_p}, the property that $\expectation\left(\arrival_i(\tau) \mmiddle \hat{p}_i(\tau)\right)\ge \frac{\lambda p_i^*}{2}$ in the event $\eventonetwo$ guarantees that the expected number of jobs we dispatch to each server in the optimal support set is at least linear in time, resulting in enough samples for estimating the service rates of these servers.  For servers outside of the optimal support set, event $\eventoneone$ ensures that we do not dispatch exploitation jobs to those servers.



==> old/old_files2/simulation.tex <==
\section{Simulation Results}
\label{sec:simulation}

In this section we compare the expected regret of our proposed $K \ln t/t$-exploration policy with three other policies that are also based on multi-armed bandits: (i) an $\epsilon_t$-exploration with a faster decaying exploration probability $\epsilon_t=\numofserver/t$, (ii) a variant of the upper confidence bound (UCB) policy \citep{auer2002finite}, and (iii) a variant of Thompson sampling \citep{thompson1933likelihood, agrawalgoyal2012thompson}, described in more detail below. Our simulation set-up consists of a system of $6$ servers with service rates $\mu_i$ such that $\mu_i = 2^{i-1} \mu_1$, and $\sum_{i=1}^{6} \mu_i = 0.99$. We consider $5$ different job arrival rates $\lambda = 0.1, 0.2, 0.4, 0.5 \text{ and } 0.7$. To compute the regret, we find the cumulative queue length $\sum_{\tau=1}^{t} \sum_{i=1}^{\numofserver} \queue_i(\tau)$ for $t \in [0,2\times 10^7]$ for each of the policies and the optimal weighted random routing policy. The regret $\regret_{\policy \policy^*}(t) = \sum_{\tau = 1}^t \sum_{i = 1}^{\numofserver}( \queue_i(\tau) - \queue_i^{*}(\tau))$ is then averaged over $20000$ simulation runs.
% This comparison demonstrates that these other policies may either explore too much or too little depending on the traffic regime, whereas our proposed policy gives lower and more consistent regret.
%
%The the mean cumulative queue length for all the policy is computed as a function of time, where the mean is taken over $20000$ samples and each sample is run for $2\times 10^7$ units of time. The mean cumulative queue length for the optimal weighted random routing is also computed in similar fashion. Finally the regret is calculated by taking the difference between the mean cumulative length of the proposed policies and the optimal weighted random routing policy. 
%
We compare the regret of our proposed policy with that of the three other policies in \Cref{fig:regret_policies}.

\vspace{0.1cm} \noindent  \textbf{$\numofserver/t$-exploration:} Instead of the $\epsilon_t = \numofserver \ln t/t$ probability of exploration used in our proposed policy, this policy sets $\epsilon_t = K/t$, which decays much faster. Because of the aggressive exploitation, this policy can exclude servers from the optimal support set, similar to the situation described in \Cref{subsec:exploration}. As a result, we observe linearly increasing regret in \Cref{fig:regret_policies} and it is clearly outperformed by our proposed $\numofserver \ln t /t$-exploration policy, especially for small $\lambda$. For larger $\lambda$, only a small amount of exploration is required to ensure that none of the servers in the optimal support set is excluded and hence the performance of the policy improves. %Therefore, a $\numofserver/t$ exploration probability is insufficient to correctly identify the support set $\mathcal{S}$. %$\frac{K}{t}-exploration$, especially in the low and moderate load regime. %; however, its performance improves with the load of the system. Our algorithm performs well in almost load regimes and the reason is that it is balancing the trade-off between exploration and exploitation.
    
%each time slot, the policy sends any arriving job random to any server with probability $\frac{K}{t}$, else if uses $\bm{p}^*(\lambda, \hat{\bm{\mu}}(t))$ to route the job. Since, the probability of exploration at each time is $o(K\log t/t)$ \Gauri{Instead of using $o$, maybe just say that the probability of exploration is decays much faster than our policy, which explores with probability $\numofserver \log t/t$ } , this is a more exploitative policy as compared to our proposed policy given in \Cref{poli:bandit}.
    
\vspace{0.1cm} \noindent  \textbf{Upper Confidence Bound (UCB) variant}: This is a variant of the UCB policy \citep{auer2002finite}, where in each time slot, we compute the routing probability vector $f\left(\lambda, \bm{\mu}^{UCB}(t)\right)$ using optimistic estimates of the service rates $\mu_i^{UCB}(t) = \hat{\mu}_i(t) + \frac{1}{\sqrt{N_i(t)}}$, where $N_i(t)$ is the number of jobs that have departed from server $i$ till time $t$. Using optimistic service rate estimates induces more exploration of slower servers by including them in the support set more often. %And as $N_i(t) \rightarrow \infty$ for $i \in \mathcal{S}$, the policy converge to the optimal random routing policy. 
As a result, UCB explores more aggressively than our proposed $\numofserver \ln t /t$-exploration policy and therefore, UCB performs well for small $\lambda$. However, as $\lambda$ increases, the additional exploration results in a higher regret. 
    
% The random routing vector send less jobs in the slower servers. Hence, $N_i(t)$ is usually small for the slower servers. Using $\bm{\mu}^{UCB}(t)$ instead of $\hat{\bm{\mu}}(t)$ to calculate the routing vector hence pushes a server with slower estimate in the support set. Hence, this is a more explorative policy as compared to our proposed policy given in \Cref{poli:bandit}. However, because of more exploration it usually do not exclude servers in the optimal support set. 
   
\vspace{0.1cm} \noindent  \textbf{Thompson Sampling (TS) variant}: This is a variant of the Thompson sampling \citep{thompson1933likelihood, agrawalgoyal2012thompson}. At each time slot, we compute the routing probability vector $f\left(\lambda, \bm{\mu}^{TS}(t)\right)$ by sampling the service rates $\mu_i^{TS}(t)$ from a Beta distribution with parameters $\hat{\mu}_i(t)N_i(t) + 1$ and $(1 - \hat{\mu}_i(t))N_i(t) + 1$. The variance of the Beta distribution is roughly $O(1/N_i(t))$. The exploration in this policy comes from the fact $\mu_i^{TS}(t)$ lies within $\hat{\mu}_i(t) \pm O(1/\sqrt{N_i(t)})$ region. While similar to UCB, TS performs less exploration of slow servers because $\mu_i^{TS}(t)$ can be lower than the optimistic estimates $\hat{\mu}_i(t)$. Thus, we observe in \Cref{fig:regret_policies} that the regret of TS is similar to, but better than UCB.

%$\frac{K}{t}-exploration$, unlike UCB and TS, performs terribly in the low and moderate load regime; however, its performance improves with the load of the system. Because of aggressive exploitation, the policy sometimes excludes servers from the optimal support set in the low and moderate load regime. The situation is similar to the example we discussed in \Cref{subsec:exploration}. In higher load regimes, most of the servers are included the optimal support set. Only a small amount of exploration is required to ensure that none of the servers in the optimal support set is excluded and hence the performance of the policy improves. Our algorithm performs well in almost load regimes and the reason is that it is balancing the trade-off between exploration and exploitation.

A common trend in these results is that %the relative performance of these policies differs based on arrival rate $\lambda$ -- 
we need more exploration in the low $\lambda$ regime and less exploration for larger $\lambda$. In the low $\lambda$ regime, the optimal weighted random routing usually sends the job to the fastest server, which essentially reduces to a typical MAB setting. Hence, UCB and TS perform well in very low $\lambda$ regime. However, their performance worsens as $\lambda$ increases due to over-exploration. Unlike traditional MAB problems where the user either explores or exploits at each time, in queueing bandits every exploitation also acts as an exploration. As long as the servers in the optimal support set has a non-zero probability of assignment associated with it, there would be a steady flow of jobs to those servers which in turn will improve their service rate estimates. 

%\Gauri{If there is space, shall we also show a plot of how the estimation errors $p_i(t)-p_i^*$ for each of these policies? It would be interesting to see how to change over time. We could show bar plots of these for $3$ different times, maybe $t= 10000$, and $t = 1000000$}


%\Cref{fig:regret_policies} shows the performance of different policies in different load regimes. TS and UCB perform well in very low load regime. In very low load regimes, the optimal weighted random routing usually sends the job to the fastest server, which essentially changes the problem to a typical MAB setting. Hence, UCB and TS perform well in very low load regime. However, their performance worsens as the load increase. The main reason for the poor performance is over-exploration. Unlike traditional MAB problem, where the user either explores or exploits at each time, in queueing bandits every exploitation also acts as an exploration. As long as the servers in the optimal support set has a non-zero probability of assignment associated with it, there would be a steady flow of jobs in those servers which in turn will improve their service rate estimates. Since UCB and TS are designed for MAB problems, they explore more aggressively than required. 




